Shuffle and Joint Differential Privacy for Generalized Linear Contextual Bandits

We present the first algorithms for generalized linear contextual bandits under shuffle differential privacy and joint differential privacy. While prior work on private contextual bandits has been restricted to linear reward models -- which admit closed-form estimators -- generalized linear models (GLMs) pose fundamental new challenges: no closed-form estimator exists, requiring private convex optimization; privacy must be tracked across multiple evolving design matrices; and optimization error must be explicitly incorporated into regret analysis. We address these challenges under two privacy models and context settings. For stochastic contexts, we design a shuffle-DP algorithm achieving $\tilde{O}(d^{3/2}\sqrt{T \log T}/\sqrt{\varepsilon})$ regret in dominant term, differing from the non-private rate by a factor of $\sqrt{d/\varepsilon}$. For adversarial contexts, we provide a joint-DP algorithm with regret $\tilde{O}\!\big(d\sqrt{T} \log T + d^{3/4}\sqrt{T/\varepsilon}\,(\log T)\,(d + \log T)^{1/4}\big)$ -- matching the non-private rate $\tilde{O}(d\sqrt{T} \log T)$ in the leading term, with privacy contributing only an additive correction. Unlike prior work on locally private GLM bandits, our methods require no spectral assumptions on the context distribution beyond $\ell_2$ boundedness.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerYes{} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerYes{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNo{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work is of theoretical interests and we do not see any social impacts.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> checklist_aistats.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

  \item For all models and algorithms presented, check if you include:
  \begin{enumerate}
    \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
    \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
    \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes]
  \end{enumerate}

  \item For any theoretical claim, check if you include:
  \begin{enumerate}
    \item Statements of the full set of assumptions of all theoretical results. [Yes]
    \item Complete proofs of all theoretical results. [Yes]
    \item Clear explanations of any assumptions. [Yes]     
  \end{enumerate}

  \item For all figures and tables that present empirical results, check if you include:
  \begin{enumerate}
    \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
    \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes]
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
  \end{enumerate}

  \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
  \begin{enumerate}
    \item Citations of the creator If your work uses existing assets. [Not Applicable]
    \item The license information of the assets, if applicable. [Not Applicable]
    \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
    \item Information about consent from data providers/curators. [Not Applicable]
    \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
  \end{enumerate}

  \item If you used crowdsourcing or conducted research with human subjects, check if you include:
  \begin{enumerate}
    \item The full text of instructions given to participants and screenshots. [Not Applicable]
    \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
    \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
  \end{enumerate}

\end{enumerate}


==> content.tex <==
\section{Introduction}

%\sss{ToDo's: Experiments and literature on amplification via shuffling}
In the contextual bandit problem \cite{NIPS2011_e1d5be1c,newsarticlerecomcontextualbandits,pmlr-v15-chu11a,pmlr-v9-lu10a}, at each time step \( t \), the learner is presented with a set of \( K \) arms $\gX_t$ (called the context set), each represented by a \( d \)-dimensional feature vector. The learner must then choose an arm \( x_t \in \gX_t \) to pull, receiving a reward \( r_t \) associated with the selected arm \( x_t \). The regret in a round is defined as the difference between the maximum possible reward and the reward obtained in that round. The goal of the algorithm is to choose an action at every step such that the cumulative regret (also called the regret of the algorithm) is minimized over a specified number of rounds $T$. This problem has been extensively studied for various classes of reward models, for example, a) linear models \cite{10.5555/944919.944941,pmlr-v15-chu11a,NIPS2011_e1d5be1c, hanna2023contexts,kuroki2024bestofbothworldsalgorithmslinearcontextual}, b) logistic models \cite{faury2020improvedoptimisticalgorithmslogistic, pmlr-v130-abeille21a, faury2022jointlyefficientoptimalalgorithms,NEURIPS2023_5ef04392,10.5555/3327345.3327373}, and c) generalized linear models \cite{NIPS2010_c2626d85, li2017provablyoptimalalgorithmsgeneralized,sawarni2024generalizedlinearbanditslimited}. 


% —in settings ranging from news article recommendation \cite{newsarticlerecomcontextualbandits} to healthcare \cite{healthcarecontextualbandits} and education \cite{educationcontextualbandits}, 

At each time step $t$, the contextual-bandit algorithm interacts with a new user whose context set is $\gX_t$, after which the user receives a reward $r_t$. Given the wide applicability of contextual bandits—often processing sensitive personal data, protecting both the context and reward sets from adversaries becomes paramount. In this paper, we study generalized linear models with DP constraints under two different setups (called $\mone$ and $\mtwo$) under bounded reward and context vectors. In $\mone$, the context set $\gX_t$ is generated stochastically, whereas in $\mtwo$, it is generated adversarially. In $\mone$, we study the multi-round shuffled model of DP \cite{erlingsson2019amplification,Cheu2021ShufflePS, pmlr-v162-chowdhury22a}, whereas in $\mtwo$, we study joint DP \cite{shariff2018differentiallyprivatecontextuallinear,azize2024concentrateddifferentialprivacybandits} where the action at each step is differentially private with respect to reward-context pairs at other steps. In the shuffled model of DP, each user sends noisy functions of their true context-reward pair to the shuffler, which shuffles it before sending it to the learner, and the privacy guarantee holds with respect to the shuffled data received by the learner. One can observe, via a simple application of Billboard lemma in \cite{mechanism_design_large_games}, that shuffled DP implies joint DP. Thus, we study a weaker notion of privacy in $\mtwo$.% for the case of adversarial contexts. 


The algorithms in setups $\mone$ and $\mtwo$ are inspired by batched non-private algorithms of \cite{sawarni2024generalizedlinearbanditslimited}; both involve only a limited (polylogarithmic) number of policy updates. In the case of stochastic contexts, the algorithm pre-determines a set of $M$ rounds at which policy updates occur, with each batch consisting of consecutive time steps under a fixed policy. In contrast, in the adversarial context setup, policy switches occur adaptively. Under the shuffled model of privacy in $\mone$, on a high level, each user reports noisy functions of the $(\gX_t, r_t)$ pair, and a shuffler permutes the signals received from different users in a batch. The algorithm can only access the shuffled data from previous batches to compute its policy for the next batch. The shuffled DP model does not extend naturally to the adaptive algorithm in $\mtwo$. To decide the policy-switching round for a given batch, the algorithm must inspect that batch’s data—information that is hidden until after shuffling—making real-time updates infeasible. We, therefore, adopt the weaker notion of joint DP. Our main contributions are as follows.

\begin{itemize}%[leftmargin = 10pt]
    \item In the stochastic context setting $\mone$, we design a shuffle‐DP algorithm that achieves a regret of $\tilde{O}(d^{3/2}\sqrt{T/\varepsilon})$. This is only a factor $\sqrt{d}/\sqrt \varepsilon$ worse than the order‐optimal bounds of the non‐private method in \cite{sawarni2024generalizedlinearbanditslimited}. 
    \sss{Write technical novelty over linear bandits her}
    The shuffle private algorithm requires a smart combination of techniques from shuffle convex optimizer \cite{Cheu2021ShufflePS} for optimization and shuffle private summation \cite{ghazi2021multiAnon} for mean estimation to send multiple bits of messages at each round.

    \item We give a jointly DP algorithm for the adversarial context setting $\mtwo$ 
with regret $\tilde{O}(d\sqrt{T/\varepsilon})$, matching the non-private 
order-optimal rate of \cite{sawarni2024generalizedlinearbanditslimited} 
up to a $1/\!\sqrt{\varepsilon}$ factor. 
\sss{Write technical novelty over linear bandits her}
The main technical novelty is 
ensuring that the switching steps remain private under continual 
observation, which we achieve using the binary-tree mechanism 
\cite{continualstatsrelease,continualobservation} together with an 
advanced composition analysis of log-likelihood ratios 
\cite{kairouz2015compositiontheoremdifferentialprivacy,fullyadaptiveprivacy}.


 % which is used to prove the $(\varepsilon,\delta)$ in-distinguishability of time-steps of the policy switches. 

    \item Our algorithms incur no dependence on the instance-specific parameter $\kappa$, which may grow exponentially with the dimension, in the leading $\sqrt{T}$ term, as in the non-private setting \cite{sawarni2024generalizedlinearbanditslimited}. For completeness, we also prove a lower bound of $\Omega(d\sqrt{T}+d/\varepsilon)$ using Assouad's technique. This closely matches the private lower bound for linear contextual bandits \cite{pmlr-v162-he22e}. 


    \item To the best of our knowledge, this is the first work to address either joint DP or shuffled DP in generalized linear contextual bandits. In comparison, Han et al.~\cite{han2021generalizedlinearbanditslocal} study the stronger local privacy model for stochastic contexts, but their analysis relies on spectral assumptions on the covariance matrix of the context distribution. In contrast, our algorithms dispense with such assumptions, requiring only $\ell_2$-bounded context vectors and rewards.
\end{itemize}

% We thus obtain a nearly tight characterization of DP in contextual bandits, closely mirroring the non-private setting in both stochastic and adversarial contexts.

\begin{remark}
    While the algorithms in settings $\mone$ and $\mtwo$ require time horizon $T$ to be known in advance, they can be made anytime using the standard doubling trick \cite{besson2018doubling}, at the cost of only a constant-factor increase in minimax regret.
\end{remark}

\textbf{Roadmap.} \Cref{sec:def_privacy_bandits} introduces the local, shuffle, central, and joint DP models for contextual bandits, and \Cref{sec:notations_and_prelims} covers preliminaries for generalized linear bandits. Our main results are in \Cref{sec:glm_alg,sec:glm_jdp}, which present shuffled and joint-DP algorithms for stochastic and adversarial contexts, respectively. For completeness, we prove a lower bound in \cref{sec:private_lower_bound}. Synthetic experiments appear in \Cref{sec:simulations}, with full regret and privacy analysis deferred to the appendix.



%shuffle private algorithm \cref{alg:shuffled_glm} for stochastic contexts in \cref{sec:glm_alg}




%Under shuffle DP for stochastic contexts, however, our algorithm pays an extra $\sqrt{d}$ factor—where $d$ is the context dimension—because we cannot yet incorporate distributional optimal design in a private way. Whether one can privately compute such an optimal design (and thereby eliminate the $\sqrt{d}$ gap) remains an intriguing open problem. By contrast, under joint DP the dependence on $d$ exactly matches the non-private guarantee.

\section{Related Work}

Several works have explored the problem of limited adaptivity in linear contextual bandits, including \cite{ruan2021linearbanditslimitedadaptivity,NIPS2011_e1d5be1c,han2020sequentialbatchlearningfiniteaction,hanna2023contexts}, covering both stochastic and adversarial contexts. Limited adaptivity is important since policies cannot be changed frequently in real settings such as clinical trials \cite{TheInternationalStroke1997}, online advertising \cite{10.1287/mksc.2016.1023}, and recommendations \cite{newsarticlerecomcontextualbandits}. Towards this, there have been several works on logistic bandits \cite{faury2022jointlyefficientoptimalalgorithms}, generalized linear models \cite{li2017provablyoptimalalgorithmsgeneralized, sawarni2024generalizedlinearbanditslimited}, and linear models \cite{han2020sequentialbatchlearningfiniteaction, ruan2021linearbanditslimitedadaptivity}. In this work, we utilize limited adaptivity to obtain shuffled and joint DP guarantees in stochastic and adversarial contextual setups respectively. 

Privacy amplification by shuffling has been widely studied as a way to strengthen local guarantees, showing that randomly shuffling locally privatized data can achieve central-DP–level protection with much better utility \cite{bittau2017prochlo,erlingsson2019amplification,Cheu_2019,feldman2021hiding}. In particular, multi-message protocols for tasks like binary summation and histograms further demonstrate that sending even a few short messages per user can significantly tighten shuffling guarantees \cite{ghazi2020pure,balle2020multiMessage,ghazi2021multiAnon}.


%Batched algorithms might also be necessary for shuffled privacy which proceeds in rounds and we utilize limited adaptivity in contextual bandit algorithms to obtain privacy guarantees under both the adversarial and stochastic setup.




Researchers have studied shuffled DP in linear contextual bandits in \cite{pmlr-v167-garcelon22a,pmlr-v162-chowdhury22a}, and in $K$-armed bandits in \cite{mabshuffle}. \cite{shariff2018differentiallyprivatecontextuallinear} first introduced joint DP for linear contextual bandits, using binary tree mechanisms \cite{continualobservation} to update design matrix estimators at each step. \cite{azize2024concentrateddifferentialprivacybandits} improved the regret bounds under relaxed assumptions where context sets are public and only rewards require privacy protection. \cite{chakraborty2024fliphatjointdifferentialprivacy} further tightened regret bounds for sparse linear contextual bandits. \cite{zheng2021locallydifferentiallyprivatecontextual} studied local DP in this setting, but their regret scales as $\tilde{O}(T^{3/4}/\varepsilon)$. More recently, \cite{li2024optimalregretlocallyprivate} proposed an alternative approach that achieves $\tilde{O}(\sqrt{T}/\varepsilon)$ regret, though their method incurs exponential dependence on the dimension $d$ of the context vectors.



%Under the setting of shuffled DP, this problem has been examined for linear contextual bandits in \cite{pmlr-v167-garcelon22a,pmlr-v162-chowdhury22a} and for $K$ armed multi-armed bandits in \cite{tenenbaum2021differentiallyprivatemultiarmedbandits}. Joint DP for linear contextual bandits was first introduced in \cite{shariff2018differentiallyprivatecontextuallinear}, where design matrix estimators were updated at each step using the binary tree mechanism \cite{continualobservation}. The work in \cite{azize2024concentrateddifferentialprivacybandits} improved regret bounds under a relaxed assumption where context sets are public and only rewards require privacy protection. Further, \cite{chakraborty2024fliphatjointdifferentialprivacy} tightened regret bounds for sparse linear contextual bandits. Local DP in this setting has been studied in \cite{zheng2021locallydifferentiallyprivatecontextual}, but the regret scales as $\tilde{O}(T^{3/4}/\varepsilon)$. A recent alternative approach in \cite{li2024optimalregretlocallyprivate} achieves regret scaling as $\tilde{O}(\sqrt{T}/\varepsilon)$, though it suffers from exponential dependence on the dimension $d$ of the context vector sets.


In linear bandits, \cite{osamaalmostfree} show that one can achieve joint DP almost for free, with only an additive logarithmic term involving $\varepsilon$. \cite{azize2024concentrateddifferentialprivacybandits} extend this to linear contextual bandits under relaxed assumptions—specifically, with public contexts and private rewards—and demonstrate that privacy comes at negligible cost. \cite{chakraborty2024fliphatjointdifferentialprivacy} further show that in sparse linear contextual bandits, one can obtain nearly optimal joint DP guarantees when the sparsity parameter satisfies $s \ll d$. \cite{pmlr-v247-azize24a} identifies the characterization of optimal regret for $(\varepsilon, \delta)$-jointly DP linear contextual bandits in the general case as an open problem.
Prior work on differentially private contextual bandits under the generalized linear model (GLM) is limited. Han et al.~\cite{han2021generalizedlinearbanditslocal} analyze the stronger \emph{local} DP model and achieve $\tilde{O}(T^{1/2}/\varepsilon)$ regret, but their results rely on eigenvalue assumptions on the context distribution. To the best of our knowledge, no existing work addresses \emph{shuffled} or \emph{joint} DP in GLM bandits. Our algorithms close this gap: we impose no spectral assumptions on the context distribution and achieve $\tilde{O}(\sqrt{T/\varepsilon})$ regret in both privacy settings.





%For the case of linear bandits, it has been recently shown by \cite{osamaalmostfree} that joint DP can be obtained (almost) for free with only additive logarithmic term that contains $\varepsilon$. However, for linear contextual bandits under slightly relaxed public contexts and private rewards, \cite{azize2024concentrateddifferentialprivacybandits} show that it is possible to attain privacy (almost) for free. Similarly for the case of sparse linear contextual bandits, a recent work \cite{chakraborty2024fliphatjointdifferentialprivacy} showed that privacy can be obtained almost for free when the sparsity parameter $s<<d$. It is left as an interesting open problem \cite{pmlr-v247-azize24a} to characterize the optimal regret for $(\varepsilon,\delta)$ joint differentially private linear contextual bandits in the general case. Prior work on differentially private contextual bandits under the generalized linear model (GLM) is limited. The closest result, from \cite{han2021generalizedlinearbanditslocal}, achieves $\tilde{O}(T^{1/2}/\varepsilon)$ regret under \emph{local} differential privacy (LDP), but requires eigenvalue assumptions on the context distribution.  To our knowledge, no work addresses \emph{shuffled} or \emph{joint} DP for GLM bandits---nor do we impose eigenvector assumptions on contexts and attains $\tilde{O}\left(\frac{\sqrt T}{\varepsilon}\right)$ regret in both settings.


% \mg{last two paragraphs have several lines repeated -- discussion of Azize paper and Chakraborty paper}




% \sss{to be written below, also cite some of osama's dp bandit papers like getting regret for free and maybe some other bandits as well also cite fliphat paper}










%with the objective of maximizing the cumulative reward over time. 






% the expectation of the reward $r_t$ is a linear function of the arm chosen at  , formally the $E[r_t] = \langle \theta^{*}, x_t \rangle$ 


% \sss{Some notations of policy and all to be defined properly.}
% \paragraph{Linear Contextual Bandits.} There is a hidden vector $\theta \in \mathbb{R}^d$ ($\norm{\theta} \leq 1$). For a given time horizon $T$, the arm sets at each round $t$,  $\mathcal{X}_t =\{x_{ti}\}_{i=1}^K$ is drawn independently from a distribution $\gD$ with bounded $\ell_2$ norm is bounded.

% %We assume $\norm{x_{ti}} \leq 1$ for all $i$ and $t$ almost surely. Before the game starts, the learner only knows $T$.


% At each time step of the game $t = 1, 2,\dots, T$, the learner has to first decide a policy $\pi_t$ that maps any set of context vectors $\gX$ to a distribution in $\triangle_{\gX}$. The learner then observes $\gX_t = \{x_{ti}\}_{i=1}^K$, samples an action $x_t \in \gX_t$ from $\pi_t(\gX_t)$,\footnote{When clear from the context, we interchangeably use the arm indices and their corresponding context vectors.} plays arm $x_t$, and receives the reward  $r_t \in [0,1]$, where $E[r_t|\gX_t,x_t] = \theta^Tx_t$.




% Contextual bandits have found wide applications ranging from news article recommendation \cite{newsarticlerecomcontextualbandits}, healthcare \cite{healthcarecontextualbandits} and education \cite{educationcontextualbandits}. Thus, to prevent the preferences and the arm sets (contexts) of users being inferred by an adversary, differential privacy \cite{dworkdpbook} has been used in the learning process in \cite{shariff2018differentiallyprivatecontextuallinear,pmlr-v162-chowdhury22a,pmlr-v167-garcelon22a,NEURIPS2020_908c9a56}.





%The goal of the learner is to minimize the expected regret

%In our algorithmic results, we also prove \emph{$(1-\delta)$-high probability expected regret}.

%One way to ensure shuffled differential privacy in a multi-armed bandit setup is to restrict to batched algorithms .


% Shuffled differential privacy is commonly enforced in multi-armed bandit algorithms through batching \cite{mabsshuffle,diffprivacystochasticmab,pmlr-v162-chowdhury22a}. In this approach, users are organized into batches, with each user in a batch following the same policy $\pi_t$ to select an arm. After selecting an arm $x_t$ and receiving a reward $r_t$, users send a noisy version of their data to the analyzer. At the conclusion of each batch, the analyzer shuffles the data collected from all users and aggregates it to update the model parameters, which are then used to update the policy for the next batch. Often, the batch sizes are fixed apriori since the data from the users can be analysed only at the end of a batch to ensure desired privacy guarantees. We instantiate our algorithm with increasing batch lengths as done in \cite{ruan2021linearbanditslimitedadaptivity} for linear stochastic contextual bandits. For every batch, we construct learning policies based on $G$-optimal designs that have been used in batched multi-armed bandit algorithms\cite{ruan2021linearbanditslimitedadaptivity,sawarni2024generalizedlinearbanditslimited,diffprivacystochasticmab} and we define it below.


% Since, we study make distributional stochastic assumptions on the contexts $X_t$ at each time step, we 



% %which is defined as $\sup_{A} \E\left[\ind[A] \cdot \sum_{t = 1}^T \max_{i \in [K]} x_{ti}^\top \theta - x_{t,i_t}^\top \theta\right]$ where the supremum is taken over all events $A$ such that $\Pr[A] \geq 1 - \delta$. 


% %In this definition, setting $\delta = O(1/T)$ recovers the usual expected regret up to an additive error of $O(1)$.

% In this setup, we study fixed-batched multi-armed bandit problems where the algorithm can update the policy $\pi$ only at the end of a batch. More specifically, we study a setup where the batch lengths are fixed apriori(typically increasing). Towards this, we construct learning policies based on $G$-optimal designs that have been used in batched multi-armed bandit algorithms\cite{ruan2021linearbanditslimitedadaptivity,sawarni2024generalizedlinearbanditslimited,hanna2022differentiallyprivatestochasticlinear} and we define it below.



% We now discuss our main algorithm below.

% \textbf{Notations:} Throughout the paper, we denote $[N] \defeq \{1, 2, \dots, N\}$ for any integer $N$. We define $\log x \defeq \log_2 x$ and $\ln x \defeq \log_e x$. We use $\ind[\cdot]$ to denote the indicator variable for a given event (i.e., the value of the variable is $1$ if the event happens, and $0$ otherwise). We use $\norm{\cdot}$ to denote the 2-norm of matrices and vectors. Matrix and vector variables are displayed in bold letters. For any discrete set $X$, we use $\triangle_X$ to denote the set of all probability distributions supported on $X$.

% \begin{lemma}[Lemma 3 in \cite{ruan2021linearbanditslimitedadaptivity}] For any subset $\gX \subseteq \R^d$, there exists a distribution $\gK_X$ supported on $X$, such that for any $\varepsilon > 0$, it holds that 
% \begin{align}
% \max_{x \in \gX} x^\top \left(\varepsilon \mI + \E_{y \sim \gK_\gX} y y^\top \right)^{-1} x \leq d . \label{eq:thm-KW}
% \end{align}
% Furthermore, if $X$ is a discrete set with finite cardinality, one can find a distribution such that the right-hand side of \Cref{eq:thm-KW} is relaxed to $2d$ in time  $\mathrm{poly}(\abs{X})$.
% \end{lemma}

% We now compute a distribution $\gK_X$ satisfying \Cref{eq:thm-KW} upto a factor 2 relaxation and thus, define $\pi^G(X) \defeq \gK_X$ which we shall use in our algorithm. %


\section{Differential Privacy in Multi-armed Bandits}{\label{sec:def_privacy_bandits}}
\subsection{Privacy under the Shuffle DP Model}
Here, we introduce the shuffle model, and its corresponding privacy notion called the \emph{shuffle differential privacy}. We now recall definitions of differential privacy under central and local models \cite{dworkdpbook}. Let $\mathscr{D}$ denote the data universe, and $n \in \mathbb{N}$ the number of (unique) users. Let $D_i \in \mathscr{D}, i =1,2,\ldots, n$, denote the data point of user $i$, and $D_{-i} \in \mathscr{D}^{n-1}$ denote collection of data points of all but the $i$-th user. Let $\varepsilon > 0$ and $\delta \in (0,1]$ be given privacy parameters.

\begin{definition}[Differential Privacy (DP)]
\label{def:DP}
A mechanism $\gM$ satisfies $(\varepsilon,\delta)$-DP if, for each user $i \in [n]$, each pair of datasets $D, D' \in \mathscr{D}^n$, and each event $\gE$ in the range of $\gM$,
\begin{align*}
    \prob{\gM(D_i,D_{-i}) \in \gE} \leq \exp(\varepsilon) \prob{\gM(D'_i,D_{-i}) \in \gE} + \delta.
\end{align*}
\end{definition}
\begin{definition}[Local Differential Privacy (LDP)]
\label{def:LDP}
A mechanism $\gM$ satisfies $(\varepsilon,\delta)$-LDP if for each user $i \in [n]$, each data point $D_i,D'_i \in \mathscr{D}$ and each event $\gE$ in the range of $\gM$,
 \begin{align*}
    \prob{\gM(D_i) \in \gE} \leq \exp(\varepsilon) \prob{\gM(D'_i) \in \gE} + \delta.
\end{align*}
\end{definition}
Central DP guarantees that the mechanism’s outputs on any two datasets differing by one user are nearly indistinguishable, whereas local DP enforces this indistinguishability on each user’s own randomized output. We now present shuffle privacy \cite{erlingsson2019amplification} below which bridges between the central and local model.


% will formally introduce the shuffle model for linear contextual bandits and define a new notion of privacy called \emph{shuffle differential privacy} (SDP) for it. To this end, we present a general algorithmic framework for linear contextual bandits by leveraging batched learning and the shuffle primitive. 
% As we will see, this framework not only allows us to design and analyze various learning protocols in the shuffle model, but more importantly offers the first unified view of linear contextual bandits under three trust models (i.e., JDP, LDP, SDP). 

%\subsection{Shuffle Differential Privacy}
% Our general framework builds on batched learning and the shuffle primitive, i.e., a shuffler $\kS$ that randomly permutes a collection (batch) of users' messages to provide anonymity to each of the messages. 
% We briefly introduce the well-studied one-round shuffle model over a data set of $n$ users, which will serve as a building block for our case. 
% In this setting, 
% To better introduce it, we first recall the standard one-round shuffle model . 
A (standard) shuffle protocol $\gP = (\gR, \gS, \gA)$ consists of three parts: (i) a (local) randomizer $\gR$, (ii) a shuffler $\gS$ and (iii) an analyzer $\gA$. For $n$ users, the overall protocol works as follows. Each user $i$ first applies the randomizer on its raw data $D_i$ and then sends the resulting messages $\gR(D_i)$ to the shuffler. The shuffler $\gS$ permutes messages from all the users uniformly at random and then reports the permuted messages $\gS(\gR(D_1), \ldots, \gR(D_n))$ to the analyzer. However, we consider a fully interactive shuffle protocol \cite{Cheu2021ShufflePS,lowy2024privatefederatedlearningtrusted} that allows the users to participate in the protocol multiple times. Formally, the analyzer receives the messages $\left[\gS(\gR^{(i)}(D_1), \ldots, \gR^{(i)}(D_n))\right]_{i=1}^{I}$ where the randomiser $R^{(i)}(.)$ is adaptive and could be a function (deterministic or random) of the output of the previous messages $\left[\gS(\gR^{(j)}(D_1), \ldots, \gR^{(j)}(D_n))\right]_{j=1}^{i-1}$.  


% Finally, the analyzer $\gA$ computes the output using received messages. In this protocol, the users trust the shuffler but not the analyzer. Hence, the privacy objective is to ensure that the outputs of the shuffler on two neighbouring datasets are indistinguishable in the analyzer's view. To this end, define the mechanism $(\gS \circ \gR^n)(D)\!:=\! \gS(\gR(D_1), \ldots, \gR(D_n))$, where $D \in \gD^n$.


\begin{definition}[Shuffle differential privacy (SDP)]
A (multi-rounded) protocol $\gP = (\gR, \gS, \gA)$ for $n$ users satisfies $(\varepsilon,\delta)$-SDP if the mechanism $\gS \circ \gR^n = \left[\gS(\gR^{(i)}(D_1), \ldots, \gR^{(i)}(D_n))\right]_{i=1}^{I}$ satisfies $(\varepsilon,\delta)$-DP.
\end{definition}


\subsection{Joint differential privacy (JDP) for multi armed bandits}

% \sss{Lot of repetition here check}
% Here, we discuss the differential privacy notions for the contextual multi armed bandit setup where we assume that every user is unique. 

%Towards this, we present the general differential privacy notion \cite{dworkdpbook}.

% \begin{definition}[General DP]{\label{def:general_DP}}
%     A randomised mechanism $\gM: \gD \rightarrow \gR$ satisfies $(\varepsilon,\delta)$ differential privacy if for any two adjacent datasets $X,X' \in \gD$ and any measurable subsets of output $\gY \subseteq \gR$, it holds that 
%     $$\mathbb{P}[\gM(X) \in \gY] \leq e^{\varepsilon} \mathbb{P}[\gM(X) \in \gY] + \delta$$
% \end{definition}

% Observe that all definitions of DP in the paper can be viewed as instantiations of \Cref{def:DP}. A straightforward adaptation of \Cref{def:DP} to linear contextual bandits would be to consider the set of $T$ users in the dataset $U_T := \{u_1,u_2,\ldots,u_T\}$ and the corresponding prescribed actions as the output sequence denoted as $\gM (U_T) = \{a_1,a_2,\ldots,a_T\} \in \gA^{\top}$. This is the central trust model because the learning agent in the protocol can have direct access to users’ sensitive information, but all the prescribed actions via the deployed algorithm are indistinguishable on two
% neighboring user sequences. Unfortunately, it is not hard to see that this is in conflict with the goal of
% personalization of linear contextual bandits, which essentially requires the algorithm to prescribe different
% actions to different users according to their contexts. Indeed, as shown in \cite{shariff2018differentiallyprivatecontextuallinear} any learning protocol that satisfies this notion of privacy is known to achieve a linear regret. Hence, to obtain a non-trivial regret bound, we relax the notion of differential privacy to joint differential privacy(JDP) \cite{mechanism_design_large_games,shariff2018differentiallyprivatecontextuallinear,vietri2020privatereinforcementlearningpac} in the central model which requires the joint distribution of the actions recommended to all users other than $u_t$ be differentially private in the type of user $u_t$.\footnote{The definition of JDP in \cite{mechanism_design_large_games,vietri2020privatereinforcementlearningpac} is stronger than the one in \cite{shariff2018differentiallyprivatecontextuallinear} which we will use this definition in our work.} Technically speaking, the type of the user is identified by the reward response she would give to all possible actions recommended based on her context information.

All definitions of DP in the paper can be viewed as instances of \Cref{def:DP}. 
A direct adaptation to (generalized) linear contextual bandits is to consider the $T$ users 
$U_T := \{u_1,\ldots,u_T\}$ and their prescribed actions 
$\gM (U_T) = \{a_1,\ldots,a_T\} \in \gA^{T}$. 
This corresponds to the central model, where the agent has access to users’ sensitive information, 
but the sequence of prescribed actions must remain indistinguishable on neighboring user sequences. 
However, this conflicts with the personalization goal of contextual bandits, which requires 
different actions for different user contexts. Indeed, \cite{shariff2018differentiallyprivatecontextuallinear} 
shows that any protocol satisfying this notion incurs linear regret. 
To obtain non-trivial regret bounds, we instead relax to \emph{joint differential privacy} (JDP) 
\cite{mechanism_design_large_games,shariff2018differentiallyprivatecontextuallinear,vietri2020privatereinforcementlearningpac}, 
which requires that the joint distribution of actions recommended to all users other than $u_t$ 
be differentially private in the type of $u_t$, where a user’s type is defined by her reward 
responses to all possible actions under her context.

%\footnote{The definition of JDP in \cite{mechanism_design_large_games,vietri2020privatereinforcementlearningpac} is stronger than the one in \cite{shariff2018differentiallyprivatecontextuallinear} which we will use this definition in our work. This is becuase privacy ensure with respect to all } 

\begin{definition}[Joint differential privacy (JDP)]
    A learning process of (generalized) linear contextual bandits is $(\varepsilon,\delta)$- joint differentially private (JDP) if its deployed algorithm $\gM: \gU^{\top} \rightarrow \gA^{\top}$ satisfies that for all $t \in [T]$, for all neighboring user sequences $U_T,U'_T$ differing only on the $t$-th user and for all set of actions $\gA_{-t} \subseteq \gA^{T-1}$ given to all but the $t$-th user,
    $$ \mathbb{P}[\gM_{-t}(U_T) \in \gA_{-t}] \leq e^{\varepsilon} \mathbb{P}[\gM_{-t}(U'_T) \in \gA_{-t}] + \delta $$
\end{definition}

Note that for the contextual bandit setup, each user $u_t$ in the dataset denotes a (context set $\gX_t$, reward $r_t$) tuple and each action $a_t$ denotes the arm $x_t$ that is chosen from the context set at time step $t$.




==> glm.tex <==
\section{Generalized Linear Model with Stochastic Contexts}\label{sec:glm_alg}

\paragraph{Batch lengths.}
We partition the horizon into $M \leq \log \log T$ batches 
$\mathcal{B}_1,\ldots,\mathcal{B}_M$ of lengths 
$B_1,\ldots,B_M$. Similar to 
\cite{sawarni2024generalizedlinearbanditslimited}, we define
\begin{align}
    B_1 &= \left(\frac{\sqrt{\kappa}\,e^{3S} d^2 \gamma^2}{S}\,\alpha\right)^{2/3}, 
    \qquad B_2 = \alpha, 
    \label{eq:batch_B1_B2} \\[6pt]
    B_k &= \alpha \sqrt{B_{k-1}}, \quad k \in [3,M].
    \label{eq:batch_Bk}
\end{align}

Unlike prior work, $\gamma$ is tuned to offset 
the additional shuffle-DP noise, requiring larger batches while 
minimising regret. The first batch $B_1$ serves as a 
\emph{warm-up}, and we set
\[
\alpha = T^{\frac{1}{2(1-2^{-M+1})}},
\]
ensuring the recursion \eqref{eq:batch_Bk} keeps total horizon 
within $T$ for $M \leq \log \log T$.
\paragraph{Parameters $\lambda$ and $\gamma$.}
To balance privacy noise with estimation accuracy, we set
\begin{align}{\label{eq:lambda_gamma_defn_mone}}
    \lambda &= 20dR \log T 
    + {\sigma}\!\left(6 \sqrt{\log (2dMT/\delta)}\right), \\[4pt]
    \gamma &= 30 RS \sqrt{d R\log T 
    + 12{\sigma}  \sqrt{\log (2dMT/\delta)}} 
    + \sqrt{4RS \nu}.
\end{align}
where the noise parameters $\sigma$ and $\nu$ satisfy
\begin{align}
    \sigma = O\!\left( \frac{R \,\log(d^2/\delta)}{\kappa^{*}\,\varepsilon} \right) \text{ ; }
    \nu = O\!\left( \frac{RS^2}{\varepsilon} 
    \sqrt{d \,\log^3(Td/\delta)} \right).
    \label{eq:sigma_nu_defn}
\end{align}

Unlike non-private version in \cite{sawarni2024generalizedlinearbanditslimited}, these 
choices explicitly incorporate the variance from shuffled vector 
summation and convex optimization, ensuring confidence bounds 
remain valid under differential privacy.


\paragraph{Warm-up and estimation.}
In the warm-up batch $\mathcal{B}_1$, the algorithm collects arms in order
to initialize its estimate. We form
\[
\tV \approx \sum_{t \in \mathcal{B}_1} x_t x_t^\top ,
\]
where $\tV$ denotes a noisy estimate of the empirical covariance matrix
computed using the shuffled vector summation protocol
(see \cref{sec:vector_summation_protocol}).
At the end of each batch $k$, the parameter estimate $\hat\theta_k$
is updated via a shuffled convex optimizer applied to the loss $\ell(\cdot)$.


\paragraph{Arm scaling set.}
For $k \geq 2$, arms are scaled before elimination as
\begin{align}
    \tilde{\mathcal{X}}_t 
    &:= \left\{
        \sqrt{\tfrac{\dot{\mu}(\langle x, \hat\theta_1 \rangle)}{\beta(x)}}\, x 
        : x \in \mathcal{X}_t
    \right\},
    \label{eq:arm_scaling} \\[6pt]
    \beta(x) 
    &:= \exp\!\Bigl(R \min\!\bigl(2S, \gamma \sqrt{\kappa}\,\|x\|_{\tV^{-1}}\bigr)\Bigr).
    \label{eq:beta_def}
\end{align}
A $G$-optimal design is then applied to $\tilde{\mathcal{X}}_t$. We form
\[
\tH_k \approx 
\sum_{t \in \mathcal{B}_k}
\frac{\dot{\mu}(x_t,\hat\theta_1)}{\beta(x_t)} \, x_t x_t^\top ,
\]
where $\tH_k$ denotes a noisy estimate of the corresponding weighted
design matrix, obtained using the shuffled vector summation protocol
(see \cref{sec:vector_summation_protocol}). 
Together, $\tV$ and $\{\tH_k\}_{k \ge 2}$ serve as consistently noisy
surrogates for their ideal (non-private) design matrices, ensuring
that the resulting confidence bounds remain valid under shuffle
privacy.


\paragraph{Confidence bounds.}
Upper and lower confidence bounds are defined as
\begin{align}
    \text{UCB}_k(x) &:= 
    \begin{cases}
        \langle x, \hat \theta_1 \rangle + \gamma \sqrt{\kappa}\,\|x\|_{\tV^{-1}}, & k=1, \\[4pt]
        \langle x, \hat \theta_1 \rangle + \gamma \sqrt{\kappa}\,\|x\|_{\tH_k^{-1}}, & k \ge 2,
    \end{cases} 
    \label{eq:ucb_def} \\[10pt]
    \text{LCB}_k(x) &:= 
    \begin{cases}
        \langle x, \hat \theta_1 \rangle - \gamma \sqrt{\kappa}\,\|x\|_{\tV^{-1}}, & k=1, \\[4pt]
        \langle x, \hat \theta_1 \rangle - \gamma \sqrt{\kappa}\,\|x\|_{\tH_k^{-1}}, & k \ge 2.
    \end{cases}
    \label{eq:lcb_def}
\end{align}
These follow \cite{sawarni2024generalizedlinearbanditslimited} 
but remain valid under noisy shuffled estimates.

\paragraph{Loss function.}
For GLM rewards, the negative log-likelihood
\[
\ell(\theta,r,x) := -r \langle x, \theta \rangle 
+ b(\langle x,\theta\rangle) - c(r)
\]
is convex in $\theta$ and $(R+RS)$-Lipschitz over 
$\{\theta:\|\theta\|_2 \le S\}$. The regularized empirical loss is
\begin{equation}
\gL_{\gD}(\theta) 
= \sum_{(r,x)\in\gD} \ell(\theta,r,x) 
+ \tfrac{\lambdau}{2}\,\|\theta\|_2^2,
\end{equation}
with $\lambdau$ as in \Cref{alg:shuffled_glm}.

\paragraph{Requirements.}\begin{itemize}
  \item $\tV$ and $\{\tH_k\}_{k=2}^M$ deviate from their true 
  design matrices by symmetric, zero-mean sub-Gaussian noise 
  (variance proxy $\tilde\sigma^2$).
  \item Each $\hat\theta_k$ achieves empirical loss within $\nu$ 
  of the constrained minimum.
\end{itemize}
These are satisfied by our shuffled instantiations.

\paragraph{Protocol instantiation.}
We use the shuffle convex optimizer and vector summation protocol 
of \cite{Cheu2021ShufflePS,Cheu_2019}. The optimizer runs for 
$T = \tfrac{\varepsilon^2 B_k^2}{d \log^3(B_k d/\delta)}$ steps 
with step size $\eta=2S/(RS \sqrt{T})$. The summation protocol 
privately aggregates $x_t x_t^\top$ entries via shuffled bit 
summation. These instantiations satisfy the above requirements 
and ensure JDP via the Billboard lemma 
\cite{mechanism_design_large_games}, yielding the regret bound 
stated in \Cref{sec:proof_theorem1_regret_ass}.

% We first show that our instantiations of shuffle vector protocol $\gP_{\gD}$ (\cref{sec:shuffle_convex_optimizer}) and private vector summation protocol (\cref{sec:vector_summation_protocol}) satisfy \cref{ass:sub_Gaussian_summation} and \cref{ass:sco_glm_shuffled} with $\tilde \sigma$ and $\nu$ from \cref{eq:sigma_nu_defn_mone}. Details on shuffled privacy are in \cref{sec:privacy_instantiation_utility_regret_tradeoff}. The algorithm satisfies JDP via \cite[Billboard's lemma]{mechanism_design_large_games}, and on application of \cref{theorem:main_theoremone_assumptions} we get the following informal theorem.

\begin{theorem}[Concise version of \Cref{thm:shuffled_regret_glm}]{\label{inf_thm:privacy_utility_m1}}
    For $\varepsilon<5,\delta<1/2$,  the \Cref{alg:shuffled_glm} satisfies $(\varepsilon,\delta)$ shuffle differential privacy and the expected regret 
    $R_T= \tilde{O}\left(\frac{\sqrt T}{ \sqrt{\kappa^{*}}}\left({d^{3/2}}  +\frac{d^{9/8}}{\sqrt{\varepsilon \kappa^{*}}}   \right) + \frac{d^2T^{1/3} e^{3S} \kappa^{1/3}}{(\varepsilon \kappa^{*})^{2/3}}\right) \text{poly}(R,S)$.
\end{theorem}

Observe that the dominant $\sqrt T$ term does not contain the constant $\kappa$ or exponential dependence on the bound $S$ similar to the non-private counterpart in \cite{sawarni2024generalizedlinearbanditslimited}. Further, observe that this bound differs by  at most a factor $\tilde{O}(\sqrt{d/\varepsilon})$ from its non-private counterpart in Theorem 3.2 of \cite{sawarni2024generalizedlinearbanditslimited} for sufficiently large $T$.


%Before we present a specific implementation of these protocols, we first present the following assumptions on the quantities $\tH_k$ and $\hat \theta_k$. 

\begin{algorithm}[!tb] 
    \caption{ Shuffled Differentially Private Generalized Linear Bandits Algorithm}
    \label{alg:shuffled_glm} 
    \textbf{Input:} Number of batches $M$, horizon of play $T$ and privacy parameters $\varepsilon$ and $\delta$. 

    \begin{algorithmic}[1]    
    %\vspace{-3mm}
    \State Initialize batches  $\gB_1, \ldots, \gB_M$, as defined in \Cref{eq:batch_B1_B2} and \Cref{eq:batch_Bk}. % and set \textit{batch number} $k=1$. %, and set $\lambda \coloneqq 20 R d \log{T}$.%\\ 
        %\texttt{Warmup}
    \State Set $\lambda_{\text{max}} = \lambda + \frac{8 R \log (d^2 /\delta)}{\kappa^{*} \varepsilon} (\sqrt d + 6 \sqrt{ \log (2MT/\delta)})$ and $\lambda_{\text{min}} = \lambda - \frac{8 R \log (d^2 /\delta)}{\kappa^{*} \varepsilon} (\sqrt d + 6 \sqrt{ \log (2MT/\delta)})$ \labelline{line:lambda_l_u_defn}\footnotemark
    
    
    %\algfootnote{$\lambdau$ is chosen such that $\tV_k \preceq \sum_{s \in \gB_k}\frac{\dot{\mu} (\langle x_s, \hat \theta_1\rangle)}{\beta(x_s)} x_s x^{\top}_s + \lambdau \mI \text{ if } k \geq 2$ and $\tV_1 \preceq x_s x^{\top}_s + \lambdau \mI \text{ otherwise }$. The computation of this term is done in  \cref{obs:bounds_lambda_min_lambda_max}}
        
        
        \For{local user $t \in \gB_1$} \labelline{line:warmup_start} 
        \State Observe user's arm set $\gX_t$, sample arm $x_t \sim \pi_G(\gX_t)$, %\quad  \texttt{// G-optimal design}
        and observe reward $r_t$. % and update $\bV \leftarrow \bV + x_t x_t^\T$.
        

        \textcolor{gray}{\# For the local randomizer:}

        \State Compute randomized messages $M_{t,2} = R_2\left(x_tx^{\top}_t, \Delta = 1\right)$ with privacy parameters $\varepsilon/2$ and $\delta/2$ and number of users $n = B_k$.

        
        
        %$Y_{t,1} = (r^{(n)}_t, x^{(n)}_t) = R_1(r_t,x_t)$
        
        \EndFor \labelline{line:warmup_end}

        \textcolor{gray}{ \# For the shuffler: }

        % Sample a uniform permutation $\rho$ over $\gB_1$ and then apply it to the received messages.

        \State Permute all received messages $Y_{k,2} = S_2 (\{M_{\tau,2}\}_{\tau \in \mathcal{B}_k})$ and compute batch statistics ${\tV} = A_2(Y_{k,2}) + \lambda \mI$.  

        % Compute $\hat\theta_w = \argmin_\theta \sum_{s \in \mathcal{B}_k } \ell\left(\theta, x^{(n)}_{\rho(s)}, r^{(n)}_{\rho(s)}\right)$ and 
        % Compute $\hat \theta_w = \mathcal{P}$
        
        \textcolor{gray}{ \# For the shuffle convex optimizer}


        \State Apply shuffle convex optimizer $\mathcal{P}_{\text{GD}}$ on data-points $\{r_t,x_t\}_{t \in \mathcal{B}_k}$ with loss function $\ell(.) + \frac{\lambdau}{2B_k} \left|\left|\theta\right|\right|^2_2$ under privacy parameters $\varepsilon/2$ and $\delta/2$ to obtain $\hat \theta_k$.

        %with number of iterations $T= \frac{\varepsilon_o^2(t-1-|\gT_o|)^2}{d\log^3(d/\delta_0)}$ and parameter $\eta = \frac{2S}{L\sqrt{T}}$
        
        \For{batches $k =2$ to $M$}
        %\State Initialize $\bH_k \leftarrow \lambda \bI $.
        \For{each local user $t \in \gB_k$}
            \State Each user observes arm set $\gX_t$.
            \For{$j = 1$ to $k-1$}  
                \State Update arm set $\gX_t \leftarrow \gX_t \setminus \{ x \in \gX_t: {\text{UCB}_j} (x) < \max_{y \in \gX_t} \text{LCB}_j (y) \}$. 
            \labelline{line:elimination_glm_stochastic}
            \EndFor
            \State Scale $\gX_t$, as in \Cref{eq:arm_scaling}, to obtain $\tilde{\gX}_t$.\labelline{line:modified_arms}, then
             sample $x_t \sim \pi^G\left(\tilde{\gX_t} \right)$.  \labelline{line:g_opt_sampling_glm} 

             \textcolor{gray}{\# For the local randomizer:}

         \State Send messages $M_{t,2} = R_2\left(\frac{\dot{\mu}(\langle x_t, \hat \theta_1 \rangle)}{\beta(x_t)} x_tx^{\top}_t, \Delta = \frac{1}{\kappa^{*}}\right)$ with privacy parameters $\varepsilon/2, \delta/2 - \frac{1}{T^2}$ and number of users $n=B_k$. \footnotemark

%Send  messages $(r_t,x_t)$ to SCO (Algorithm )
       
        \EndFor

        \textcolor{gray}{ \# For the shuffler: }

        \State Permute all received messages $Y_{k,2} = S_2 (\{M_{\tau,2}\}_{\tau \in \mathcal{B}_k})$ and compute batch statistics ${\tH}_k = A_2(Y_{k,2}) + \lambda \mI$.  


        \textcolor{gray}{ \# For the shuffle convex optimizer: }

        \State Apply shuffle convex optimizer $\mathcal{P}_{\text{GD}}$ on data-points $\{r_t,x_t\}_{t \in \mathcal{B}_k}$ with loss function $\ell(.) + \frac{\lambdau}{2B_k} || \theta||^2_2 $ to obtain $\hat \theta_k$ under privacy parameters $\varepsilon/2$ and $\delta/2$. 
        \labelline{line:batch_end}  

        %Set the number of iterations $T = \frac{\varepsilon^2n^2}{d \log^3(nd/\delta)}$ with parameter $\eta = \frac{2S}{L\sqrt{T}}$
        \EndFor
    \end{algorithmic}
   \end{algorithm}

\addtocounter{footnote}{-1} % Go back two footnotes
\footnotetext{ We choose $\lambdau$ such that $\tV_k \preceq \sum_{s \in \gB_k}\frac{\dot{\mu} (\langle x_s, \hat \theta_1\rangle)}{\beta(x_s)} x_s x^{\top}_s + \lambdau \mI \text{ if } k \geq 2$ and $\tV_1 \preceq \sum_{s \in \gB_1}x_s x^{\top}_s + \lambdau \mI \text{ otherwise }$. We compute this term in  \Cref{obs:bounds_lambda_min_lambda_max}.}

\stepcounter{footnote}
\footnotetext{Observe that $\frac{\dot{\mu}(\langle x_t, \hat \theta_1 \rangle)}{\beta(x_t)} \leq \dot{\mu} (\langle x_t, \theta^{*} \rangle) \leq \frac{1}{\kappa^{*}}$ from \Cref{lemma:H_bound_H_star} with probability at least $1- \frac{1}{T^2}$. Therefore we set the bound $\Delta$ to $\frac{1}{\kappa^{*}}$.}


%\cref{alg:shuffled_glm}
%Define $\tH_k = \lambda \mI + \sum_{t \in \gB_k} \left(\dot{\mu} \left(\langle x^{(n)}_{\rho(t)}, \hat\theta_w\rangle\right)/ \beta(x^{(n)}_{\rho(t)})\right) x^{(n)}_{\rho(t)} (x^{(n)}_{\rho(t)})^{\top} + \lambda \mI$,
        
        
        
        %

        %Now define $\tH_k := \lambda \mI + \tilde{\tH}_k$
        
        
        %\State Compute \textsc{Distributional optimal design} policy $\pi_{k} $ using the arm sets $\{ \cX_t \}_{t \in \mathcal{B}}$. 







%\sss{Invoke lemma B.4 with $T=n^2$ and $\eta = \frac{1}{n}$.}





% \begin{lemma}
%     With probability at least $1- \frac{\delta}{2T^2}$, we have $$\tH_k = \hat \lambda_k \mI + \sum_{t \in \mathcal{B}_k} \frac{\dot{\mu} (\hat\theta_w, x_t)}{\beta(x_t)} x_t x^{\top}_t \text { for $k \in [2,M]$ and } \tV = \hat \lambda_1 \mI + \sum_{t \in \mathcal{B}_1} x_t x^{\top}_t \text{ where,}$$ 

%     $$ 0 \leq \hat{\lambda}_k - 16R \log \left(2dT /\delta \right) \leq  4\sqrt{\frac{32}{\varepsilon} \log \left(\frac{2.5B_k}{\delta}\right) \log \left(2/\delta\right)} \left(\sqrt{d}+ 6 \sqrt{\log \left(\frac{2dKT}{\delta}\right)}\right)  \Forall k \in [M]$$
    
% \end{lemma}


% \begin{proof}
%     First, observe that $\mLambda_{k} = \lambda \mI+ \sum_{t \in \gB_k} x_t x^T_t + \gN_{k}$. Observe that $\gN_{k}$ is  upper diagonal elements being independent Gaussian elements with variance $\sigma^2_3B_{\kappa} = \frac{32}{\kappa^{*}\varepsilon} \log \left(\frac{2.5B_{\kappa}}{\delta}\right) \log \left(2/\delta\right)$. Thus using \cite[Corollary 4.4.8]{vershynin_high-dimensional_2018}, $$\prob{||\gN_{\kappa}|| >4 \sqrt{\frac{32}{\varepsilon} \log \left(\frac{2.5B_{\kappa}}{\delta}\right) \log \left(2/\delta\right)} (\sqrt{d}+ \gamma)} \leq 1/2 \exp(-\gamma^2)$$. 

%     Setting $\gamma = 6 \sqrt{\log \left(2dT/ \delta\right)}$ we get the desired result. A very similar technique can be used to bound $\tV$ as well.
    
% \end{proof}




%First, observe that $\mLambda_{\kappa} = \lambda \mI+ \sum_{t = \gT_{k-1}+1}^{\gT_{k}} x_t x^T_t + \gN_{\kappa}$. Observe that $\gN_{\kappa}$ is a symmetric matrix with upper diagonal elements being independent Gaussian elements with variance $\sigma^2_2B_{\kappa} = \frac{32}{\varepsilon} \log \left(\frac{2.5B_{\kappa}}{\delta}\right) \log \left(2/\delta\right)$. Thus using \cite[Corollary 4.4.8]{vershynin_high-dimensional_2018}, $$\prob{||\gN_{\kappa}|| >4 \sqrt{\frac{32}{\varepsilon} \log \left(\frac{2.5B_{\kappa}}{\delta}\right) \log \left(2/\delta\right)} (\sqrt{d}+ \gamma)} \leq 1/2 \exp(-\gamma^2)$$. 


    % Thus, $\mLambda_{\kappa} = \tilde{\lambda} + \sum_{t = \gT_{k-1}+1}^{\gT_{k}} x_t x^T_t$ with probability at least $1- \exp(-\gamma^2)$ where 
    % $$16 \log (2dT/ \delta) \leq \tilde{\lambda} \leq 16 \log (2dT/ \delta) + c_1 \sqrt{\frac{32}{\varepsilon} \log \left(\frac{2.5B_k}{\delta}\right) \log \left(2/\delta\right)} \left(\sqrt{d}+ 6 \sqrt{\log \left(\frac{2dKT}{\delta}\right)}\right)$$
    
    
    
    
    
    % Choosing $\gamma = 6 \sqrt{\log \left(\frac{2dKT}{\delta}\right)}$ and applying \cref{lem:analysis-lr} and union bound over all stages and candidate arms to prove the lemma.



% Define $$(\tH^{(n)}_k)^{*} = \sum_{t \in \mathcal{B}_k} \dot{\mu} \left(\langle x^{(n)}_t, \theta^{*}\rangle\right)x^{(n)}_t (x^{(n)}_t)^{\top} + \lambda \mI \text{ for $k \in [2,M]$}$$ 

% and we similarly define 

% \begin{equation}
%     \tV = \sum_{t \in \mathcal{B}_1} \dot{\mu}\left(\langle x_t, \theta \rangle\right) \text { and } \tH_k = \sum_{t \in \mathcal{B}_k} \dot{\mu}\left(\langle x_t, \theta \rangle\right)
% \end{equation}

% \begin{lemma}
%     $\tH^{*}_k $
% \end{lemma}


%\subsection{Regret Guarantee under Assumptions \protect\ref{ass:sub_Gaussian_summation} and \protect\ref{ass:sco_glm_shuffled} }


\newcommand{\maintheoremoneregretassumptions}{
    If \Cref{ass:sub_Gaussian_summation} and \Cref{ass:sco_glm_shuffled} hold true, and $\lambdal \geq 20dR \log T$, the expected regret $R_T$ can be bounded as follows where $M$ denotes the number of rounds
    \begin{align}
    R_T & = O\Biggl(  \left( \sqrt{\kappa} d^2 e^{3S} RS T^{\frac{1}{2\left(1-2^{-M}\right)} } \left(d R\log T + 12\tilde{\sigma}  \sqrt{\log (2dMT/\delta)} + \sqrt{4RS\nu}\right) \right)^{2/3} \nonumber\\
    & \hspace{ 10 em} + \frac{d}{\sqrt {\kappa^{*}}} RS T^{ 
 \frac{1}{2\left(1-2^{-M}\right)}} \sqrt{d R\log T + 12\tilde{\sigma}  \sqrt{\log (2dMT/\delta)} + \sqrt{4RS\nu}}\Biggr) M\nonumber
\end{align}

}

%\sss{maybe theorem statement requires a bound on $\lambdal$ just check once.}

%\sss{To revisit later}








% \begin{lemma}{\label{lemma:bounding_expected_score}}
% \lemmaboundingexp
% \end{lemma}










==> glm_adversarial_context.tex <==
\section{Generalized Linear Model with Adversarial Contexts}{\label{sec:glm_jdp}}

\begin{algorithm}[!tb] 
    \caption{Joint Differentially Private generalized Linear Bandits}
    \label{alg:jdp_glm_adversarial} 
    \textbf{Initialize:} $\lambda, \gamma,\beta$ (from Equations \ref{eq:beta_gamma_defn_glm_adv} and \ref{eq:lambda_defn_glm_adv}) and $\tV,\tH_1 \gets \lambda \mI$,  $\text{count1},\text{count2} \gets 0$ and $\gT_o \gets \emptyset$
    
    \begin{algorithmic}[1]
    \State Set $\lambdal \gets \lambda \frac{4 \sqrt d}{4\sqrt d+1}$ and $\lambdau \gets \lambda \frac{4 \sqrt d +2}{4 \sqrt d+ 1}$
    %\State Set $\lambdal \gets \lambda  - \frac{64 \log(32/\delta)\log T \left(\log(16 T/\zeta) + \sqrt{d} \right)}{\varepsilon (\kappa^{*})}$ and set $\lambdau \gets \lambda + \frac{64 \log(32/\delta) \log T\left(\log(16 T/\zeta)+ \sqrt{d}\right)}{\varepsilon (\kappa^{*})}$
    
    %\State Set $\lambdal \gets \lambda^{(2)} - \frac{64 \log(32/\delta) \left(\log(16 T/\zeta)\right)^2}{\varepsilon (\kappa^{*})}$ and set $\lambdau \gets \lambda^{(2)} + \frac{64 \log(32/\delta) \left(\log(16 T/\zeta)\right)^2}{\varepsilon (\kappa^{*})}$
    
    \State Set $\ccut \gets 8dR^2 \kappa \gamma^2 \log T$ and $\ccuttwo \gets \log_2 \left(\dfrac{\lambdau}{\lambdal} + \dfrac{T/(\kappa^{*})^2}{\lambdal d}\right)$
    % \State Set $\ccuttwo \gets \log_2 \left(\dfrac{\lambdau}{\lambdal} + \dfrac{T/(\kappa^{*})^2}{\lambdal d}\right)$ and noise value $\hat{n}_{0} \gets \text{Lap}(\sigma_q)$
    
    \For{$t \gets 1$ \textbf{to} $T$}
        
        \State Observe arm set $\gX_t$.

        % \If{$\text{count1} \geq \ccut$ or $\text{count2} \geq \ccuttwo$}\label{line:var_count1_exceed_threshold}

        %     \State Play an arm $x_t \in \gX_t$ uniformly at random. % and set
            

        %     \State \textbf{Continue}
            
        % \EndIf


        

        %$\gamma^2 \kappa R^2\max\limits_{x \in \gX_t} ||x||^2_{\tV^{-1}} + \text{Lap}\left(2\sigma \right) \geq (1+ \hat n_{\text{count1}})$
        
        %\If{$\lambdal \max\limits_{x \in \gX_t} ||x||^2_{\tV^{-1}} + \text{Lap}(2\sigma_q) \geq \hat n_{\text{count1}} + \frac{\lambdal}{\gamma^2 \kappa R^2}$} 
        
        
        \If{$\max\limits_{x \in \gX_t} ||x||^2_{\tV^{-1}} \geq \frac{1}{\gamma^2 \kappa R^2}$}\Comment{Policy I switches }\labelline{line:policy_I_switch}
        %\Comment{Private Policy I switches using DP sparse vector technique}
        
        
        
        \State Play arm $x_t = \argmax_{x \in \gX_t} ||x||_{\tV^{-1}}$ and observe reward $r_t$. \labelline{line:max_arm_selected_V_norm}
        \State Update $\gT_o \leftarrow \gT_o \cup \{t\}$, $\tV \leftarrow \tV + x_t x^{\top}_t + \mathcal{R}_t, \tH_{t+1} \leftarrow \tH_t + \gR_t$ \labelline{line:noise_addition_R_t_step_I}
        \Comment{Regualizer $\gR_t$ is added for privacy and described in \Cref{sec:privacy_analysis_regret_glm_adversarial}}
        \State Set  parameter $\varepsilon_0 = \frac{\varepsilon}{6\sqrt {2 \ccut \log (4/\delta)}}$ and $\delta_0 = \frac{\delta}{6\ccut}$
 \footnotemark{}


        \State  Compute $\hat \theta_o$ by applying shuffle convex optimizer $\mathcal{P}_{\text{GD}}$ on $\{r_t,x_t\}_{t \in \gT_o}$ with loss function $\ell(.)+ \frac{\lambdau}{2|\gT_o|} ||\theta||^2_2$ under convex set $\Theta := \{\theta: ||\theta||_2 \leq S\}$ with privacy parameters $\varepsilon_o$ and $\delta_o$ and increment $\text{count1}$. \labelline{line:theta_o_defn}
        
        %$ \leftarrow \text{count1}+1$.
        %\quad  \texttt{// G-optimal design}

        
       

        

        \Else

            \If{$ \max\limits_{s \leq t}\text{det}(\tH_s) > 2 \max\limits_{s \leq \tau}\text{det}(\tH_{s})$} \Comment{Policy II switches}\labelline{line:policy_II_switch}
            
            %\tcp*[r]{Policy II switches}}
            

             \State  Set $(\varepsilon_0,\delta_0) := \left(\frac{\varepsilon}{6\sqrt {2 \ccuttwo \log (4/\delta)}},\frac{\delta}{6 \ccuttwo}\right)$. \labelline{line:epsilon_0_delta_0_optimizer}

            \State Set $\tau =t$ and compute $\hat \theta_{\tau}$ via shuffle optimizer $\mathcal{P}_{\text{GD}}$ on $\{r_t,x_t\}_{[t-1]\setminus \gT_o}$ with loss function $\ell(.)+ \frac{\lambdau}{2(t-1-|\gT_o|)} ||\theta||^2_2$  under convex set $\Theta := \{\theta: ||\theta - \hat \theta_o||_{\tV} \leq \gamma \sqrt{\kappa}\}$ with privacy parameters $\varepsilon_0$ and $\delta_0$ and increment $\text{count2}$. % \gets \text{count2} + 1$.
                %\textbf{with number of iterations $T= \frac{\varepsilon_o^2(t-1-|\gT_o|)^2}{d\log^3(d/\delta_0)}$ and parameter $\eta = \frac{2S}{L\sqrt{T}}$}
            

            \EndIf
            
            \State Update $\gX_t \leftarrow \gX_t \setminus \{x: \gX_t: \text{UCB}_o(x) < \max_{z \in \gX_t} \text{LCB}_o(z)\}$ \labelline{line:elimination_glm_adversarial}

            \State Play arm $x_t = \argmax_{x \in \gX_t} \text{UCB}(x,\tH_\tau, \hat \theta_\tau)$ and observe reward $r_t$. \labelline{line:arm_selected_regular}

            \State Update $\tH_{t+1} \leftarrow \tH_t + \frac{\dot{\mu} \left(\langle x_t, \hat \theta_o\rangle\right)}{e} x_t x^{\top}_t + \gR_t$ and $\tV \leftarrow \tV+ \gR_t$ \Comment{Regularizer $\gR_t$ is added for privacy and described in \Cref{sec:privacy_analysis_regret_glm_adversarial}}
            \labelline{line:noise_addition_R_t_step_II}

        \EndIf

    \EndFor
    \end{algorithmic}
    
   \end{algorithm}
   \footnotetext{We choose the parameters $(\varepsilon_0,\delta_0)$ such that the privacy loss is at most $(\frac{\varepsilon}{3},\frac{\delta}{3})$ after $\ccut$ compositions.}


We propose a joint differentially private algorithm for generalized 
linear bandits with adversarial contexts (\Cref{alg:jdp_glm_adversarial}). 
Our design adapts the switching-criterion framework of 
\cite{sawarni2024generalizedlinearbanditslimited}, but introduces 
new ingredients to ensure privacy while retaining low regret.

At each round $t$, the algorithm first checks \emph{switching criterion~I},
namely whether there exists an arm $x \in \gX_t$ whose norm exceeds a
$\kappa$-dependent threshold. If the criterion is triggered, the algorithm
selects the arm maximizing $\|x\|_{\tV^{-1}}$, adds round $t$ to $\gT_o$,
and updates the unscaled design matrix
\[
\tV \approx \sum_{s \in \gT_o} x_s x_s^\top .
\]
Here, $\tV$ denotes a noisy estimate maintained using the binary tree
mechanism \cite{continualstatsrelease,continualobservation}.
We denote by $\hat\theta_o$ the estimate of the true parameter $\theta^*$
obtained by running the private optimizer on the data points indexed by
$\gT_o$ (see \cref{line:theta_o_defn}).


For rounds $t \notin \gT_o$, the algorithm instead maintains a scaled
design matrix
\[
\tH_t \approx 
\sum_{s \notin \gT_o}
\frac{\dot{\mu}(\langle x_s, \hat\theta_o \rangle)}{e} \,
x_s x_s^\top ,
\]
where $\tH_t$ is a noisy estimate updated via the same binary tree
mechanism \cite{continualstatsrelease,continualobservation}.
A detailed privacy analysis of the updates to $\tV$ and $\tH_t$, and
their impact on the regret guarantees, is provided in
\cref{sec:privacy_analysis_regret_glm_adversarial}.

If criterion I is not met, the algorithm checks \emph{switching criterion II}: 
whether the maximum determinant among the released scaled design matrices 
$\{\tH_s\}_{s \leq t}$ has doubled relative to its value at the last trigger 
round $\tau$. Unlike the non-private setting, these design matrices are 
maintained via a binary tree mechanism 
\cite{continualstatsrelease,continualobservation} with an added symmetric 
regularizer $\gR_t$ instantiated through Gaussian noise 
(see \Cref{sec:jdp_instantiation_utility_regret_tradeoff}). Since the 
noise may cause $\{\tH_s\}$ to be non-monotone, we compare against the 
\emph{running maximum determinant} rather than the raw determinant at 
round $t$. This modification ensures that criterion II remains meaningful 
while preserving the privacy guarantees for $\tH_t$ and $\tV$.

Overall, while our algorithm retains the high-level structure of 
\cite{sawarni2024generalizedlinearbanditslimited}, two modifications 
are necessary. First, to release $\tV$ and $\{\tH_s\}_{s=1}^t$ privately, 
we employ the binary tree mechanism augmented with Gaussian regularizers 
$\gR_t$, ensuring valid confidence sets even under continual observation. 
Second—and more critically—we must protect the index sets $\gT_o$ and 
$[T]\setminus \gT_o$ on which these matrices are computed. Because the 
action at round $t$ is a deterministic function of $\gX_t$, these indices 
are not private a priori. Our main contribution is to show that 
$\gT_o \setminus \{t\}$ remains $(\varepsilon,\delta)$-indistinguishable 
for any two datasets differing at time-step $t$. This guarantee follows 
from an advanced composition analysis of log-likelihood ratios 
\cite{kairouz2015compositiontheoremdifferentialprivacy,fullyadaptiveprivacy}, 
applied to the binary tree construction by tracking the sequence of 
updated leaf nodes. Combining this analysis with the privacy guarantees 
of the binary tree mechanism establishes the required privacy bounds 
for $\{\tH_s\}, \tV, \theta_o$ and $\theta_{\tau}$.
% While at a high level our algorithm retains this structure, we need to incorporate two major changes. a) The running set of indices $\{\gT_o\}$ should be $(\varepsilon,\delta)$ differentially private and b) The running design matrix $\tV$ and $\{\tH_s\}_{s=1}^{t}$ should also be $(\varepsilon,\delta)$ DP w.r.t the data points $\{r_t,\gX_t\}_{t \in \gT_o}$ and $\{r_t,\gX_t\}_{t \in [t-1]\setminus \gT_o}$. The former condition a) requires a novel adaptation of the sparse vector technique \cite{dworkdpbook} in differential privacy as one could potentially view the evaluation of criterion as adaptive queries $\{f_i\}_{i=1}^{k}$ to the database. However, to get good accuracy as shown in \cite[Theorem 3.26]{dworkdpbook}, we need a bound on the number of times it is true which follows from a variant of \cite[Lemma B.11]{sawarni2024generalizedlinearbanditslimited}. The later condition b) uses a binary tree mechanism \cite{continualstatsrelease,continualobservation} to estimate the design matrices $\tV$ and $\{\tH_s\}_{s=1}^{t}$ which involves the addition of a symmetric regularizer $\gR_t$ at each step that may be instantiated using addtive Gaussian noise. A similar approach has been taken in \cite{shariff2018differentiallyprivatecontextuallinear} for the case of linear contextual bandits with adversarial contexts.

%{\color{red} Highlight the technical novelty in privacy analysis.}

%A similar approach has been taken in \cite{shariff2018differentiallyprivatecontextuallinear} for the case of linear contextual bandits with adversarial contexts.

% While our algorithm broadly retains the structure in \cite{sawarni2024generalizedlinearbanditslimited}, two key modifications are required. 
% First, to obtain accurate yet private estimates of the design matrices, we employ a binary tree mechanism 
% \cite{continualstatsrelease,continualobservation} to release $\tV$ and $\{\tH_s\}_{s=1}^t$, 
% augmented with a symmetric regularizer $\gR_t$ instantiated via additive Gaussian noise 
% (see \Cref{sec:privacy_analysis_alg_glm_shuffled} for details). Further, since the noisy design matrices may not be monotonic post noise addition, we require the adapt the switching criterion to consider the largest value of determinant of all design matrices so far in step II.

% Second—and more critically in our setting—beyond ensuring private release of the design matrices, 
% we must also protect the index sets $\gT_o$ and $[T]\setminus \gT_o$ on which they are computed. 
% Since the action at round $t$ is a deterministic function of the context set $\gX_t$, 
% these indices are not private by default. 
% Our main contribution here is to show that 
% $\gT_o \setminus \{t\}$ remains $(\varepsilon,\delta)$-indistinguishable 
% for any two datasets differing in the context or reward at time-step $t$. 
% This result follows from an advanced composition analysis of log-likelihood ratios 
% \cite{kairouz2015compositiontheoremdifferentialprivacy,fullyadaptiveprivacy}, 
% applied to the binary tree construction by tracking the sequence of updated leaf nodes. 
% Combining this with the differential privacy guarantees of the binary tree mechanism 
% establishes the desired privacy bounds for $\tH_t$ and $\tV$.


%\sss{check if peeling is a valid word.}

%Since policy I update is clearly non-private, we need to alternately argue that $\gT_o \setminus \{t\}$ is $(\varepsilon,\delta)$ indistinguishable for any two datasets over arms and rewards differing at index $t$.


We now formally define $\text{UCB}_o$ and $\text{LCB}_o$, which are used in arm elimination, and $\text{UCB}(x,\tH, {\theta})$, which is used in arm selection.  
We also define the parameters $\gamma$, $\lambda$, and $\beta$ that appear in the algorithm.
\begin{align}
    \text{UCB}_o(x) 
    &= \langle x, \hat \theta_o \rangle 
       + \gamma \sqrt{\kappa}\,\|x\|_{\tV^{-1}}, 
    \label{eq:ucb_o} \\[6pt]
    \text{LCB}_o(x) 
    &= \langle x, \hat \theta_o \rangle 
       - \gamma \sqrt{\kappa}\,\|x\|_{\tV^{-1}}, 
    \label{eq:lcb_o} \\[6pt]
    \text{UCB}(x, \tH,  \theta) 
    &= \langle x, \theta\rangle 
       + \beta \,\|x\|_{\tH^{-1}}.
    \label{eq:ucb_general}
\end{align}

\begin{align}
& \hspace{-2 em}\lambda := \frac{64(4 \sqrt d+1) {\log(32/\delta) \log T} \left(\log (16 T/\zeta) + \sqrt{d}\right)}{\varepsilon \kappa^{*}}\label{eq:lambda_defn_glm_adv}\\
    \beta & = \frac{CRS d^{0.5} \log (T/\zeta) \log (1/\delta)}{\sqrt{\varepsilon \kappa^{*}}} \\ \text{ and } \gamma & = \frac{cR^{5} S^{4} d \log^2 (Td/\zeta) \log (32/\delta)}{\min(\varepsilon,1) (\kappa^{*})^2 } \label{eq:beta_gamma_defn_glm_adv}
\end{align}



% Set $\lambda^{(1)} := \frac{64 \sqrt {\log(32/\delta)} \left( \log (16 T/\zeta)\right)^2}{\varepsilon \kappa^{*}} + \frac{100 \gamma^3 \kappa^{1.5} R^3}{\varepsilon} \log\left(32T/\zeta\right) \sqrt{\log (8/\delta) \log T}$

% Set $\lambda^{(2)} := \frac{64 \sqrt {\log(32/\delta)} \left( \log (16 T/\zeta)\right)^2}{\varepsilon \kappa^{*}}+ \frac{10d\log(16T/\zeta)}{R^2}$


A central part of our regret and privacy analysis is to show that the matrices $\tV$ and $\tH_k$ approximate the true design matrices up to a small error that decays with $\varepsilon$ and grows logarithmically in $T$. Likewise, the estimator $\hat \theta_\tau$ minimizes the empirical loss up to an error with the same $\varepsilon$– and $\log T$–dependence. The privacy guarantees and the fact that the algorithm satisfies the required assumptions are established in \Cref{sec:privacy_analysis_regret_glm_adversarial}. Under these assumptions, \Cref{sec:glm_jdp_regret_analysis_assumption} shows that our algorithm achieves the desired regret guarantees.

    % Before we present the regret and private analysis of this algorithm, we first present the the two assumptions that matrices $\tV$ and $\tH_k$ estimate the true design matrices upto a small error and the estimator $\hat \theta_\tau$ minimises empirical loss upto a small error with a detailed description in \Cref{sec:jdp_instantiation_utility_regret_tradeoff}. We prove a regret bound under this assumption and then show that both our private algorithms satisfy this assumption and in turn leads to a bound on the regret. The privacy guarantee and the algorithm satisfying the desired assumptions is proven in \Cref{sec:privacy_analysis_regret_glm_adversarial}. In \Cref{sec:regret_analysis_alg_glm_shuffled}, we show that our algorithm satisfies the desired regret guarantees under these assumptions.

    %\sss{To satisfy the utility bound from sparse vector technique maybe we need an extra log T into $\lambda$ term} %to satisfy \cref{ass:indices_selected}}

    % {\color{blue} Describe the innovation in obtaining the privacy guarantee.}

    % Further, we define the regularized loss functions where $\gS = \{r_t,x_t\}_{t\in \gT}$.
    % \begin{align}
    %     \gL^{(1)}_{\gT}(\theta) = \sum_{t\in \gT} \ell(\theta, r_t,x_t) + \frac{\lambdau}{2} ||\theta ||^2 \text{ and }
    %     \gL^{(2)}_{\gT}(\theta) = \sum_{t\in \gT} \ell(\theta, r_t,x_t) + \frac{\lambdau}{2} ||\theta ||^2
    % \end{align}


        %$$$$


    
    % \sss{Describe the innovations in privacy analysis and check text above written above something to revisit later.}


    % \sss{$\nu_1$ and $\nu_2$ chosen as the former would be $\kappa$ dependent but the latter won't be thus the regret is still $\kappa$ independent in dominant term.}


    

    % In \cref{alg:jdp_glm_adversarial}, policy I’s switches are non-private because they directly use the context set $\gX_t$ at time $t$. Nonetheless, for any adjacent datasets $\gD,\gD'$ differing only at round $t$, the transcript excluding that switch—i.e.\ $\gT_o!\setminus!{t}$—remains $(\varepsilon,\delta)$-indistinguishable. The proof applies the advanced‐composition theorem to log-likelihood ratios, following the peeling argument on the binary tree from \cite{kairouz2015compositiontheoremdifferentialprivacy,fullyadaptiveprivacy}, and then invokes the binary-tree mechanism’s privacy guarantee to show that the design matrices ${\tilde V_t}$ are also private. The full privacy proof and resulting regret bounds appear in \cref{sec:privacy_analysis_regret_glm_adversarial}.


    

    %\sss{check whether peeling is appropriate.}
    % In \cref{sec:privacy_analysis_regret_glm_adversarial}, we prove the $(\varepsilon,\delta)$ joint differential privacy guarantees and show that the above assumptions are satisfied. Now applying \cref{theorem:glm_joint_dp_regret_assumptions}, we can prove the desired regret and privacy bound. One may observe that 


    \begin{theorem}[Concise version of \Cref{thm:jdp_regret_glm}]
        \Cref{alg:jdp_glm_adversarial} satisfies $(\varepsilon,\delta)$ joint differential privacy and with probability at least $1-\zeta$ (for $\delta > \zeta$) we have $R^T = \tilde{O}\left( \sqrt{{T}} \left(\frac{d}{\sqrt \kappa^{*}} + \frac{d^{3/4}}{\kappa^{*} \sqrt{\varepsilon}}\right) \right) \text{poly}(R,S)$.
    \end{theorem}

In the non-private setting, adversarial contextual bandits achieve regret 
$\tilde{O}\!\left(d\sqrt{T/\kappa^{*}}\right)\,\text{poly}(R,S)$~\cite{sawarni2024generalizedlinearbanditslimited}, 
optimal up to poly-logarithmic factors in $T$ (cf. \cref{eq:kapa_mtwo}). 
Our private bound matches this up to an additional $\tilde{O}(1/\sqrt{\varepsilon})$ factor.


\begin{remark}[Computational Efficiency]
    The amortized per-step complexity is $O(\log \log T)$ and $O(\log ^2 T)$ for algorithms in settings $\mone$ and $\mtwo$ respectively.
\end{remark}



% \section{}
    
    

%    \section{Regret bounds of Algorithm \ref{alg:jdp_glm_adversarial} under  assumptions \ref{ass:regularizer_noise} and \ref{ass:sco_loss}}{\label{sec:glm_jdp_regret_bounds_assumption}}

    %\sss{Check how $\zeta$ is related to $\delta$ like $\delta< \zeta$ for boundedness to add laplace noise in differential privacy}

    
    
    % \begin{theorem}{\label{theorem:glm_joint_dp_regret_assumptions}}
    %     \maintheoremjointprivacyassumptions
        
    % \end{theorem}

    

==> glm_old.tex <==
\section{Generalized linear model}

\begin{definition}{\label{def:glm}}
    A generalized linear model (GLM) with parameter vector $\theta^{*} \in \mathbb{R}^d$ is a real valued random variable $r$ that belongs to the exponential family of distribution with density function
    $$P(r_t | x_t) = \exp(r.\langle x,\theta^{*}\rangle - b\left(\langle x,\theta^{*}\rangle\right) + c(r)) $$

    Funtion $b(.)$ (called the log-partition function) is assumed to be twice differentiable and $\dot{b}$ is assumed to be monotone. Further, we assume $r \in [0,R]$ and $\theta^{*} \in [0,S]$. 
\end{definition}

Important properties of GLM such as $\mathbb{E}[r] = \dot{b}\left(\langle x,\theta^{*}\rangle\right)$ and $\text{Var}(r) = \ddot{b}\left(\langle x,\theta^{*}\rangle\right)$. Further, we define $\mu\left(\langle x,\theta^{*}\rangle\right) = \dot{b}\left(\langle x,\theta^{*}\rangle\right)$ as the link function.

We now state a lemma from \cite[Lemma 2.2]{sawarni2024generalizedlinearbanditslimited}. An analysis of GLMs and a computation of its mean/variance is presented in \cite[Appendix C]{sawarni2024generalizedlinearbanditslimited}.

\begin{lemma}[Self concordance of GLMs \cite{sawarni2024generalizedlinearbanditslimited}]
    For any GLM supported on $[0,R]$ almost surely, the link function $\mu(.)$ satisfies $||\ddot{\mu}(z)|| \leq R\dot{\mu}(z)$ for all $z \in \mathbb{R}$.
\end{lemma}

We also use the following multiplicative bound on the $\dot{\mu}$ from \cite[Appendix C]{sawarni2024generalizedlinearbanditslimited}.

\begin{lemma}[Multiplicative bound on $\dot{\mu}$ \cite{sawarni2024generalizedlinearbanditslimited}]
    For any $z_1,z_2 \in \mathbb{R}$, we have $\frac{\dot{\mu}(z_2)}{\exp(R|z_1-z_2|)} \leq \dot{\mu}(z_1) \leq \dot{\mu}(z_2)\exp(R|z_1-z_2|) $
\end{lemma}


At each time step of the game $t = 1, 2,\dots, T$, the learner has to first decide a policy $\chi_t$ that maps any set of context vectors $X$ to a distribution in $\triangle_X$. The learner then observes $X_t = \{\vx_{ti}\}_{i=1}^K$, samples an action $x_t \in X_t$ from $\chi_t(X_t)$,\footnote{When clear from the context, we interchangeably use the arm indices and their corresponding context vectors.} plays arm $x_t$ and obtains reward $r_t$ sampled from GLM distribution. The aim of the learner is to mimimise regret 

$$ R^T = \mathbb{E}\left[\sum_{t=1}^{T}\max_{x \in \mathcal{X}_t} \mu \left( \langle x,\theta^{*}\rangle\right)
 - \sum_{t=1}^{T} \mu \left(\langle x_t,\theta^{*}\rangle\right)\right]$$.

  More specifically, for any arm set $\mathcal{X}$, write optimal arm $x^{*} = \argmax_{x \in \mathcal{X}} \mu\left(\langle x, \theta^{*}\rangle\right)$ and define,

 \begin{equation}
     \kappa := \max_{\mathcal{X} \in \supp(\mathcal{X})} \max_{x \in \mathcal{X}} \frac{1}{\dot{\mu}\left(\langle x, \theta^{*}\rangle\right)}, \text{ }  1/\kappa^{*} := \max_{\mathcal{X} \in \supp(\mathcal{X})}  \frac{1}{\dot{\mu}\left(\langle x^{*}, \theta^{*}\rangle\right)} , \text{ } \frac{1}{\hat \kappa} = \mathbb{E}_{\mathcal{X} \sim \mathcal{D}} \left[\dot{\mu} \left( \langle x^{*},\theta^{*} \rangle\right)\right]
 \end{equation}

We minimize regret in the shuffled model of learning and we now study privacy in the shuffled model of differential privacy, and thus we study regret minimization in the shuffled setting with $M \leq \log \log T$ batches and we let $\mathcal{B}_1,\mathcal{B}_2,\ldots,\mathcal{B}_M$ denote the batches with ${B}_1,{B}_2,\ldots,{B}_M$ denoting their lengths.

\textbf{Batch lengths}: For each $k \in [M]$, we define $B_k$ as follows similar to \cite{sawarni2024generalizedlinearbanditslimited}. The constants $\lambda$ and $\gamma$ are chosen differently to account for the noise addition to preserve privacy.

\begin{equation}{\label{eq:batch_length}}
    B_1 = \left(\frac{\sqrt{\kappa}e^{3S} d^2 \gamma^2}{S} \alpha\right)^{2/3} \text{ , } B_2 = \alpha \text{ and } B_k = \alpha \sqrt{B_{k-1}} \text{ for $k \in [3,M]$}
\end{equation}

We call the first batch as the warmup batch and choose $\alpha = T^{\frac{1}{2(1-2^{-M+1})}}$ if $M \leq \log \log T$ and \sss{define $\gamma$ later.} 

During the warmup batch (first batch), the user computes $G$-optimal design on the arm-set. At the end of the batch, the algorithm computes the estimate of $\theta^{*}$ (call it $\hat\theta_w$) based on the received noisy arm sets ($\vx^{(n)}_t$) and noisy rewards $r^{(n)}_t$. Also, compute the design matrix $\tV^{(n)} : = \sum_{t \in \mathcal{B}_1} x^{(n)}_t(x^{(n)}_t)^\top + \lambda \mI$.


For each round $k \geq 2$, at each round the user elimiates arms from the original arm set $\mathcal{X}_t$ at each round using the confidence bounds computed in the previous rounds. Specifically, it computed a scaled version of the remaining arms as follows. 
\begin{equation}{\label{eq:arm_scaling}}
    \tilde{\mathcal{X}}_t := \left\{\sqrt{\dot{\mu}\left(\langle x, \hat\theta_w \rangle\right) /\beta(x)} x: \text{ for all $x \in \mathcal{X}_t$ }\right\}
\end{equation}
%$$

And now the user applies the G-optimal design on this scaled arm set $\tilde{X}_t$ to choose its arm. Observe the algorithm is a batches algorithm since the policy changes only at the end of each round.


\textbf{Confidence bounds}: The scaled design matrix $H_k$ is computed at the end of each batch $k \in [2,M]$:

\begin{equation}
    \tH^{(n)}_k = \sum_{t \in \mathcal{B}_k} \left(\dot{\mu} \left(\langle x^{(n)}_t, \hat\theta_w\rangle\right)/ \beta(x^{(n)}_t)\right) x^{(n)}_t (x^{(n)}_t)^{\top} + \lambda \mI \text { where } \beta(x) = \exp\left(R \min\left(2S, \gamma \sqrt{\kappa} ||x||_{(V^{(n)})^{-1}}\right)\right) 
\end{equation}

Using this, we first compute the upper and lower bounds as follows very similar to \cite{sawarni2024generalizedlinearbanditslimited}.

\begin{equation}
    \begin{aligned}
    \text{UCB}_k(x) &:= 
        \begin{cases}
            \langle x, \hat \theta_w \rangle + \gamma \sqrt{\kappa} ||x||_{(\tV^{(n)})^{-1}} & \text{if } k = 1 \\
            \langle x, \hat \theta_w \rangle + \gamma \sqrt{\kappa} ||x||_{(\tH^{(n)}_k)^{-1}} & \text{otherwise}
        \end{cases} 
    %\hspace{1cm} & \quad
    \text{LCB}_k(x) := 
        \begin{cases}
            \langle x, \hat \theta_w\rangle - \gamma \sqrt{\kappa} ||x||_{(\tV^{(n)})^{-1}} & \text{if } k = 1 \\
            \langle x, \hat \theta_w \rangle - \gamma \sqrt{\kappa} ||x||_{(\tH^{(n)}_k)^{-1}} & \text{otherwise}
        \end{cases}
    \end{aligned}
\end{equation}

Since $P(r_t| x_t)$ is given by a GLM, the loss function $\ell(\theta,r,x) := r \langle x, \theta \rangle - b \left(\langle x, \theta \rangle\right) + c(r)$ which follows from the Maximum Likelihood Estimate.



{{
\begin{algorithm}[!tb] 
    \caption{ Batched Generalized Linear Bandits Algorithm}
    \label{alg:shuffled_glm} 
    \textbf{Input:} Number of batches $M$ and horizon of play $T$. \\
    %\vspace{-3mm}
    Initialize batches  $\gB_1, \ldots, \gB_M$, as defined in equation (\ref{eq:batch_length})\\%, and set $\lambda \coloneqq 20 R d \log{T}$.%\\ 
        %\texttt{Warmup}
        \For{local user $t \in \gB_1$}{ \label{line:warmup_start} 
        Observe user's arm set $\gX_t$, sample arm $x_t \sim \pi_G(\gX_t)$, %\quad  \texttt{// G-optimal design}
        and observe reward $r_t$. % and update $\bV \leftarrow \bV + x_t x_t^\T$.
        

        \textcolor{gray}{\# For the local randomiser:}

        Send randomised messages $(r^{(n)}_t, x^{(n)}_t) = R(r_t,x_t)$

        
        } \label{line:warmup_end}

        \textcolor{gray}{ \# For the shuffler: }

        Sample a uniform permutation $\rho$ over $\gB_1$ and then apply it to the received messages.
        
        Compute $\hat \theta_w = \argmin_{\substack{\theta }}  \sum_{s\in \gT_1} \ell(\theta, x^{(n)}_{\rho(s)}, r^{(n)}_{\rho(s)}) $ and matrix $\tV^{(n)} = \lambda \mI + \sum_{t \in \gT_1} x^{(n)}_{\rho(t)} \left(x^{(n)}_{\rho(t)}\right)^{\top}$. \\
        %\\ 
        %\texttt{Phased Elimination}
        %Initialize policy $\pi_1$ as \textsc{G-optimal design}. 
        %\alglinelabel{line:}
        \For{batches $k =2$ to $M$}{
        %\STATE Initialize $\bH_k \leftarrow \lambda \bI $.
        \For{each local user
        $t \in \gB_k$}{
            Each user observes $\gX_t$.\\
            \For{$j = 1$ to $k-1$}{  
           Update arm set $\gX_t \leftarrow \gX_t \setminus \{ x \in \gX_t: {\text{UCB}_j} (x) < \max_{y \in \gX_t} \text{LCB}_j (y) \}$. \\
            \label{line:filter_arms}
            }
            Scale $\gX_t$, as in \cref{eq:arm_scaling}, to obtain $\tilde{\gX}_t$.\label{line:modified_arms}, then
             sample $x_t \sim \pi^G\left(\tilde{\gX_t} \right)$.  \label{line:d_opt_sampling} 

             \textcolor{gray}{\# For the local randomiser:}

        Send randomised messages $(r^{(n)}_t, x^{(n)}_t) = R(r_t,x_t)$
        }

         \textcolor{gray}{ \# For the shuffler: }

        Sample a uniform permutation $\rho$ over $\gB_1$ and then apply it to the received messages.

        % $\hat\theta_k = \argmin_\theta \sum_{s \in \mathcal{A} } \ell( \theta, x^{(n)}_s, r^{(n)}_s)$. 
        

        Define $\tH^{(n)}_k = \lambda \mI + \sum_{t \in \gB_k} \left(\dot{\mu} \left(\langle x^{(n)}_{\rho(t)}, \hat\theta_w\rangle\right)/ \beta(x^{(n)}_{\rho(t)})\right) x^{(n)}_{\rho(t)} (x^{(n)}_{\rho(t)})^{\top} + \lambda \mI$, and
        compute $\hat\theta_k = \argmin_\theta \sum_{s \in \mathcal{B}_k } \ell\left(\theta, x^{(n)}_{\rho(s)}, r^{(n)}_{\rho(s)}\right)$. \label{line:batch_end}  
        %\State Compute \textsc{Distributional optimal design} policy $\pi_{k} $ using the arm sets $\{ \cX_t \}_{t \in \mathcal{B}}$. 
       }
   
\end{algorithm}
}}

\subsection{Achieving privacy via LDP shuffling}

The local randomiser $R(.)$ computes the noisy reward $r^{(n)}$ from reward $r$ by adding Gaussian noise of variance $\sigma^2_1$ and computed the noisy feature vector $x^{(n)}_t$ from the feature vector $x_t$ by adding Gaussian noise of variance $\sigma^2_2$ to each component. Further, we define the noise levels 
$$\sigma_1 = R\sigma_2 = \frac{4R \sqrt{2 \log (\frac{2.5B_k}{\delta}) \log (2/ \delta)}}{\epsilon \sqrt{B_k}}$$.

The noise level $\sigma_1$ and $\sigma_2$ is chosen so that the randomiser satisfies $(\epsilon,\delta)$ LDP. 


\subsubsection{Privacy analysis}

%Denote the size of $k^{th}$ batch by $B_k = \gT_k - \gT_{k-1}$ and define noise levels $\sigma_1 = \sigma_2 = \frac{4 \sqrt{2 \log (\frac{2.5B_k}{\delta}) \log (2/ \delta)}}{\epsilon \sqrt{B_k}}$.

We restrict the privacy parameter $\epsilon \leq \sqrt{\frac{\log (2/ \delta)}{T}}$ and $\delta \leq 1$. Setting $\epsilon_0 = \frac{\epsilon \sqrt{B_k}}{\sqrt{\log (2/\delta)}}$ and $\delta_0 = \frac{\delta}{B_k}$, we observe that $\sigma_1 = R\sigma_2 = \frac{4R \sqrt{2 \log \left(\frac{2.5}{\delta_0}\right)}}{\epsilon_0}$. Using the standard Gaussian mechanism \cite{dworkdpbook} and boundedness, we can observe both of the local randomisers $R(.)$ is $(\epsilon_0/2,\delta_0/2)$ LDP. \footnote{While the reward vector \( r_t \) is bounded by \( R \), the vector \( x_t \) is bounded by 1, which distinguishes \( \sigma_1 \) and \( \sigma_2 \).
} Now applying \cref{lem:shuffle_amp} and composition theorem, we can observe that the mechanism is $(\epsilon,\delta)$ SDP. 



\subsection{Regret Analysis}

Define $$(\tH^{(n)}_k)^{*} = \sum_{t \in \mathcal{B}_k} \dot{\mu} \left(\langle x^{(n)}_t, \theta^{*}\rangle\right)x^{(n)}_t (x^{(n)}_t)^{\top} + \lambda \mI \text{ for $k \in [2,M]$}$$ 

and we similarly define 

\begin{equation}
    \tV = \sum_{t \in \mathcal{B}_1} \dot{\mu}\left(\langle x_t, \theta \rangle\right) \text { and } \tH_k = \sum_{t \in \mathcal{B}_k} \dot{\mu}\left(\langle x_t, \theta \rangle\right)
\end{equation}

\begin{lemma}
    $\tH^{*}_k $
\end{lemma}


\begin{lemma}
    Let $y$ be a fixed vector with $||y||<1$. Then, with notation setup in Lemma , the following inequality holds with probability at least $1-\delta$

    $$\sum_{j=1}^{s} \left( \mu\left( \langle \theta^{*},x^{(n)}_j\right) -r^{(n)}_j \right) y^{\top} (\tH^{*})^{-1/2} x^{(n)}_j $$
\end{lemma}

\begin{proof}
    We first define 
\end{proof}



\begin{lemma}{\label{lemma:bounding_matrix_sum}}
        Consider $\vx_1,\vx_2, \ldots,\vx_n \in \mathbb{R}^d$ with $\ell_2$ norm bounded by 1. We now define i.i.d random vectors $\{n_i\}_{i=1}^{n} \sim \mathcal{N}(0,\sigma^2\mI)$. For $n>d^2$, with probability at least $(1-\delta)$, 
        
        
        $$\left|\left| \sum_{i=1}^{n} (x_i+n_i)(x_i+n_i)^T - \sum_{i=1}^{n} x_i x^T_i\right|\right| \leq  2d\sqrt{2n\sigma^2} \log (4d^2/\delta) + 5n\sigma^2 $$
    \end{lemma}


    \begin{proof}
        We first simplify 
        \begin{equation}
            \sum_{i=1}^{n} (x_i+n_i)(x_i+n_i)^T - \sum_{i=1}^{n} x_i x^T_i
            = \sum_{i=1}^{n} (x_in^{T}_i + x^{T}_i n_i) + \sum_{i=1}^{n} n_i n^{T}_i
        \end{equation}

        With probability at least $(1- \frac{\delta}{2})$ using \cite[Chapter 6]{Wainwright_2019} that $$\left|\left|\sum_{i=1}^{n} n_i n^{T}_i\right|\right| \leq n\sigma^2  + 4 \sigma^2 \max \left(\sqrt{n(d+ \log (2/ \delta))}, (d+ \log (2/ \delta)) \right)$$.


        Now we bound the operator $\ell_2$ norm of $\sum_{i=1}^{n} x_in^{T}_i$ and observe that the $(j,k)^{th}$ entry of matrix is given by $\sum_{i=1}^{n} x_{i,j}n_{i,k}$.  Using matrix norm inequalities \footnote{This follows since $||A||_2 \leq \sqrt{d}(||A||_1, ||A||_1)$ for $A \in \mathbb{R}^{d\times d}$},


        \begin{align}
            \left|\left| \sum_{i=1}^{n} x_i n^T_i\right|\right| \leq \max_{j \in [d]} \left(\sum_{k \in [d]} \left|\sum_{i \in [d]} x_{i,j} n_{i,k}\right| \right) 
        \end{align}


        Now observe that $\sum_{i \in [d]} x_{i,j} n_{i,k}$ that this is a zero mean Gaussian random variable with variance $\sum_{i} x^2_{i,j}\sigma^2$. Thus for a given $(j,k)$, with probability at least $(1-\frac{\delta}{4d^2})$, we have $\left|\left|\sum_{i \in [d]} x_{i,j} n_{i,k}\right|\right|_2 \leq \sqrt{2\sum_{i} x^2_{i,j}\sigma^2} \log (4d^2/\delta)$. Union-bounding over all $(j,k)$ pairs we have with probability at least $(1-\frac{\delta}{4})$, we have $\left|| \sum_{i=1}^{n} x_i n^T_i|\right| \leq d\sqrt{2n\sigma^2} \log (4d^2/\delta)$. Using a similar approach, one can bound 
        $\left|| \sum_{i=1}^{n} x_i n^T_i|\right|$ as well and thus, we have 

        \begin{equation}
            \left|\left| \sum_{i=1}^{n} (x_i n^T_i + n_i x^T_i)\right|\right| \leq 2d\sqrt{2n\sigma^2} \log (4d^2/\delta) \text{ with probability at least $1-\delta/2$}.
        \end{equation}


       
        
    \end{proof}

    While we define quantities $\tH_k, \tH^{*}_k \text{ and } \tV$ using the noisy rewards $r^{(n)}_t$ and played arms $x^{(n)}_t$, we now define $\tilde{\tH}_k, \tilde{\tH}^{*}_k \text{ and } \tilde{\tV}$ using the true rewards below. 


\begin{equation} {\label{eq:denoised_vect_H}}
    \tilde{\tH}^{*}_k = \lambda^{(h)}_1 \mI + \sum_{t \in \gB_k} \dot{\mu} \left(\langle x_t , \theta^{*}\rangle\right) x_t x^{\top}_t \text{ for $k \geq 2$ }%; \tilde{\tH}_k = \lambda \mI + \sum_{t \in \gB_k} \frac{\dot{\mu} \left(\langle x_t , \hat \theta_w\rangle\right)}{\beta (x_t)} x_t x^{\top}_t \text{ for $k \geq 2$}
\end{equation}

% \begin{equation}{\label{eq:denoised_vect_H}}
%     \tilde{V} = \lambda \mI + \sum_{t \in \gB_1} x_t x^{\top}_t
% \end{equation}

\begin{lemma}{\label{lemma:upper_bound_H_k}}
    With probability at least $1- \frac{\log \log T}{T^2}$, we have
    $$\tH_k \preceq \lambda^{(h)}_1\mI + \sum_{t \in \gB_k} \frac{\dot{\mu} \left(\langle \hat \theta_w, x_t\rangle\right)}{\beta(x_t)} x_t x^{\top}_t \text{ for $k \in [2,M]$ and } \tV \preceq \lambda^{(h)}_1\mI + \sum_{t \in \gB_1} x_t x^{\top}_t$$
\end{lemma}


\begin{proof}
    First, observe that $\tH_{k} = \lambda \mI+ \sum_{t \in \gB_k} \frac{\dot{\mu} \left(\langle \hat \theta_w, x_t\rangle\right)}{\beta(x_t)} x_t x^T_t + \gN_{k}$. Observe that $\gN_{k}$ is  upper diagonal elements being independent Gaussian elements with variance $\sigma^2_{(k)}B_{k} = \frac{32}{(\kappa^{*})^2\epsilon^2} \log \left(\frac{2.5B_{\kappa}}{\delta}\right) \log \left(2/\delta\right)$. Thus using \cite[Corollary 4.4.8]{vershynin_high-dimensional_2018}, $$\prob{||\gN_{\kappa}|| >\frac{32}{\epsilon \kappa^{*}} \sqrt{ \log \left(\frac{2.5B_{k}}{\delta}\right) \log \left(2/\delta\right)} (\sqrt{d}+ \gamma)} \leq 1/2 \exp(-\gamma^2)$$. 

    Setting $\gamma = 6 \sqrt{\log \left(2dT\right)}$ we get the desired result. Further since $T> e^{O(d)}$, we can bound $\sqrt{d} + \gamma$ by $2\gamma$.

    The bound on $\tV$ also follows similarly.
    
    
    %A very similar technique can be used to bound $\tV$ as well.
\end{proof}

We now show that $\tilde{\tH}^{*}_k, \tilde{\tH}_k \text{ and } \tilde{\tV}$ is upper bounded
by  ${\tH}^{*}_k, {\tH}_k \text{ and } {\tV}$ upto small multiplicative and additive factors with high probability under symmetric matrix inequalities.


\sss{Key issue in analysis is the exponent term present here. To address this we may need to bound the magnitude of noise added. However, key issue is that we may have to move to laplace bounded noise. 

One key paper here is "Truncated Laplacian Mechanism for Approximate
Differential Privacy"



}

\begin{lemma}
    With probability at least $1-\frac{ \log \log T}{T^2}$ we have 

    $$\tH^{*}_k \succeq \exp \left(-\frac{7RS\sqrt{d}}{\epsilon} \frac{(\log (T/ \delta))^2}{T^{0.25}}\right) \tilde{\tH}^{*}_k\text{ and }\tilde{\tH}^{*}_k \succeq \tH_k \text{ } \forall k \in [M].$$
    
\end{lemma}


\begin{proof}

Let $n_{t,1} \sim \gN(0, \sigma^2_1 \mI)$ denote the noise added to chosen arm $x_t$ where $\sigma^2_1 = \frac{16}{\epsilon^2 B_k} \log \left( \frac{2.5 B_k}{\delta} \right) \log (2/ \delta)$  

Applying \cref{eq:bounding_mu_dot_log_ratio}, for a given $t \in \gB_k$, we have 


\begin{equation}
    \left| \log \left(\frac{\dot{\mu} \left( \langle \theta^{*}, x^{(n)}_t\rangle\right)}{\dot{\mu} \left( \langle \theta^{*}, x_t\rangle\right)}\right)\right| \leq R \left| \langle \theta^{*}, n_{t,1} \rangle\right| \leq \frac{7RS\sqrt{d}}{\epsilon} \frac{(\log (T/ \delta))^2}{T^{0.25}} \text{ w.p. at least $1- \frac{1}{2T^3}$}
\end{equation}


% Thus, 

% % \begin{align}
% %     \tH^{*}_k \succeq & \exp\left(-\frac{7RS\sqrt{d}}{\epsilon} \frac{(\log (T/ \delta))^2}{T^{0.25}}\right) \left(\lambda \mI + \sum_{t \in \gB_k} \dot{}\right) \text{ w.p at least $1-\frac{1}{2T^2}$} \\
% %     \succeq & 
% % \end{align}

% Now, 
% \begin{align}
%     \sum_{t \in \gB_k} \dot{\mu} \left(\langle x_t, \theta^{*}\rangle\right) \left(x^{(n)}_t \right)
% \end{align}

% Now similarly 


%Observe that the last inequality follows from the fact that $\langle \theta^{*}, n_{t,1} \rangle$ is zero mean Gaussian with variance $S^2 \sigma^2_1$. Thus, with probability at least $1- \frac{1}{T^3}$, one may bound it by $S \sigma_1 \log (T^3) \leq \frac{6S}{\epsilon} \frac{(\log (T/\delta))^2}{T^{1/4}}$. This follows since the smallest batch size $B_2 \geq \sqrt{T}$.

Now we invoke \cref{lemma:bounding_scaled_matrix_sum} to argue that \footnote{Choose $\dot{\mu} (x,\theta^{*})$ as the function $f(x)$ which is bounded by $1/ \kappa^{*}$.} 

\sss{Invoke some lower bounds on $T$ and define appropriately}

\begin{equation}
    \tH^{*}_k \succeq \exp \left(-\frac{7RS\sqrt{d}}{\epsilon} \frac{(\log (T/ \delta))^2}{T^{0.25}}\right) \tilde{\tH}^{*}_k \text{ w.p at least $1-1/T^2$.}
\end{equation}


From \cref{lemma:multiplicative_bound}, we have $\dot{\mu} \left(\langle x_t, \theta^{*} \rangle\right) \geq \frac{\dot{\mu} \left( \langle x_t, \hat\theta_w\rangle\right)}{\beta(x_t)}$. Now apply \cref{lemma:upper_bound_H_k} to conclude the proof. 

Now applying  \cref{lemma:upper_bound_H_k}, we can show with high probability $\tilde{\tH}^{*}_k \succeq \tH_k$ and thus, conclude the proof.





    
    
\end{proof}


\sss{Also mention $x_j$ correspond to some arm from the support of $\gD$.}

\begin{lemma}
    Let $y$ be a fixed vector with $||y||<1$. Then, with notation setup in Lemma , the following inequality holds with probability at least $1-\delta$

    $$\sum_{j=1}^{s} \left( \mu\left( \langle \theta^{*},x^{(n)}_j \rangle\right) -r^{(n)}_j \right) y^{\top} (\tH^{*})^{-1/2} x^{(n)}_j $$
\end{lemma}




% \begin{claim}
    
% \end{claim}

\begin{proof}
    Let $n_{j,1} \sim \mathcal{N}(0,\sigma^2_1 \mI)$ and $n_{j,2} \sim \mathcal{N}(0,\sigma^2_2 )$ denote the noise added to feature vector $x_j$ and reward $r_j$. From mean value theorem we have,



    \begin{align}
        \mu\left( \langle \theta^{*},x^{(n)}_j\rangle\right)
        =\mu\left( \langle \theta^{*},x_j\rangle\right) + \dot{\mu}(z_j) (\langle \theta^{*}, n_{j,1} \rangle) \text{ for some  $z_j$ between $\langle \theta^{*},x_j \rangle, \langle \theta^{*},x^{(n)}_j \rangle$}
    \end{align}

    % Further, applying \cref{lemma:multiplicative_bound} and concentration property of a Gaussian distribution, we can argue with probability at least $\left(1-\frac{\delta}{4}\right)$ that $\frac{e^{-2RS}}{\kappa} \leq \dot{\mu}(z_j) \leq \frac{e^{2RS}}{\kappa^{*}} \text{ } \forall j \in [s]$. 


    
    Given a $j \in [s]$, applying \cref{lemma:multiplicative_bound}, we get 

    \begin{align}{\label{eq:bounding_mu_dot_log_ratio}}
        \left| \log \left(\frac{\dot{\mu}(z_j)}{\dot{\mu} \left(\langle \theta^{*},x_j \rangle\right)}\right)\right| \leq & R \left|\langle \theta^{*},n_{j,1}\rangle\right|\nonumber\\
        \overset{(a)}{\leq} & \min \left(2RS \sigma_1 \sqrt{ \log (8s/\delta)},R \left|\langle \theta^{*},n_{j,1}\rangle\right| \right) \text{ with probability at least $1- \delta/8s$}
    \end{align}


    $(a)$ follows from the fact that $\langle \theta^{*},n_{j,1} \rangle$ is zero mean Gaussian with variance $\sigma S$. Now apply concentration bounds to get the desired result. 


    %With probability at least $1- \delta/8$, we have the following

    \begin{align}
        & \left|\left|\sum_{j=1}^{s} \left(\left( \mu\left( \langle \theta^{*},x^{(n)}_j \rangle\right) -r^{(n)}_j \right)  x^{(n)}_j -\left( \mu\left( \langle \theta^{*},x_j \rangle\right) -r_j \right) x_j \right)\right|\right| \nonumber\\
        = &  \quad \underbrace{\left|\left|\sum_{j=1}^{s}\left(\mu\left( \langle \theta^{*},x_j \rangle\right) -r_j\right)n_{j,1} \right|\right|}_{\text{(I)}}  + \underbrace{\left|\left|\sum_{j=1}^{s} n_{j,2} x_j\right|\right|}_{\text{(II)}}+ \underbrace{\left|\left|\sum_{j=1}^{s}\dot{\mu}(z_j) \langle \theta^{*}, n_{j,1} \rangle x_j\right|\right|}_{\text{(III)}} + \underbrace{\left|\left|\sum_{j=1}^{s} \left(\dot{\mu}(z_j) \langle \theta^{*}, n_{j,1} \rangle - n_{j,2} \right)n_{j,1} \right|\right|}_{\text{(IV)}} \label{eq:bounding_diff_1}
\end{align}


%2se^{2RS}\sqrt{d}\sigma_1 \sigma_2 \left(\log (8s/\delta)\right)^2
    %Since $\dot{\mu} (z_j) \leq \frac{e^{2RS}}{\kappa^{*}}$, 
    
    Now we have \begin{align}
        (IV) & \leq \left|\left|\sum_{j=1}^{s}\dot{\mu}(z_j) (\langle \theta^{*}, n_{j,1} \rangle) n_{j,1} \right| \right| + \left|\left| \sum_{j=1} ^{s} n_{j,1} n_{j,2}  \right|\right|\\
        & \overset{(b)}{\leq} \frac{e^{{2RS\sigma_1 \sqrt{ \log (8s/ \delta)}}}}{\kappa^{*}}S \left|\left|\sum_{j=1}^{s} n_{j,1} n_{j,1}^{\top}\right|\right| + \left|\left| \sum_{j=1}^{s} n_{j,2} n_{j,1} \right|\right| \text{ w.p. at least $1-\delta/8$ }\\
        & \overset{(c)}{\leq} \frac{Se^{{2RS\sigma_1 \sqrt{ \log (8s/ \delta)}}}}{\kappa^{*}}(s + \log (16/\delta)) (\sigma^2_1 + \sigma^2_2\sigma^2_1) \text{ w.p at least $1-\delta/8$} 
    \end{align}



    (b) follows since $\dot{\mu}(z_j) \leq \frac{e^{2RS\sigma_1 \sqrt{ \log \left( \frac{8s}{\delta} \right)}}}{\kappa^{*}} \quad \forall j \in [s]$ with probability at least \( 1 - \frac{\delta}{8} \), which follows from \cref{eq:bounding_mu_dot_log_ratio} and a union bound.


    $(c)$ follows on applying Covariance estimation bounds from \cite[Chapter 6]{vershynin_high-dimensional_2018}.  

    % The last term follows by applying concentration bounds on the Gaussian distribution. 

    

    Observe that the random variables $n_{j,1}$ and $r_j$ are independent. Now applying concentration bounds on the Gaussian distribution, we have

    \begin{equation}
        (I) \leq \sqrt{ds} (R+1)\sigma_2 \log (4/\delta) \text{ w.p. at least $(1-\delta/4)$}    
    \end{equation}

    Similarly, we get 

    \begin{equation}
        (II) \leq \sqrt{ds} \sigma_2 \log (4/\delta) \text{ w.p. at least $(1-\delta/4)$} 
    \end{equation}

    To bound (III), we use the following inequalities using convexity of $e^x$


    \begin{align}
        1 - |x| \leq e^x \leq (e^M - 1) \frac{|x|}{M} + 1 \text{ for $x \in (-\infty,M]$}
    \end{align}


    
    
    Thus, from \cref{eq:bounding_mu_dot_log_ratio}, we get with probability at least $1-\delta/8$,

    \begin{align}
         1 - R |\langle \theta^{*},n_{j,1} \rangle|\leq \frac{\dot{\mu}(z_j)}{\dot{\mu} \left(\langle \theta^{*},x_j \rangle\right)} \leq 1+ \left(\frac{e^{2RS\sigma_1 \sqrt{ \log (8s/ \delta)}}-1}{2RS\sigma_1 \sqrt{ \log (8s/ \delta)}}\right)R \left|\langle\theta^{*}, n_{j,1} \rangle\right| \text{ } \forall j \in [s]
    \end{align}

    Thus with probability at least $1- \delta/8$, we have

    \begin{align}
        \sum_{j=1}^{s} \dot{\mu}(z_j) \langle \theta^{*},n_{j,1} \rangle x_j \overset{(d)}{\leq} \sum_{j=1}^{s} \dot{\mu}\left(\langle \theta^{*},x_j\rangle\right) \langle \theta^{*},n_{j,1} \rangle x_j + \left(\frac{e^{2RS\sigma_1 \sqrt{ \log (8s/ \delta)}}-1}{2R\kappa^{*}S\sigma_1 \sqrt{ \log (8s/ \delta)}}\right)R \sum_{j=1}^{s} \langle \theta^{*},n_{j,1} \rangle^2 |x_j|
    \end{align}


    
     
    The second term in $(d)$ follows from the fact that $-|b|< a < R|b|$ implies that $ab \leq Rb^2$ for any two real numbers $a,b$ and a constant $R>1$. Now apply this inequality point-wise to every co-ordinate in the vector. We also use the fact that $\dot{\mu} \left(\langle \theta^{*},x_j\rangle\right) \leq \frac{1}{\kappa^{*}}$.

    Thus, 

    \begin{align}
        (II) \overset{(e)}{\leq} & \left| \left|\sum_{j=1}^{s} \dot{\mu}\left(\langle \theta^{*},x_j\rangle\right) \langle \theta^{*},n_{j,1} \rangle x_j\right| \right| + \frac{Re^{2RS\sigma_1 \sqrt{ \log (8s/ \delta)}}-1}{2R\kappa^{*}S\sigma_1 \sqrt{ \log (8s/ \delta)}} \sum_{j=1}^{s} \langle \theta^{*}, n_{j,1}\rangle^2 \text { w.p at least $1-\delta/8$} \nonumber\\
        \leq & \sqrt{dSs/ \kappa^{*}} \sigma_1 \log (4/ \delta) + \frac{Re^{2RS\sigma_1 \sqrt{ \log (8s/ \delta)}}-1}{2R\kappa^{*}S\sigma_1 \sqrt{ \log (8s/ \delta)}} S^2 \sigma^2_1 (s + \log (16 /\delta) \text { w.p at least $1-\delta/4$}
    \end{align}

    The last inequality follows from the fact that $\langle \theta^{*}, n_{j,1} \rangle$ is a zero-mean Gaussian random variable with variance $S^2 \sigma^2_1$. Now observe that the first term is a zero mean Gaussian random vector and apply desired concentration bounds on Gaussian. The second term also follows from similar arguments.


    Sum up to conclude the proof


    %\sqrt{dSs/ \kappa^{*}} \sigma_1 \log (4/ \delta)

    %Since, $\dot{\mu}(z_j)$ with  
    
    
\end{proof}


\begin{lemma}
    Let 
\end{lemma}



\begin{lemma}{\label{lemma:bounding_scaled_matrix_sum}}
        Consider $x_1,x_2, \ldots,x_n \in \mathbb{R}^d$ with $\ell_2$ norm bounded by 1. We now define i.i.d random vectors $\{n_i\}_{i=1}^{n} \sim \mathcal{N}(0,\sigma^2\mI)$. Consider a function $f: \mathbb{R}^d \rightarrow \mathbb{R}_{\geq 0}$ satisfying $\max_i f(x_i) \leq M$. Then for $n>d^2$, with probability at least $(1-\delta)$, 
        
        
        $$\left|\left| \sum_{i=1}^{n} f(x_i)(x_i+n_i)(x_i+n_i)^T - \sum_{i=1}^{n} f(x_i) x_i x^T_i\right|\right| \leq  M(2d\sqrt{2n\sigma^2} \log (4d^2/\delta) + 5n\sigma^2) $$
    \end{lemma}


    \begin{proof}
        We first simplify 
        \begin{align}
            \sum_{i=1}^{n} f(x_i)(x_i+n_i)(x_i+n_i)^T - \sum_{i=1}^{n} f(x_i)x_i x^T_i
            = \sum_{i=1}^{n} f(x_i) (x_in^{T}_i + x^{T}_i n_i) + \sum_{i=1}^{n} f(x_i) n_i n^{T}_i
        \end{align}

        Refer to this lecture note as well.
        %https://www.stat.cmu.edu/~siva/teaching/709/lec8.pdf

        With probability at least $(1- \frac{\delta}{2})$ using \cite[Chapter 6]{Wainwright_2019} that 
        
        \begin{equation}{\label{eq:temp_1}}
            \left|\left|\sum_{i=1}^{n} f(x_i) n_i n^{T}_i\right|\right| \leq M \left(n\sigma^2  + 4 \sigma^2 \max \left(\sqrt{n(d+ \log (2/ \delta))}, (d+ \log (2/ \delta)) \right)\right)
        \end{equation}


        Now we bound the operator $\ell_2$ norm of $\sum_{i=1}^{n} f(x_i) x_in^{T}_i$ and observe that the $(j,k)^{th}$ entry of matrix is given by $\sum_{i=1}^{n} f(x_i) x_{i,j}n_{i,k}$.  Using matrix norm inequalities \footnote{This follows since $||A||_2 \leq \sqrt{d}(||A||_1, ||A||_1)$ for $A \in \mathbb{R}^{d\times d}$},


        \begin{align}
            \left|\left| \sum_{i=1}^{n} f(x_i) x_i n^T_i\right|\right| \leq \max_{j \in [d]} \left(\sum_{k \in [d]} \left|\sum_{i \in [d]} f(x_i)x_{i,j} n_{i,k}\right| \right) 
        \end{align}


        Now, observe that $\sum_{i \in [d]} f(x_i) x_{i,j} n_{i,k}$ that this is a zero mean Gaussian random variable with variance $\sum_{i} (f(x_i))^2 x^2_{i,j}\sigma^2$. Thus, for a given $(j,k)$, with probability at least $(1-\frac{\delta}{4d^2})$, we have $\left|\left|\sum_{i \in [d]} (f(x_i))^2 x_{i,j} n_{i,k}\right|\right|_2 \leq \sqrt{2\sum_{i} f(x_i) x^2_{i,j}\sigma^2} \log (4d^2/\delta)$. Union-bounding over all $(j,k)$ pairs, we have with probability at least $(1-\frac{\delta}{4})$, $\left|\left| \sum_{i=1}^{n} f(x_i) x_i n^T_i\right|\right| \leq dM\sqrt{2n\sigma^2} \log (4d^2/\delta)$. Using a similar approach, one can bound 
        $\left|| \sum_{i=1}^{n} x_i n^T_i|\right|$ as well and thus, we have 

        \begin{equation}\label{eq:temp_2}
            \left|\left| \sum_{i=1}^{n} f(x_i) (x_i n^T_i + n_i x^T_i)\right|\right| \leq 2dM\sqrt{2n\sigma^2} \log (4d^2/\delta) \text{ with probability at least $1-\delta/2$}.
        \end{equation}

        Combining \cref{eq:temp_1} and \cref{eq:temp_2}, we get the desired result.


       
        
    \end{proof}


==> header.tex <==
\usepackage{hyperref}

\usepackage[numbers,semicolon,square,authoryear]{natbib}
%\usepackage[style=alphabetic]{biblatex}
%\usepackage{bibtex}


%\usepackage{mathpazo}
%\usepackage{euler}

\usepackage{url}
\usepackage{amsthm, amssymb}
\usepackage{verbatim}
\usepackage[inline]{enumitem}
\usepackage{xcolor}
\usepackage[ruled,noline,noend,linesnumbered]{algorithm2e}

\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor    = blue, %Colour of citations
  linktoc      = page
}
\setlist[enumerate, 1]{label=(\alph*)}
\setlist[enumerate]{nosep}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}
%\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}{Lemma}
%\newtheorem{coro}[thm]{Corollary}
\newtheorem{fact}{Fact}

\theoremstyle{definition}
\newtheorem{defn}{Definition}
%\newtheorem{assum}{Assumption}
%\newtheorem{ex}{Exercise}
%\newtheorem{eg}{Example}
%\newtheorem{prob}{Problem}

\theoremstyle{remark}
%\newtheorem{claim}{Claim}
%\newtheorem{rem}{Remark}

\SetCommentSty{rmfamily}

\SetKwComment{Comment}{$\triangleright$\ }{}

\renewcommand{\algorithmautorefname}{Algorithm}
\newcommand{\lemautorefname}{Lemma}
\newcommand{\defnautorefname}{Definition}
\newcommand{\propautorefname}{Proposition}
\newcommand{\thmautorefname}{Theorem}
\newcommand{\factautorefname}{Fact}
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}
\renewcommand{\algorithmcflinename}{Line}



\SetNlSty{textbf}{}{:}


==> ldp_shuffling_lm.tex <==
% \subsection{Achieving privacy via LDP shuffling}\label{sec:ldp_amplification_shuffling}

% In this section, we use our general framework that enables us to use existing LDP mechanisms for linear contextual bandits to attain a better tradeoff. The key idea to obtain a shuffled differntial private protocol is to use private amplification by shuffling protocol \cite{feldman2021hidingclonessimplenearly}. The privacy guarantee in the $k^{th}$ batch can be amplified by approximately $\sqrt{B_k}$ by randomly permuting the responses of all the users in the $k^{th}$ batch. The (local) randomiser functions $R_1(.)$ and $R_2(.)$ injects independent Gaussian noise of variance $\sigma^2_1$ and $\sigma^2_2$ to each entry of the vector $r_t x_t$ and matrix $x_t x_t^T$. However, we ensure that the noise matrix that is added by randomiser function $R_2(.)$ is symmetric by perturbing upper diagonal entries and copying them to the lower terms. Further, we define the parameters as follows.


% \begin{align}{\label{eq:parameters_ldp_shuffle}}
%     \sigma_1 & = \sigma_2  = \frac{4 \sqrt{2 \log (\frac{2.5B_k}{\delta}) \log (2/ \delta)}}{\epsilon \sqrt{B_k}} \text{         
%       } \\
%      \alpha & = 80\epsilon^{-1}\sqrt{\log \left(2dKT\right) \log (T/ \delta)} \nonumber\\
%     \lambda & = 16 \log (2dT) + \sqrt{B_k} \sigma_2 (\sqrt{d} + 6 \sqrt{\log (2dKT)})
% \end{align}
% % $$$$.

% The parameters $\sigma_1$ and $\sigma_2$ are chosen to ensure $(\epsilon,\delta)$ SDP after application of amplification by shuffling lemma \cite[Theorem 3.8]{feldman2021hidingclonessimplenearly} (restated in \cref{lem:shuffle_amp})

% \begin{theorem}{\label{thm:privacy_regret_LDP_shuffle}}
%     Suppose the privacy parameter $\epsilon \leq \sqrt{\frac{\log (2 \delta)}{T}}$ and $\delta \leq 1$ with $T > e^d$. Then setting parameters $\sigma_1, \sigma_2$ and $\lambda$ as defined in \cref{eq:parameters_ldp_shuffle} ensures that the following bound on the expected regret $R^T$

%     \begin{equation}
%         R^T = O\left(\frac{d}{\epsilon} \sqrt{T \log \left({2dKT}\right) \log (\frac{T}{\delta}) \log (2/ \delta)}  \log \log T\right)
%     \end{equation}
% \end{theorem}


% % Set $$$$.

% %$$$$

% %which follows from an upper bound on $\alpha$ in \cref{thm:general_regret_guarantee}.

% %+ 28 \sqrt{\frac{32}{\epsilon} \log \left(\frac{2.5B_k}{\delta}\right) \log \left(2/\delta\right)\log \left(\frac{2dKT}{\delta}\right)}




% \sss{Define the shuffle protocols and amplification $(S_{\text{amp}},R_{\text{amp}}, P_{\text{amp}})$ formally in boxes and also define $R_{\text{amp}}$ as combination of two protocols.}

% \sss{Check the bounds on $R$ and $S$ got correctly reflected.}

% Before, we analyse the performance (regret and privacy guarantee), we first state the amplification by shuffling lemma \cite[Theorem 3.8]{feldman2021hidingclonessimplenearly}. Observe that we have a fixed local randomiser rather than an adaptive one in \cite{feldman2021hidingclonessimplenearly} and we also first randomise then shuffle in our setup. However, since the local randomiser is fixed, these two cases are equivalent.

% \begin{lemma}[Amplification by shuffling \cite{feldman2021hidingclonessimplenearly}]
% \label{lem:shuffle_amp}
% Consider a one-round protocol $\gP=(\gR, \gS, \gA)$ over $n$ users. 
% Let $\gR$ be an $(\epsilon_0,\delta_0)$-LDP mechanism. Then, for any $\delta' \in [0,1]$ such that $\epsilon_0 \le \log(\frac{n}{16\log(2/\delta')})$,  $\gP$ is $(\widetilde{\epsilon},\widetilde{\delta})$-SDP, i.e., the analyzer's view is $(\widetilde{\epsilon},\widetilde{\delta})$-DP, where 
% \begin{align*}
%     \widetilde{\epsilon} & \le \log\left(1+ \frac{e^{\epsilon_0}-1}{e^{\epsilon_0}+1} \left(\frac{8\sqrt{e^{\epsilon_0}\log(4/\delta')}}{\sqrt{n}}  + \frac{8e^{\epsilon_0}}{n}\right)\right), \\
%      \widetilde{\delta} & = \delta' + (e^{\epsilon} + 1)\left(1+\frac{e^{-\epsilon_0}}{2}\right)n\delta_0,
% \end{align*}
% That is, when $\epsilon_0 > 1$, $\widetilde{\epsilon} = O\left(\frac{\sqrt{e^{\epsilon_0}\log(1/\delta') }}{\sqrt{n}}\right)$ and when $\epsilon_0 \le 1$, $\widetilde{\epsilon} = O\left(\epsilon_0\frac{\sqrt{\log(1/\delta')}}{\sqrt{n}}\right)$.
% \end{lemma}

% % Set $\alpha = 8\epsilon^{-1}\sqrt{\log \left(\frac{2dKT}{\delta}\right)} \left(4 \sqrt{d } + \sqrt{ 6 \log (\frac{2dkT}{\delta})}\right)$.



% \subsubsection{Privacy analysis}

% %Denote the size of $k^{th}$ batch by $B_k = \gT_k - \gT_{k-1}$ and define noise levels $\sigma_1 = \sigma_2 = \frac{4 \sqrt{2 \log (\frac{2.5B_k}{\delta}) \log (2/ \delta)}}{\epsilon \sqrt{B_k}}$.

% We restrict the privacy parameter $\epsilon \leq \sqrt{\frac{\log (2/ \delta)}{T}}$ and $\delta \leq 1$. Setting $\epsilon_0 = \frac{\epsilon \sqrt{B_k}}{\sqrt{\log (2/\delta)}}$ and $\delta_0 = \frac{\delta}{B_k}$, we observe that $\sigma_1 = \sigma_2 = \frac{4 \sqrt{2 \log \left(\frac{2.5}{\delta_0}\right)}}{\epsilon_0}$. Using the standard Gaussian mechanism \cite{dworkdpbook} and boundedness, we can observe both of the local randomisers $R_1(.)$ and $R_2(.)$ is $(\epsilon_0/2,\delta_0/2)$ LDP. Now applying \cref{lem:shuffle_amp} and composition theorem, we can observe that the mechanism is $(\epsilon,\delta)$ SDP. 

% \begin{observation}
%     For privacy via the LDP protocol, choosing $\sigma_1 = \sigma_2 = \frac{4 \sqrt{2 \log (\frac{2.5B_k}{\delta}) \log (2/ \delta)}}{\epsilon \sqrt{B_k}}$ ensures that \cref{ass:subGaussian_noise} is satisfied with 

%     $$ \tilde{\sigma} = \frac{4 \sqrt{2 \log (\frac{2.5B_k}{\delta}) \log (2/ \delta)}}{\epsilon}$$
% \end{observation}

% Since LDP via shuffling protocol satisfies \cref{ass:subGaussian_noise}, application of \cref{thm:general_regret_guarantee} gives the desired regret guarantee of \cref{thm:privacy_regret_LDP_shuffle}.

\subsection{Achieving privacy via SDP}

The local randomiser $R_1(.)$ computed the noisy feature vector $x^{(n)}_t$ from the feature vector $x_t$ by adding Gaussian noise of variance $\sigma^2_1$ to each component and computes the noisy reward $r^{(n)}$ from reward $r$ by adding Gaussian noise of variance $\sigma^2_2$. The randomiser $R^{(k)}_2(.)$ adds injected Gaussian noise of variance $\sigma^2_{(k)}$ independently to every upper diagonal element of the input matrix and copies them to lower terms. %For $k=1$, the randomiser $R^{(k)}_2(.)$ adds injected Gaussian noise of variance $\sigma^2_4$ independently to every upper diagonal element of matrix $x_t x^{\top}_t$ and copies them to lower terms. 

Further, we define the noise levels 
$$\sigma_1= \frac{4\sqrt{2 \log (\frac{2.5B_k}{\delta}) \log (2/ \delta)}}{\epsilon \sqrt{B_k}}; \text{ } \sigma_{(k)} = \frac{1}{R\kappa^{*}}\sigma_2 = \frac{1}{\kappa^{*}}\sigma_1 \text{ for $k > 1$ and } \sigma_{(1)} = \frac{1}{R} \sigma_1$$.

The noise levels are chosen so that each randomiser $R_1(.)$ and $R_2(.)$ satisfy $(\epsilon/2,\delta/2)$ LDP. 



% \subsubsection{Privacy analysis}

% %Denote the size of $k^{th}$ batch by $B_k = \gT_k - \gT_{k-1}$ and define noise levels $\sigma_1 = \sigma_2 = \frac{4 \sqrt{2 \log (\frac{2.5B_k}{\delta}) \log (2/ \delta)}}{\epsilon \sqrt{B_k}}$.

% We restrict the privacy parameter $\epsilon \leq \sqrt{\frac{\log (2/ \delta)}{T}}$ and $\delta \leq 1$. Setting $\epsilon_0 = \frac{\epsilon \sqrt{B_k}}{\sqrt{\log (2/\delta)}}$ and $\delta_0 = \frac{\delta}{B_k}$, we observe that $\sigma_3 = \frac{1}{R\kappa^{*}}\sigma_1 = \sigma_2 = \frac{4\sqrt{2 \log \left(\frac{2.5}{\delta_0}\right)}}{\kappa^{*}\epsilon_0}$. 

% Now observe from Lemma \cref{lemma:multiplicative_bound} that $\frac{\dot{\mu}(x_t,\hat\theta_w)}{\beta(x_t)} \leq \dot{\mu}(x_t,\theta^{*}) \leq \frac{1}{\kappa^{*}}$. Using the standard Gaussian mechanism \cite{dworkdpbook} and boundedness, we can observe both of the local randomisers $R(.)$ is $(\epsilon_0/2,\delta_0/2)$ LDP. \footnote{While the reward vector \( r_t \) is bounded by \( R \), the vector \( x_t \) is bounded by 1, which distinguishes \( \sigma_1 \) and \( \sigma_2 \). Also the symmetric matrix $\frac{\dot{\mu}(x_t,\hat\theta_w)}{\beta(x_t)} x_t x^{\top}_t$ is bounded by $\frac{e^{2RS}}{\kappa^{*}}$. 
% } Now applying \cref{lem:shuffle_amp} and composition theorem, we can observe that the mechanism is $(\epsilon,\delta)$ SDP. 



==> lm_stochastic_context.tex <==
\section{Linear Contextual Stochastic Bandits}{\label{sec:linear_contextual_stochastic}}


We now consider the case of linear contextual bandits in which a reward $r_t$ with $\mathbb{E}[r_t|x_t] = \langle\theta^{*},x_t\rangle$ is obtained on picking arm $x_t$ from the set of arms (context vector) $\gX_t \subseteq \mathbb{R}^d$. We assume that the parameter and the arms satisfy the boundedness as \cref{ass:boundedness}. However, we stick to the case where the context set is obtained stochastically from an unknown distribution $\gD$ and we study the shuffle differential private privacy in this case. For the case of adversarial context sets, joint differential privacy has already been studied in \cite{shariff2018differentiallyprivatecontextuallinear}. Our algorithm is inspired by \cite{ruan2021linearbanditslimitedadaptivity} however, we only use the $G$ optimal design in our case, as we currently do not have an algorithm to privately compute the distributional optimal design.

\subsection{A shuffle DP algorithm for multi-armed bandits}

Our shuffle algorithm is inspired from \cite{ruan2021linearbanditslimitedadaptivity} where we define a static grid with $\mathcal{T} := \{\mathcal{T}_1,\mathcal{T}_2, \ldots, \mathcal{T}_M \} $ where $M$ denotes the total number of batches. For ease of notation, we also denote $\gB_k$ as the set of rounds in batch $k$ which consists of rounds from $\gT_{k-1}+1$ to $\gT_k$. For each batch $k$, the algorithm keeps an estimate of $\hat \theta_k$ for parameter $\theta$ based on data from that batches. When the user decides on an arm for the $k^{th}$ batch, it first performs $k-1$ eliminations based on the estimate $\hat\theta_{\kappa}$ and its confidence region for every $\kappa \in \{1,2,\ldots,k-1\}$ with confidence bounds in \cref{eq:confidence_bounds} which is a function of the term $\mLambda_{\kappa}$, a noisy estimate of $\lambda \mI + \sum_{t= \mathcal{T}_{k-1} + 1}^{\mathcal{T}_k} x_t x^{\top}_t$. The arm to play in the $t^{th}$ round is chosen by applying the $G$ optimal design to the set of survived arms. In this setup, the algorithm shares the private parameter estimate $\hat \theta_k$ (computed from previous batches) with the user at each step in $k^{th}$ batch.


\begin{align}{\label{eq:confidence_bounds}}
    & \text{UCB}_{\kappa}(x) \defeq x^T \hat{\theta}_{\kappa} + \alpha\sqrt{x^T\mLambda_\kappa^{-1}x} \text{ and,,}\\
    & \text{LCB}_{\kappa}(x) \defeq x^T \hat{\theta}_{\kappa} - \alpha\sqrt{x^T\mLambda_\kappa^{-1}x}
\end{align}

%$\alpha$ is defined and set below.

Observe that a key component of this shuffle linear stochastic contextual bandits algorithm is the instantiation of the shuffle protocol $(\gR, \gS, \gA)$ where $\gR = (R_1, R_2)$, $\gS = (S_1,S_2)$ and $\gA = (A_1,A_2)$. We present an instantiation in\cref{sec:amplification_vector_summation_sdp}. The latter is based on vector summation protocol \cite{Cheu_2019,Cheu2021ShufflePS} where each user only transmits bits corresponding to its data and also transmits additional bits for privacy noise. 

To analyze regret, we first present the following assumption on the noisy estimators of $\sum_{t} x_t x^{\top}_t + \lambda \mI$ and $\sum_t r_tx_t$. We show in \cref{sec:amplification_vector_summation_sdp} that shuffling algorithms satisfy \cref{ass:subGaussian_noise_lm} and use this assumption to bound the regret in \cref{sec:regret_analysis} while preserving privacy guarantees.



\begin{assumption}[sub-Gaussian private noise]{\label{ass:subGaussian_noise_lm}}
    There exists a constant $\tilde{\sigma}$ such that the following properties holds.
    \begin{itemize}
        \item ${\vxi}_k-\sum_{t=\mathcal{T}_{k-1}}^{\mathcal{T}_k} r_tx_t$ is a random vector with independent entries where each entry is a sub-Gaussian zero mean random variable with variance proxy $\tilde{\sigma}^2$ for every $k \in [M]$. 
        \item The matrix \({\mLambda}_k - \lambda \mI- \sum_{t=\mathcal{T}_{k-1}+1}^{\mathcal{T}_k} x_t x_t^{\top} \) is symmetric, where the upper diagonal entries are independent sub-Gaussian random variables with zero mean and a variance proxy of \( \tilde{\sigma}^2 \) for each \( k \in [M] \).

    \end{itemize}
\end{assumption}




\begin{algorithm}[t]
\caption{Shuffled DP for stochastic linear contextual bandits}
\label{alg:shuffled_linear_stochastic}
\textbf{Input} $\lambda, \alpha$ and $M$.
\begin{algorithmic}[1]
\State Initialize batches $\gB_1,\ldots,\gB_M$ with batch sizes $B_k = T^{1-2^{-k}} - T^{1-2^{-{(k-1)}}} \text{ for } k \in [M]$
% \State $\gT_0 = 0, \gT_M = T, \forall i \in [M - 1]: \gT_i = T^{1 - 2^{-i}}$; \\$\forall i \in [M]: B_i = \gT_i - \gT_{i-1}$\;
\For{$k \gets 1, 2, \dots, M$}
 % $\lambda \gets 16 \ln (2dT/\delta) + c_1 \sqrt{\frac{32}{\varepsilon} \log \left(\frac{2.5B_k}{\delta}\right) \log \left(2/\delta\right)} \left(\sqrt{d}+ 6 \sqrt{\log \left(\frac{2dKT}{\delta}\right)}\right)$\\
\For{ \text{local user } $t \gets\gT_{k - 1} + 1, \gT_{k - 1} + 2, \dots, \gT_k$}
\State Observe user's arm set ${X}_t$.
\For{$\kappa \gets 1, 2, \dots, k - 1$}
\State Update arm set $\gX_t \leftarrow \gX_t \setminus \{x \in \gX_t: \text{UCB}_\kappa(x) < \max_{y \in \gX_t} \text{LCB}_{\kappa}(y) \}$ \label{line:lm_elimination}
\EndFor
% $A_t \gets A_{t}^{(k - 1)}$\; %, \omega_{ti} \gets \omega_{ti}^{(k - 1)}, \hat r_{ti} \gets \hat r_{ti}^{(k-1)}$\;
\State Play arm $x_t \sim \pi^G(\gX_t)$, and receive reward $r_t$\;\label{line:lm_arm_select_shuffle}

\textcolor{gray}{\# For the local randomiser:}

\State Send randomised messages $M_{t,1} = R_1(r_tx_t)$ and $M_{t,2} = R_2(x_{t}x_{t}^T)$ to the local shuffler. \footnotemark
\EndFor

\textcolor{gray}{\# For the shuffler:}

\State Permute all the received messages $Y_{k,1} = S_1(\{M_{\tau,1}\}_{\gT_{k-1}+1 \leq \tau \leq \gT_{k}})$ and $Y_{k,2} = S_2(\{M_{\tau,2}\}_{\gT_{k-1} + 1 \leq \tau \leq \gT_{k}})$

%Compute batch statistics $\mLambda_k + \lambda \mI$ and $xi_k$.

\State Compute batch statistics ${\mLambda}_k = A_1 (Y_{k,2}) + \lambda \mI$ and ${\xi}_k = A_2 (Y_{k,1})$ from the received messages $Y_{k,1}$ and $Y_{k,2}$ and define $\hat{\theta}_{k} \defeq \mLambda_k^{-1}\xi_k$.
%Compute $\mLambda_k = \lambda \mI + \tilde{\mLambda}_k$ and 

%Compute parameter $\hat{\theta}_{\kappa} \defeq \mLambda_k^{-1}xi_k$
\EndFor
\end{algorithmic}
\end{algorithm}

\footnotetext{ In the shuffle protocol, we set privacy parameters to $\varepsilon/2$ and $\delta/2$ and number of users $n$ is set to $B_k$.}


%A key aspect of this shuffle protocol is given by the randomizer function $R_1(.), R_2(.)$




\subsection{Achieving privacy via vector summation protocol}\label{sec:amplification_vector_summation_sdp}

We now instantiate Algorithm \ref{alg:shuffled_linear_stochastic} with the shuffle protocol, where we rely on an efficient and accurate mechanism to sum vectors with bounded $\ell_2$ norms \cite{Cheu2021ShufflePS}. We present a formal description of the algorithm below from \cite{pmlr-v162-chowdhury22a} in Algorithms \ref{alg:Avec}, \ref{alg:Rvec} and \ref{alg:Svec}.

%This protocol operates independently on each entry of vector $r_tx_t$ and $x_tx^{\top}_t$, transmits only 0/1 bits, and the number of bits sent is sampled from a binomial distribution. This implementation has three parameters $g$ (accuracy parameter), $b \in \mathbb{N}$ and $p\in [0,1]$ where the latter two parameters control the accuracy. For an entry $x \in [0,1]$, it is first encoded as $\hat{x} = \bar{x} + \gamma_1$ where $\bar{x} = \floor{xg}$ and $\gamma_1 \sim \text{Bern}(xg - \bar{x})$. Then a binomial noise $\gamma_2 \sim \text{Bin}(b,p)$ is generated. The output of the one-dimensional randomiser is simply a collection of $g+b$ bits where $\hat x + \gamma_2$ bits are one and the rest are zero. As discussed in \cite{Cheu2021ShufflePS}, the vector is transmitted by biasing each entry by $\Delta$ \footnote{The bias term is chosen as the bound on $r_tx_t$ and $x_t x^{\top}_t$.} and then applying the mechanism described above. The shuffler shuffles the messages received from all users uniformly at random and then sums them pointwise and finally debiases it by subtracting $n\Delta$ from the sum where $n$ denotes the total number os users. 

%\sss{Read the bias part above once again.}

%Now in this analysis we set 



Further we set \begin{align}
    \lambda &= 16 \log \left({2dT}\right) + \Theta\left(\frac{ \log \left(\frac{d^2}{\delta}\right)}{\varepsilon} \right) \times\left(\sqrt{d} + 6 \sqrt{\log \left({2dKT}\right)}\right) \text{ and, } \nonumber\\
    & \hspace{ 7 em} \alpha = 80\varepsilon^{-1} \sqrt{\log \left(2dkT\right) \log (d^2/\varepsilon)}
\end{align}
%\text{ and } 

\begin{theorem}\label{thm:privacy_regret_vector_sum_shuffle}
    Set parameters $g,b$ and $p$ and parameters $\lambda,\alpha$ as defined in \cref{eq:parameters_setting_vector_summation}. Suppose $\varepsilon \leq 15$ and $\delta \leq \frac{1}{2}$ with $T> e^d$, then with probability at least $1-\delta$ we have the following guarentee on regret.

    \begin{equation}
        R^T = O\left(\frac{dRS}{\varepsilon} \sqrt{T\log \left(2dkT\right) \log (d^2/\varepsilon)} \log \log T\right)
    \end{equation}
\end{theorem}


\subsubsection{Privacy Analysis}

The privacy part of SDP follows from \cite[Theorem 3.2]{Cheu2021ShufflePS} and by adapting the parameters $g,b$ and $p$ accordingly. Thus, we can show that it satisfies $(\varepsilon,\delta)$ SDP and we can show it also satisfies JDP via \cite[Billiboard's lemma]{mechanism_design_large_games}.

\begin{lemma}[Theorem 3.2 in \cite{Cheu2021ShufflePS}]\label{lemma:subGaussian_noise}
    Choose parameters $g,b$ and $p$ as defined in \cref{eq:parameters_setting_vector_summation} in the vector summation protocol with $\varepsilon \leq 15$ and $\delta \leq \frac{1}{2}$. Then \cref{ass:subGaussian_noise_lm} holds true with $$\tilde{\sigma}^2= O\left(\frac{ R^2(\log (d^2 / \delta)) ^2 }{\varepsilon^2}\right)$$
\end{lemma}


%We can now use Theorem \ref{thm:general_regret_guarantee} to get the desired regret bound.


Since SDP via vector summation satisfies \cref{ass:subGaussian_noise_lm}, application of \cref{thm:general_regret_guarantee} gives the desired regret guarantee in \cref{thm:privacy_regret_vector_sum_shuffle}.



\subsection{Regret under Assumption \ref{ass:subGaussian_noise_lm}}{\label{sec:regret_analysis}}

We now present a framework generic regret analysis below and give a regret guarantee for any learner that estimates the parameter with noisy estimates of $\sum_{i} x_i x^{\top}_i$ and $\sum_{i} r_i x_i$ (stated formally in Defintion).








\begin{theorem}[Regret guaarantee under sub-Gaussian noise]\label{thm:general_regret_guarantee}
    Let \cref{ass:subGaussian_noise_lm} and \cref{ass:boundedness} hold with $T > e^d$. Choosing $\lambda = 16 \log (2dT) + \tilde{\sigma}_2 (\sqrt{d} + 6 \sqrt{\log (2dKT)})$ and 
    \begin{align}
    \alpha \geq & (10 + 4 S\tilde{\sigma})\sqrt{\log \left(2dKT\right)} + \sqrt{2\tilde{\sigma} (\sqrt{d} + 6 \sqrt{\log (2dKT)})} 
    \end{align}
    
    ensures the regret $R^T = O\left(d\alpha \sqrt{T} \log \log T\right)$ %with probability at least $1-\delta$.

   
\end{theorem}



Before we start proving our result, we first state the following lemma which is an adaptation of \cite[Lemma 31]{ruan2021linearbanditslimitedadaptivity}. Observe that in this term to ensure privacy, we add Gaussian noise to term $\sum_{i} y_ix_i$.



\begin{lemma}{\label{lemma:bounding_design_matrix}}
    Fix a batch $k \in [M]$ and let \cref{ass:boundedness} and \cref{ass:subGaussian_noise_lm} hold. With probability at least $(1-\frac{1}{4T^6})$, we have $\mLambda_k = \mathcal{N}_k + \sum_{t= \mathcal{T}_{k-1}+1}^{\mathcal{T}_k} x_t x^{\top}_t$ where 

    $$-4\tilde{\sigma} \left(\sqrt{d}+ 6 \sqrt{\log \left({2dMT}\right)}\right) \mI \preceq \mathcal{N}_k - \lambda \mI \preceq 4\tilde{\sigma} \left(\sqrt{d}+ 6 \sqrt{\log \left({2dMT}\right)}\right) \mI$$
\end{lemma}

\begin{proof}
     First, observe that $\mLambda_{k} = \sum_{t = \gT_{k-1}+1}^{\gT_{k}} x_t x^T_t + \gN_{k}$. From assumption \ref{ass:subGaussian_noise_lm}, $\gN_{k} - \lambda \mI$ is a symmetric matrix with upper diagonal elements being independent zero mean sub-Gaussian elements with variance-proxy  ${\sigma}^2_2$. Thus using \cite[Corollary 4.4.8]{vershynin_high-dimensional_2018}, $$\prob{||\gN_{\kappa} - \lambda \mI|| >4 \tilde{\sigma} (\sqrt{d}+ \gamma)} \leq 1/2 \exp(-\gamma^2)$$

     Now choose $\gamma = 6 \sqrt{\log \left({2dMT}\right)}$ to prove the desired result.

     %= \frac{32}{\varepsilon} \log \left(\frac{2.5B_{\kappa}}{\delta}\right) \log \left(2/\delta\right)$

\end{proof}


\begin{lemma}\label{lem:analysis-lr}
Given $\theta, x_1, x_2, \dots, x_n \in \R^d$ such that $\norm{\theta} \leq S$, for all $i \in [n]$, let $y_i = x_i^\top \theta + \varepsilon_i$ where $\varepsilon_i$ is an independent sub-Gaussian random variable with variance proxy $1$. Let $\mLambda = \mathcal{N} + \sum_{i=1}^n x_i x_i^\top$ where $\lambda_{\text{min}} \mI\preceq \mathcal{N} \preceq \lambda_{\text{max}} \mI$ and $\hat\theta = \mLambda^{-1} \left(\sum_{i=1}^n y_i x_i+ n_1\right)$ where each entry of $n_1$ is independent sub-Gaussian with variance proxy $\sigma^2$. Then we have
% $n_1 \sim \mathcal{N}(0,\sigma^2 \mI_d)$  For any $x \in \R^d$ and any $\gamma > 0$, we have that
\begin{align*}
    \prob{\abs{x^\top (\theta - \hat\theta)} > \left(\gamma + S\sqrt{\lambda_{\text{max}}} + \frac{4 \sigma (\sqrt{d} + \gamma)}{\lambda_{\text{min}}^{0.5}}\right) \sqrt{x^\top \mLambda^{-1} x}} \leq 3\exp(-\gamma^2/2).
\end{align*}
\end{lemma}


\begin{proof}
    Note that

    \begin{align}
        \left|x^{\top} \left( \theta- \hat{\theta} \right)\right| \leq &\Biggl|\sum_{i=1}^{n}x^{\top} \left(\mLambda^{-1} x_i\varepsilon_i \right) + x^{\top} \mLambda^{-1} n_1 + \nonumber\\
        & \hspace{8 em} + x^{\top} (\mLambda^{-1} (\mLambda-\mathcal{N})\theta -\theta) \Biggr|\\
        & \leq \left|\sum_{i=1}^{n}x^{\top} \mLambda^{-1} x_i\varepsilon_i \right| + \left| \lambda_{\text{max}} x^{\top} \mLambda^{-1}\theta\right| + \left|x^{\top} \mLambda^{-1}n_1\right|
    \end{align}

    Now consider the first term. Since, $x^{\top} \mLambda^{-1} x_i\varepsilon_i$ is independent sub-Gaussian for every $i$, their sum is sub-Gaussian with variance proxy $x^{\top} \mLambda^{-1} \left(\sum_i x_i x^{\top}_i \right)  \mLambda^{-1} x^{\top} \leq x^{\top} \mLambda^{-1} x^{\top}$. Thus, by sub-Gaussian concentration inequalities we have,

    \begin{equation}{\label{eq:first_term}}
        \prob{\left| \sum_{i=1}^{n} x^{\top} \mLambda^{-1}x_i \varepsilon_i\right| > \gamma \sqrt{x^{\top} \mLambda^{-1} x^{\top}}} \leq 2\exp{-\gamma^2/2}
    \end{equation}

    Now consider the second term. Since $||\theta||<S$ and $\mLambda \succeq \lambda\mI$, we have

    \begin{equation}{\label{eq:second_term}}
        |x^{\top} \mLambda^{-1}\theta| \leq S\sqrt{x^{\top} \mLambda^{-2} x} \leq S\lambda_{\text{min}}^{-0.5} \sqrt{x^{\top} \mLambda^{-1} x}
    \end{equation}

    For the third inequality we bound the norm of $n_1$. Since every entry of $n_1$ is independent Gaussian with mean $\sigma_1$, we bound its norm with high probability using \cite[Theorem 3.1.1]{vershynin_high-dimensional_2018} as $\prob{||n_1|| > 4 \sigma (\sqrt{d} + \gamma)} \leq \exp\left(-\gamma^2\right)$.
   

    Thus, with probability at least $1-\exp\left(-\gamma^2\right)$, we have 

    \begin{equation}{\label{eq:third_term}}
        |x^{\top} \mLambda^{-1}n_i| \leq |n_i| \sqrt{x^{\top} \mLambda^{-2} x} \leq  \frac{4 \sigma(\sqrt{d} + \gamma)}{\lambda_{\text{min}}^{0.5}} \sqrt{x^{\top} \mLambda^{-1}x}
    \end{equation}

    Combining \cref{eq:first_term}, \cref{eq:second_term} and \cref{eq:third_term}, we prove the desired result.
    
\end{proof}


We now prove a variant of \cite[Lemma 1]{ruan2021linearbanditslimitedadaptivity} for our setup. Observe that this result is different since the computed matrix is a noisy estimate of $\sum_{t = \mathcal{T}_{k-1}+1}^{\mathcal{T}_k} x_t x^{\top}_t$ unlike \cite[Lemma 1]{ruan2021linearbanditslimitedadaptivity}.

% {\color{red}Recall that $\alpha = 10 \sqrt{\log \left(\frac{2dKT}{\delta}\right)} + \frac{C}{\varepsilon} \frac{\sqrt{\log (2.5 B_k/ \delta) \log(2/\delta) }}{\sqrt{4 \log (2dT / \delta)}} (\sqrt{d} + \sqrt{6 \log (2dKT / \delta)}) $ It is set from previous lemma statement.}


% We can set $\alpha = 8\varepsilon^{-1}\sqrt{\log \left(\frac{2dKT}{\delta}\right)} \left(4 \sqrt{d } + \sqrt{ 6 \log (\frac{2dkT}{\delta})}\right)$.


\begin{lemma}\label{lemma:conf}
    Fix any batch $k$ and set $\alpha$ and $\lambda$ as defined in \cref{thm:general_regret_guarantee}. For each time step $t$ in batch $k$ and let $A_t$ denote the arms that survived elimination in Line \ref{line:lm_elimination}. Then with probability at least $(1-\frac{1}{T^2})$, for all $\kappa \in \{1,2,\ldots,k-1\}$ and $x \in A_t$, we have

    $$ |\langle x, \hat\theta_{\kappa} \rangle - \langle x, \theta\rangle| \leq \alpha\sqrt{x^T\mLambda_\kappa^{-1}x} $$
\end{lemma}



    % First, observe that $\mLambda_{\kappa} = \lambda \mI+ \sum_{t = \gT_{k-1}+1}^{\gT_{k}} x_t x^T_t + \gN_{\kappa}$. Observe that $\gN_{\kappa}$ is a symmetric matrix with upper diagonal elements being independent Gaussian elements with variance $\sigma^2_2B_{\kappa} = \frac{32}{\varepsilon} \log \left(\frac{2.5B_{\kappa}}{\delta}\right) \log \left(2/\delta\right)$. Thus using \cite[Corollary 4.4.8]{vershynin_high-dimensional_2018}, $$\prob{||\gN_{\kappa}|| >4 \sqrt{\frac{32}{\varepsilon} \log \left(\frac{2.5B_{\kappa}}{\delta}\right) \log \left(2/\delta\right)} (\sqrt{d}+ \gamma)} \leq 1/2 \exp(-\gamma^2)$$. 


    % Thus, $\mLambda_{\kappa} = \tilde{\lambda} + \sum_{t = \gT_{k-1}+1}^{\gT_{k}} x_t x^T_t$ with probability at least $1- \exp(-\gamma^2)$ where 
    % $$16 \log (2dT/ \delta) \leq \tilde{\lambda} \leq 16 \log (2dT/ \delta) + c_1 \sqrt{\frac{32}{\varepsilon} \log \left(\frac{2.5B_k}{\delta}\right) \log \left(2/\delta\right)} \left(\sqrt{d}+ 6 \sqrt{\log \left(\frac{2dKT}{\delta}\right)}\right)$$
    
    
    
    
    
    % Choosing $\gamma = 6 \sqrt{\log \left(\frac{2dKT}{\delta}\right)}$ and 


    
\begin{proof}   
    Applying \cref{lem:analysis-lr} and \cref{lemma:bounding_design_matrix} followed by union bounding over all stages and candidate arms to prove the lemma.
  
\end{proof}

We now state a lower bound on $\mLambda_k$ using a simple application of matrix Chernoff bound which would be used in bounding the regret.

\begin{lemma} \label{lem:exploration} 
Set $\lambda$ as defined in \cref{thm:general_regret_guarantee}. For a batch $k \in [M]$, let $\gD_k$ denote the distribution of the survived arms after $k-1$ rounds of elimination in Line \ref{line:lm_elimination}. For each batch $k$ ($k < M$), with probability $(1 - \delta/T^2)$, we have that 
\begin{align}
    \mLambda_k \succeq \frac{\gT_{k}}{16} \left(\frac{ \ln T}{ \gT_{k}} \mI + \E_{X \sim \gD_{k}} \E_{x \sim \pi^G(X)}[x x^\top]\right). \label{eq:lem-exploration}
\end{align}
\end{lemma}

To prove this lemma, we first state the following lemma from \cite[Lemma 21]{ruan2021linearbanditslimitedadaptivity}.

\begin{lemma}\label{lemma:matrix_concentration}
    Suppose $x_1,x_2,\ldots,x_n$ are drawn i.i.d from a distribution $\gD$ and $|| x_i || \leq 1 \forall i \in [n]$ almost surely. For any cutoff level $\lambda$, with probability at least $(1-2d\exp(-\lambda n/8))$, we have that

    $$3 \lambda \mI + \frac{1}{n} \sum_{i=1}^{n} x_i x^{\top}_i \succeq \frac{1}{8} \mathbb{E}_{x \sim \gD} xx^{\top}$$
\end{lemma}

The proof of \cref{lem:exploration} follows on application of \cref{lemma:matrix_concentration} and \cref{lem:exploration}. 


We now prove \cref{thm:general_regret_guarantee} which directly follows from \cite[Section 4.1]{ruan2021linearbanditslimitedadaptivity}. We restate the proof below for exposition.




==> problem_setup.tex <==
\section{Notation and Preliminaries}{\label{sec:notations_and_prelims}}
A policy $\pi$ is a function that maps any given arm set $\mathcal{X}$ to a probability distribution over the same set, i.e., 
$\pi(\mathcal{X}) \in \Delta(\mathcal{X})$, where $\Delta(\mathcal{X})$ is the probability simplex supported on $\mathcal{X}$. We will denote matrices in bold upper case (e.g., $\mathbf{M}$). $\|x\|$ denotes the $\ell_2$ norm of vector $x$. We write $\|x\|_{\mathbf{M}}$ to denote $\sqrt{x^\top \mathbf{M} x}$ for a positive semi-definite matrix $\mathbf{M}$ and vector $x$. For any two real numbers $a$ and $b$, we denote by $a \wedge b$ the minimum of $a$ and $b$. Throughout, $\widetilde{O}(\cdot)$ denotes big-$O$ notation but suppresses log factors in all relevant parameters. For $m, n \in \mathbb{N}$ with $m < n$, we denote the set $\{1, \ldots, n\}$ by $[n]$ and $\{m, \ldots, n\}$ by $[m, n]$.

\begin{definition}{\label{def:glm}}
    A generalized linear model (GLM) with parameter vector $\theta^{*} \in \mathbb{R}^d$ is a real valued random variable $r$ that belongs to the exponential family of distribution with density function
    $$P(r \mid x) = \exp(r.\langle x,\theta^{*}\rangle - b\left(\langle x,\theta^{*}\rangle\right) + c(r)) $$

    Function $b(.)$ (called the log-partition function) is assumed to be twice differentiable and $\dot{b}$ is assumed to be monotone. Further, we assume $r \in [0,R]$ and $|\theta^{*}| \leq S$. 
\end{definition}
Important properties of GLM such as $\mathbb{E}[r] = \dot{b}\left(\langle x,\theta^{*}\rangle\right)$ and $\text{Var}(r) = \ddot{b}\left(\langle x,\theta^{*}\rangle\right)$. Further, we define $\mu\left(\langle x,\theta^{*}\rangle\right) = \dot{b}\left(\langle x,\theta^{*}\rangle\right)$ as the link function. 
Next we describe the two contextual bandit (CB) problems with generalized linear model (GLM) rewards that we address in this paper. Let $T \in \mathbb{N}$ be the total number of rounds. At each round $t \in [T]$, we receive an arm set $\gX_t \subset \mathbb{R}^d$ with number of arms $K = |\gX_t|$, and must select an arm $x_t \in \gX_t$. Following this selection, we receive a reward $r_t$ sampled from the GLM distribution $P(r|x)$ with unknown parameter $\theta^*$.


% We now state a lemma from \cite[Lemma 2.2]{sawarni2024generalizedlinearbanditslimited} with additional properties of GLMs in \cref{sec:appendix_glm_properties}


% \begin{proposition}[Self-Concordance]{\label{lemma:self_concordance_multiplicative}}
%     For any GLM supported on $[0,R]$ almost surely, the link function $\mu(.)$ satisfies $||\ddot{\mu}(z)|| \leq R\dot{\mu}(z)$ for all $z \in \mathbb{R}$ and $\frac{\dot{\mu}(z_2)}{\exp(R|z_1-z_2|)} \leq \dot{\mu}(z_1) \leq \dot{\mu}(z_2)\exp(R|z_1-z_2|)$ for any $z_1,z_2 \in \mathbb{R}$. 
% \end{proposition}



\textbf{Problem 1}:  In this setting $\mone$, we assume that at each round $t$, the context set $\gX_t \subseteq \mathbb{R}^d$ is drawn from an unknown
distribution $\gD$. Further, the apriori algorithm decides the lengths of each batch where the policy remains the same within each batch and updates the policy only at the start of each batch. We study $(\varepsilon,\delta)$ multi-rounded shuffled differential privacy in this setup and the goal is to minimise the expected cumulative regret as defined below.

\begin{equation}{\label{eq:cumulative_regret_setupone}}
    R_T = \mathbb{E}\left[\sum_{t=1}^T \max_{x \in \gX_t} \mu(\langle x, \theta^* \rangle) - \sum_{t=1}^T \mu(\langle x_t, \theta^* \rangle)\right]
\end{equation}

Here the expectation is taken over the randomness of the algorithm, the distribution of rewards $r_t$, and the distribution of the arm set $\gD$.


\textbf{Problem 2}: In this problem, we do not make any assumptions on the context set $\gX_t$ i.e. the context sets can be adversarially chosen. The goal in this setup $\mtwo$ is to minimise the cumlative regret while satisfying $(\varepsilon,\delta)$ joint differential privacy. Formally, the cumulative regret is defined as 

\begin{equation}{\label{eq:cumulative_regret_setuptwo}}
    R_T = \sum_{t=1}^T \max_{x \in \gX_t} \mu(\langle x, \theta^* \rangle) - \sum_{t=1}^T \mu(\langle x_t, \theta^* \rangle)
\end{equation}

Finally, for both problems, the Maximum Likelihood Estimator (MLE) of $\theta^*$ is obtained by minimizing the cumulative log-loss. For any arm $x$, reward $r$, and parameter $\theta \in \mathbb{R}^d$, define
$\ell(\theta, x, r) := -r \cdot \langle x, \theta \rangle + \int_0^{\langle x, \theta \rangle} \mu(z)\,dz$.
After $t$ rounds, we write the regularized objective as
\[
\gL_t(\theta;\lambda) := \sum_{s=1}^t \ell(\theta, x_s, r_s) + \frac{\lambda}{2}\|\theta\|_2^2,
\]
where $\lambda > 0$ is the regularization parameter, and estimate
$\widehat{\theta}_t = \argmin_{\theta} \gL_t(\theta;\lambda)$.

\subsection{Instance dependent non-linear parameters}{\label{sec:instance_dependent_non_linear}}

Following the prior works in \cite{faury2020improvedoptimisticalgorithmslogistic,faury2022jointlyefficientoptimalalgorithms,sawarni2024generalizedlinearbanditslimited}, we define instance-dependent parameters that capture the non-linearity of the problem design that impacts our design and analysis of \Cref{alg:shuffled_glm} in setup $\mone$. For any arm set $\gX$, write optimal arm $x^{*} = \argmax_{x \in \mathcal{X}} \mu\left(\langle x, \theta^{*}\rangle\right)$ and define,
\begin{align}{\label{eq:kapa_kappa_hat_mone}}
     \kappa := \max_{\mathcal{X} \in \supp(\mathcal{D})} \max_{x \in \mathcal{X}} \frac{1}{\dot{\mu}\left(\langle x, \theta^{*}\rangle\right)}, \text{ }  & \frac{1}{\hat \kappa} = \mathbb{E}_{\mathcal{X} \sim \mathcal{D}} \left[\dot{\mu} \left( \langle x^{*},\theta^{*} \rangle\right)\right]  \text{ } \nonumber\\ & \hspace{-6 em} 1/\kappa^{*} := \max_{\mathcal{X} \in \supp(\gD)} \max_{x \in \mathcal{X}} {\dot{\mu}\left(\langle x, \theta^{*}\rangle\right)}%\footnote{ \text{Observe that $\kappa^{*}, \frac{1}{\kappa} \leq R$}}
 \end{align}

 %
Under \Cref{alg:jdp_glm_adversarial} in setup $\mtwo$, we redefine non-linear parameter $\kappa$ and $\kappa^{*}$ as 
\begin{equation}{\label{eq:kapa_mtwo}}
    \kappa := \max_{x \in \cup_{t \in [T]} \mathcal{X}_t} \frac{1}{\dot{\mu}\left(\langle x, \theta^{*}\rangle\right)}, \text{ } 1/\kappa^{*} = \max_{x \in \cup_{t \in [T]} \mathcal{X}_t} {\dot{\mu}\left(\langle x, \theta^{*}\rangle\right)}
\end{equation}
Note that $\hat \kappa \geq \kappa^{*}$. Similar to the non-private bound in \cite{sawarni2024generalizedlinearbanditslimited}, out works also do not have any $\kappa$ dependence in the most dominant term $\tilde{O}(\sqrt T)$ is the regret expression. In practice, it is unrealistic to assume that the algorithm has exact knowledge of these parameters; however, it suffices to have access to an upper bound on $\kappa$ and lower bounds on $\hat{\kappa}$ and $\kappa^{*}$. We make the following boundedness assumption that is common in contextual bandits \cite{ruan2021linearbanditslimitedadaptivity, NIPS2011_e1d5be1c}.

\begin{assumption}[Boundedness]{\label{ass:boundedness}}
    The magnitude of the reward $r_t$ at each time step $t$ is bounded by some known constant $R$. Also, the every context vector arm at each time step has its $\ell_2$ norm bounded by 1 i.e. $||x||_2 < 1$ for every $x \in \gX_t$ and time step $t$. Further, the unknown parameter vector $\theta^{*}$ has its $\ell_2$ norm bounded by some known constant $S$. \footnote{$||x||_2$ denotes the $\ell_2$ norm of $x \in \mathbb{R}^d$. }
\end{assumption}

\subsection{Optimal design}

In the stochastic‐context regime, the batches are determined ahead of time. Previous work has leveraged G‐optimal design to construct policies for both linear reward settings \cite{ruan2021linearbanditslimitedadaptivity} and generalized linear reward settings \cite{sawarni2024generalizedlinearbanditslimited}. For completeness, we now restate the fundamental lemma on G‐optimal design, which follows directly from the General Equivalence Theorem of \cite{Kiefer_Wolfowitz_1960}.
\begin{lemma}[\cite{ruan2021linearbanditslimitedadaptivity}] For any subset $\gX \subseteq \R^d$, there exists a distribution $\gK_\gX$ supported on $\gX$, such that for any $\varepsilon > 0$, it holds that 
\begin{align}
\max_{x \in \gX} x^\top \left(\varepsilon \mI + \E_{y \sim \gK_\gX} y y^\top \right)^{-1} x \leq d . \label{eq:thm-KW}
\end{align}
Furthermore, if $\gX$ is a discrete set with finite cardinality, one can find a distribution such that the right-hand side of \Cref{eq:thm-KW} is relaxed to $2d$ in time  $\mathrm{poly}(\abs{\gX})$.
\end{lemma}


While the algorithms in \cite{ruan2021linearbanditslimitedadaptivity,sawarni2024generalizedlinearbanditslimited} use distributional optimal design, we refrain from doing so as we are unable to compute it with differential privacy constraints. We thus stick to $G$-optimal designs which leads to an additional multiplicative factor of $\sqrt d$ in the leading term.
 

% In the linear contextual bandit problem \cite{NIPS2011_e1d5be1c,ruan2021linearbanditslimitedadaptivity}, the mean reward is some unknown linear function of the selected arm i.e. $\mathbb{E}[r_t] = \langle \theta^{*},x_t \rangle$ for some unknown $\theta^{*} \in \mathbb{R}^d$ where $\langle .,. \rangle$ denotes the Euclidean inner product. The agent's performance is measured with respect to the expected cumulative regret where the regret at each time step $t$ is defined as the difference between the maximum expected reward at time step $t$ and the reward from the played arm $x_t$. Formally, 
% \begin{align}
% R^T \defeq \E\left[\sum_{t = 1}^T \max_{x \in \gX_t} x^\top \theta - x_t^\top \theta\right], \label{eq:regret}
% \end{align}

% where the expectation is taken over $\mathcal{D}$, the noises, and the internal randomness of the learner. We make standard assumptions of boundedness on the rewards and the parameter vector $\theta^{*}$ that is common in the contextual bandit literature \cite{NIPS2011_e1d5be1c,diffpivacylinearbandits,pmlr-v162-chowdhury22a,ruan2021linearbanditslimitedadaptivity}.

==> sco_old.tex <==
\section{Private optimization algorithms )}\label{sec:shuffle_convex_optimizer}

    We now describe the shuffle convex optimizer $\mathcal{P}_{GD}$ which in turn uses the vector summation  protocols $(\gR_{\text{Vec}}, \gS_{\text{Vec}}, \gA_{\text{Vec}})$. Before, we present the algorithm we first define Lipschitz ness and convexity of $\ell (\theta,r,x) $ w.r.t $\theta$ in $\Theta$.


    \begin{definition}
        Loss function $\ell : \Theta \times X \rightarrow \mathbb{R}$ is convex in $\Theta$ if, for all $x \in X$, for all $t \in [0, 1]$ and $\theta, \theta' \in \Theta$, $\ell(t\theta + (1 - t)\theta', x) \leq t\ell(\theta, x) + (1 - t)\ell(\theta', x)$. $\ell$ is $L$-Lipschitz in $\Theta$ if for all $x \in X$ and $\theta, \theta' \in \Theta$, $|\ell(\theta, x) - \ell(\theta', x)| \leq L\|\theta - \theta'\|_2$
    \end{definition}

  Further, for a dataset $\gD= \{x_i\}_{i=1}^n$, we define $\ell(\theta,\gD) = \frac{1}{n} \sum_{i=1}^{n} \ell(\theta,x_i)$

    %Thus, the loss function $\ell (\theta,r,x) = -r\langle x,\theta\rangle + b \left(\langle x, \theta \right)$ is convex in $\theta$. It is also $2RS$ Lipschitz as $\dot{b} \left(\langle x, \theta\rangle\right) = \mu\left(\langle x, \theta\rangle\right) \leq R$. Also recall that 

 

    


    


    \begin{algorithm}
\caption{$\mathcal{P}_{\text{GD}}$, Multi-rounded shuffle private gradient descent \cite{Cheu2021ShufflePS}}\label{alg:shuffle_convex_optimizer}
\textbf{Require:} Data points $\{(x_i)\}_{i=1}^{n}$, privacy parameters $\varepsilon$, $\delta$, pointwise loss function $\ell(.)$ with Lipschitz parameter $L$, convex set $\Theta$.

Set number of iterations $T = \frac{\epsilon^2 n^2}{ d \log^3(nd/\delta)}$, step size $\eta = \frac{2D}{L \sqrt T}$ 
\begin{algorithmic}[1]
\State Initialize parameter estimate $\theta_0 \leftarrow 0$
\For{ $t = 1, 2, \ldots, T$} 
\State Compute the gradient at $\theta_t$, $\bar{g}_t \leftarrow \frac{1}{n} P_1\left(\nabla_\theta\ell(\theta_t, x_1), \cdots, \nabla_\theta\ell(\theta_t, x_n); \frac{\varepsilon}{2\sqrt{2T\log(1/\delta)}}, \frac{\delta}{T+1}, L\right)$ \text{where} ${P}_{1} = A_{1}\circ S_{1} \circ R_{1}$
\State Compute and store the parameter $\theta_{t+1} \leftarrow \pi_\Theta(\theta_t - \eta\bar{g}_t)$
\EndFor
\State \Return final estimate $\bar{\theta} \leftarrow \frac{1}{T}\sum_{t=0}^{T-1} \theta_t$
\end{algorithmic}
\end{algorithm}


We now have the following utility and privacy guarantee from Lemma B.4 of \citet{Cheu2021ShufflePS}. While the privacy guarantee directly follows, we reprove the utility guarantee along the lines of Theorem 3.2 of \citet{convexoptimizationbubeck} as we present a high probability guarantee instead of one in expectation.

\begin{lemma}\label{lemma:utility_shuffle_convex}
    The protocol $\mathcal{P}_{\text{GD}}$ is multi-rounded $(\epsilon,\delta)$ shuffle DP. Suppose $\ell$ is convex and $L-$ lipschitz over a convex set $\Theta \in \mathbb{R}^d$ over a diameter $D$. For any set of data-points $\gD = \{x_i\}_{i=1}^{n}$ and $\eta>0$, the output of the protocol $\mathcal{P}_{GD}$ satisfies \footnote{This follows from the substitution of the noise parameter $\sigma$ in Lemma B.4 of \citet{Cheu2021ShufflePS} with probability at least $1-\zeta$.}

    %    \sss{In lemma B.4 expectation was invoked here we invoke high probability add extra log term}

    $$\ell (\bar \theta,\gD) - \min_{\theta \in \Theta} \ell(\theta,\gD) \leq \frac{D^2}{2\eta T} + \frac{\eta L^2}{2} + O\left(\frac{\eta d TL^2 \log^2 (d^2 T/\delta)}{2n^2\epsilon^2}\right) + \eta \log (1/\zeta) \sqrt{dL^2} O\left(\sqrt{\frac{L^2 \log^2 (d^2 T/\delta)}{2n^2T\epsilon^2}}\right)$$

    Choosing $T= \frac{\epsilon^2 n^2}{ d \log ^3 (nd/\delta)}$ and $\eta = \frac{D}{L\sqrt{T}}$, the bound evaluates to 

    \begin{equation}
        \ell (\bar \theta,\gD) - \min_{\theta \in \Theta} \ell(\theta,\gD) \leq O\left(\frac{DL}{\epsilon n} \sqrt{d\log^3(dn/\delta)}\right)
    \end{equation}
\end{lemma}

\begin{proof}
    Let $g_t$ denote the actual gradient at each step $t$ and $\overline{g}_t$ denotes the computed gradient. Further, let $\alpha_{t+1}$ denote $\theta_t - \eta \overline{g}_t$ for every step $t \in [T]$. We also denote $\theta^{\ast}_\gD$ as the minimizer of $\ell(.,\gD)$. Now, drawing from the proof in Theorem 3.2 of \citet{convexoptimizationbubeck}, we have

    \begin{align}
        \ell(\theta_t,\gD) - \ell(\theta^{\ast}_\gD,\gD) \leq & \frac{1}{2\eta} \left(||\theta_t -\theta^{\ast}||^2_2 - ||\alpha_{t+1} - \theta^{\ast}||^2_2\right) + \frac{\eta}{2} || \overline{g}_t||^2_2 \nonumber%\\
        %\leq & \frac{1}{2\eta} \left(||\theta_t -\theta^{\ast}||_2 - ||\alpha_{t+1} - \theta^{\ast}||_2\right) + \frac{\eta}{2} || {g}_t||^2_2 + O \left(\frac{\eta dT L^2 \log^2 (d/\delta) \log (1/\zeta)}{n^2\epsilon^2}\right) \text{ w.p. at least $1-\zeta$} \label{eq:temp_appendix_e}. 
    \end{align}

    Denote $n_t = \overline{g}_t - g_t$. Now every component of $n_t$ is coordinate wise independent and also zero mean sub-Gaussian with variable with variance proxy $O\left(\frac{T L^2 \log^2 (d^2 T/\delta)}{2n^2\epsilon^2}\right)$ from \cref{lemma:utility_privacy_vector_summation_protocol}.

    


    

    %The last step follows from the fact that $\overline{g}_t - g_t$ is a coordinate wise zero mean Sub-Gaussian random variable with variance proxy $O\left(\frac{\eta T L^2 \log^2 (d^2 T/\delta)}{2n\epsilon^2}\right)$. We finally get the high probability bound invoking lemma \ref{lemma:square_subGaussian}.

    Now using $|| g_t|| <L $ and the fact that $||\alpha_{t+1} - \theta^{\ast}_S|| \leq || \theta_{t+1} - \theta^{\ast}_S||$ from Lemma 3.1 of \citet{convexoptimizationbubeck}, we have

    \begin{align}{\label{eq:eq:temp_2_last_lemma}}
        \ell(\bar \theta,\gD) - \ell(\theta^{\ast}_\gD,\gD) \overset{(a)} \leq & \frac{1}{T} \sum_{t=1}^{T} \left(\ell(\bar \theta_t,\gD) - \ell(\theta^{\ast}_\gD,\gD)\right) \nonumber\\
        {\leq} & \frac{D^2}{2\eta T} + \frac{\eta}{2T} \sum_{t=1}^{T}||{g}_t||^2_2 + \sum_{i=1}^{d} \left(\frac{\eta}{T} \sum_{t=1}^{T} g_{t,i} n_{t,i}\right) + \frac{\eta}{2T} \sum_{i=1}^{T} ||n_t||^2_2
        % \overset{(c)}{\leq} & \frac{D^2}{2\eta T} + \frac{\eta L^2}{2} + O \left(\frac{\eta dT L^2 \log^2 (d/\delta) \log (1/\zeta)}{n^2\epsilon^2}\right) \text{ w.p at least $1- \zeta$.}
    \end{align}

    $(a)$ follows from the the convexity of the loss function $\ell$ and 
    % $(b)$ follows since $||\alpha_{t+1} - \theta^{\ast}_S|| \leq || \theta_{t+1} - \theta^{\ast}_S||$ from the proof of \cite[Lemma 3.1]{convexoptimizationbubeck}.
    
    % \begin{itemize}
    %     \item $||\alpha_{t+1} - \theta^{\ast}_S|| \leq || \theta_{t+1} - \theta^{\ast}_S||$ from the proof of \cite[Lemma 3.1]{convexoptimizationbubeck}.
    %     \item Observe that $\frac{1}{T}\sum\limits_{t=1}^{T} g_{t,i} n_{t,i}$ is zero mean sub-Gaussian with variance proxy $ \sum_{i=1}^{d} g^2_{t,i} O\left(\frac{\eta T L^2 \log^2 (d^2 T/\delta)}{2n\epsilon^2}\right)$. Thus, with probability $1-\zeta/n$, an upper bound 
    % \end{itemize} 

    Since, $\frac{1}{T}\sum\limits_{i=1}^d \sum\limits_{t=1}^{T} g_{t,i} n_{t,i}$ is zero mean sub-Gaussian with variance proxy $ \sum_{t=1}^{T} g^2_{t,i} O\left(\frac{L^2 \log^2 (d^2 T/\delta)}{2n^2T^2\epsilon^2}\right)$, we have

    \begin{align}{\label{eq:temp_1_last_lemma}}
        \sum_{i=1}^{d} \left(\frac{\eta}{T} \sum_{t=1}^{T} g_{t,i} n_{t,i}\right) \leq & \eta \log (1/\zeta)\sqrt{\sum_{i=1}^d \sum_{t=1}^{T} g^2_{t,i}} O\left(\sqrt{\frac{ L^2 \log^2 (d^2 T/\delta)}{2n^2T\epsilon^2}}\right) \text{ w.p. } 1-\zeta/2 \nonumber\\
        \leq & \eta  \log (1/\zeta) \sqrt{dL^2T} O\left(\sqrt{\frac{L^2 \log^2 (d^2 T/\delta)}{2n^2T^2\epsilon^2}}\right) = \eta  \log (1/\zeta) \sqrt{dL^2} O\left(\sqrt{\frac{L^2 \log^2 (d^2 T/\delta)}{2n^2T\epsilon^2}}\right)
    \end{align}


    From \cref{lemma:square_subGaussian}, $\frac{1}{T}\sum\limits_{i=1}^{d}\sum\limits_{t=1}^{T} n^2_{t,i} = O\left(\frac{dTL^2 \log^2 (d^2 T/\delta)}{2n^2\epsilon^2}\right) + O\left(\frac{dTL^2 \log^2 (d^2 T/\delta)}{2n^{2.5}\epsilon^2} \sqrt{\log (1/\zeta)}\right)$  with probability at least $1-\zeta/2$.


    Thus, from \cref{eq:temp_1_last_lemma} and \cref{eq:eq:temp_2_last_lemma}, with probability $1-\zeta$ we have

    \begin{equation}
        \ell(\bar \theta,\gD) - \ell(\theta^{\ast}_\gD,\gD) \leq \frac{D^2}{2\eta T} + \frac{\eta L^2}{2} + O\left(\frac{\eta d TL^2 \log^2 (d^2 T/\delta)}{2n^2\epsilon^2}\right) + \eta \log (2T/\zeta) \sqrt{dL^2} O\left(\sqrt{\frac{L^2 \log^2 (d^2 T/\delta)}{2n^2T\epsilon^2}}\right) 
    \end{equation}

%    \sss{check why in albert chey paper they have $\log^3$ while we have $\log^2$}

\end{proof}

We now present the analysis for the full batch DP-SGD optimizer  proving a guarantee in terms of zero-CDP \cite{cryptoeprint:concentratedDP} which gives us better composition guarantees without any assumptions on the total privacy budget $\varepsilon$ being small.


\begin{lemma}[Noisy full-batch PGD under zCDP]
    Suppose $\ell(\cdot,\gD)$ is convex and $L$-Lipschitz over a closed convex set
    $\Theta \subset \mathbb{R}^d$ of diameter $D$. Let
    $\theta^\ast_\gD \in \arg\min_{\theta \in \Theta} \ell(\theta,\gD)$.
    Consider full-batch projected gradient descent with Gaussian perturbations:
    \[
        \theta_{t+1}
        =
        \Pi_{\Theta}\bigl(\theta_t-\eta(g_t+n_t)\bigr),
        \qquad
        g_t \in \partial \ell(\theta_t,\gD),
    \]
    where $n_t \sim \mathcal{N}(0,\sigma^2 I_d)$ independently across
    $t \in [T]$, and $\sigma^2= \frac{2L^2T}{n^2\rho}$
    Under replacement adjacency, the sequence of $T$ noisy gradients is
    $\rho$-zCDP. Moreover, with probability at least $1-\zeta$,
    the averaged iterate $\bar\theta = \frac1T\sum_{t=1}^T \theta_t$ satisfies
    \[
        \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
        \leq
        \frac{D^2}{2\eta T}
        +
        \frac{\eta L^2}{2}
        +
        O\left(
            \eta d\sigma^2
            +
            \frac{D\sigma\sqrt{\log(1/\zeta)}}{\sqrt{T}}
        \right).
    \]
    In particular, choosing $\eta = \frac{D}{L\sqrt{T}}$ and
    $T = \frac{\rho n^2}{d}$ gives
    \[
        \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
        \leq
        O\left(
            \frac{DL\sqrt d}{n\sqrt{\rho}}
        \right)
    \]
    with probability at least $1-\zeta$, up to logarithmic factors.
\end{lemma}

\begin{proof}
    Let $\bar g_t = g_t+n_t$ denote the noisy full-batch gradient. Since
    $\ell(\cdot,\gD)$ is convex,
    \[
        \ell(\theta_t,\gD)-\ell(\theta^\ast_\gD,\gD)
        \leq
        \langle g_t,\theta_t-\theta^\ast_\gD\rangle
        =
        \langle \bar g_t,\theta_t-\theta^\ast_\gD\rangle
        -
        \langle n_t,\theta_t-\theta^\ast_\gD\rangle .
    \]
    By the standard projected-gradient descent inequality,
    \[
        \langle \bar g_t,\theta_t-\theta^\ast_\gD\rangle
        \leq
        \frac{1}{2\eta}
        \left(
            \|\theta_t-\theta^\ast_\gD\|_2^2
            -
            \|\theta_{t+1}-\theta^\ast_\gD\|_2^2
        \right)
        +
        \frac{\eta}{2}\|\bar g_t\|_2^2 .
    \]
    Therefore,
    \[
        \ell(\theta_t,\gD)-\ell(\theta^\ast_\gD,\gD)
        \leq
        \frac{1}{2\eta}
        \left(
            \|\theta_t-\theta^\ast_\gD\|_2^2
            -
            \|\theta_{t+1}-\theta^\ast_\gD\|_2^2
        \right)
        +
        \frac{\eta}{2}\|g_t+n_t\|_2^2
        -
        \langle n_t,\theta_t-\theta^\ast_\gD\rangle .
    \]
    Averaging over $t=1,\dots,T$ and using convexity of $\ell$ gives
    \[
        \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
        \leq
        \frac{D^2}{2\eta T}
        +
        \frac{\eta}{2T}\sum_{t=1}^T \|g_t+n_t\|_2^2
        -
        \frac1T\sum_{t=1}^T
        \langle n_t,\theta_t-\theta^\ast_\gD\rangle .
    \]
    Since $\|g_t\|_2 \leq L$, standard Gaussian concentration implies
    \[
        \frac1T\sum_{t=1}^T \|g_t+n_t\|_2^2
        \leq
        O(L^2+d\sigma^2)
    \]
    with high probability. Moreover, conditional on the past,
    $\langle n_t,\theta_t-\theta^\ast_\gD\rangle$ is mean-zero Gaussian
    with variance at most $D^2\sigma^2$, since
    $\|\theta_t-\theta^\ast_\gD\|_2 \leq D$. Hence,
    \[
        \left|
        \frac1T\sum_{t=1}^T
        \langle n_t,\theta_t-\theta^\ast_\gD\rangle
        \right|
        \leq
        O\left(
            \frac{D\sigma\sqrt{\log(1/\zeta)}}{\sqrt T}
        \right)
    \]
    with probability at least $1-\zeta$. Combining these bounds yields
    \[
        \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
        \leq
        \frac{D^2}{2\eta T}
        +
        \frac{\eta L^2}{2}
        +
        O\left(
            \eta d\sigma^2
            +
            \frac{D\sigma\sqrt{\log(1/\zeta)}}{\sqrt T}
        \right).
    \]

    Finally, under replacement adjacency, the full-batch gradient has
    $\ell_2$-sensitivity at most $2L/n$. A Gaussian mechanism with sensitivity
    $2L/n$ and noise variance $\sigma^2$ is
    $\frac{2L^2}{n^2\sigma^2}$-zCDP per iteration. By composition over $T$
    iterations, the total privacy cost is
    \[
        T \cdot \frac{2L^2}{n^2\sigma^2}.
    \]
    Setting
    \[
        \sigma^2 = \frac{2L^2T}{n^2\rho}
    \]
    makes the entire optimizer $\rho$-zCDP.
\end{proof}

==> sco_old2.tex <==
\section{Private optimization algorithms}\label{sec:shuffle_convex_optimizer}

We now describe the shuffle convex optimizer $\mathcal{P}_{GD}$, which uses the vector summation protocols $(\gR_{\text{Vec}}, \gS_{\text{Vec}}, \gA_{\text{Vec}})$. Before presenting the algorithm, we first define convexity and Lipschitzness of the loss function with respect to $\theta$ over $\Theta$.

\begin{definition}
    A loss function $\ell : \Theta \times X \rightarrow \mathbb{R}$ is convex in $\Theta$ if, for all $x \in X$, all $t \in [0,1]$, and all $\theta,\theta' \in \Theta$,
    \[
        \ell(t\theta+(1-t)\theta',x)
        \leq
        t\ell(\theta,x)+(1-t)\ell(\theta',x).
    \]
    It is $L$-Lipschitz in $\Theta$ if, for all $x \in X$ and all $\theta,\theta' \in \Theta$,
    \[
        |\ell(\theta,x)-\ell(\theta',x)|
        \leq
        L\|\theta-\theta'\|_2 .
    \]
\end{definition}

For a dataset $\gD=\{x_i\}_{i=1}^n$, define the empirical loss
\[
    \ell(\theta,\gD)
    =
    \frac1n\sum_{i=1}^n \ell(\theta,x_i).
\]

\begin{algorithm}
\caption{$\mathcal{P}_{\text{GD}}$, multi-round shuffle-private gradient descent \cite{Cheu2021ShufflePS}}
\label{alg:shuffle_convex_optimizer}
\textbf{Require:} Data points $\{x_i\}_{i=1}^{n}$, privacy parameters $\varepsilon,\delta$, pointwise loss function $\ell(\cdot)$ with Lipschitz parameter $L$, convex set $\Theta$.

Set the number of iterations $T = \frac{\varepsilon^2 n^2}{d\log^3(nd/\delta)}$ and step size $\eta = \frac{2D}{L\sqrt T}$
\begin{algorithmic}[1]
\State Initialize parameter estimate $\theta_0 \leftarrow 0$.
\For{$t = 0,1,\ldots,T-1$}
    \State Compute the noisy full-batch gradient
    \[
        \bar g_t
        \leftarrow
        \frac1n P_1\left(
            \nabla_\theta \ell(\theta_t,x_1),\ldots,
            \nabla_\theta \ell(\theta_t,x_n);
            \frac{\varepsilon}{2\sqrt{2T\log(1/\delta)}},
            \frac{\delta}{T+1},
            L
        \right),
    \]
    where $P_1=A_1\circ S_1\circ R_1$.
    \State Compute and store the parameter
    \[
        \theta_{t+1} \leftarrow \pi_\Theta(\theta_t-\eta \bar g_t).
    \]
\EndFor
\State \Return final estimate $\bar\theta \leftarrow \frac1T\sum_{t=0}^{T-1}\theta_t$.
\end{algorithmic}
\end{algorithm}

The following lemma is included only for completeness. It is a standard utility analysis for projected gradient descent with noisy gradients, following the usual projected-gradient descent proof of \citet{convexoptimizationbubeck}. Our contribution is not the optimization analysis itself, but its use inside the private optimization subroutine required by our algorithm.

\begin{lemma}[Utility of noisy projected gradient descent]
\label{lemma:noisy_pgd_generic}
Suppose $\ell(\cdot,\gD)$ is convex and $L$-Lipschitz over a closed convex set $\Theta \subset \mathbb{R}^d$ of diameter $D$. Let
\[
    \theta^\ast_\gD \in \arg\min_{\theta\in\Theta}\ell(\theta,\gD).
\]
Consider the noisy projected-gradient update
\[
    \theta_{t+1}
    =
    \pi_\Theta(\theta_t-\eta\bar g_t),
    \qquad
    \bar g_t=g_t+n_t,
    \qquad
    g_t\in \partial \ell(\theta_t,\gD),
\]
for $t=0,\ldots,T-1$, where $n_t$ is the noise added to the gradient at round $t$. Let
\[
    \bar\theta=\frac1T\sum_{t=0}^{T-1}\theta_t.
\]
Assume that, with probability at least $1-\zeta$, the noise sequence satisfies
\[
    \frac1T\sum_{t=0}^{T-1}\|n_t\|_2^2 \leq B_2
\]
and
\[
    \left|
    \frac1T\sum_{t=0}^{T-1}
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle
    \right|
    \leq B_1.
\]
Then, with probability at least $1-\zeta$,
\[
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    \frac{D^2}{2\eta T}
    +
    \eta L^2
    +
    \eta B_2
    +
    B_1.
\]
\end{lemma}

\begin{proof}
Since $\ell(\cdot,\gD)$ is convex and $g_t\in \partial \ell(\theta_t,\gD)$, the subgradient inequality gives
\[
    \ell(\theta_t,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    \langle g_t,\theta_t-\theta^\ast_\gD\rangle.
\]
Since $\bar g_t=g_t+n_t$, equivalently $g_t=\bar g_t-n_t$. Therefore,
\[
    \langle g_t,\theta_t-\theta^\ast_\gD\rangle
    =
    \langle \bar g_t,\theta_t-\theta^\ast_\gD\rangle
    -
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle.
\]
Combining the previous two displays gives
\[
    \ell(\theta_t,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    \langle \bar g_t,\theta_t-\theta^\ast_\gD\rangle
    -
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle.
\]

We next bound the first inner product. Define
\[
    \alpha_{t+1}=\theta_t-\eta\bar g_t.
\]
Then
\[
    \theta_{t+1}=\pi_\Theta(\alpha_{t+1})
\]
and
\[
    \eta\bar g_t=\theta_t-\alpha_{t+1}.
\]
Thus,
\[
    \langle \bar g_t,\theta_t-\theta^\ast_\gD\rangle
    =
    \frac1\eta
    \langle \theta_t-\alpha_{t+1},\theta_t-\theta^\ast_\gD\rangle.
\]
Using the identity
\[
    2\langle a-b,a-c\rangle
    =
    \|a-c\|_2^2+
    \|a-b\|_2^2-
    \|b-c\|_2^2,
\]
with $a=\theta_t$, $b=\alpha_{t+1}$, and $c=\theta^\ast_\gD$, we get
\[
\begin{aligned}
    2\langle \theta_t-\alpha_{t+1},\theta_t-\theta^\ast_\gD\rangle
    ={}&
    \|\theta_t-\theta^\ast_\gD\|_2^2
    +
    \|\theta_t-\alpha_{t+1}\|_2^2
    -
    \|\alpha_{t+1}-\theta^\ast_\gD\|_2^2.
\end{aligned}
\]
Since $\theta_t-\alpha_{t+1}=\eta\bar g_t$,
\[
    \|\theta_t-\alpha_{t+1}\|_2^2
    =
    \eta^2\|\bar g_t\|_2^2.
\]
Therefore,
\[
\begin{aligned}
    \langle \bar g_t,\theta_t-\theta^\ast_\gD\rangle
    ={}&
    \frac{1}{2\eta}
    \left(
        \|\theta_t-\theta^\ast_\gD\|_2^2
        -
        \|\alpha_{t+1}-\theta^\ast_\gD\|_2^2
    \right)
    +
    \frac{\eta}{2}\|\bar g_t\|_2^2.
\end{aligned}
\]

Because projection onto a closed convex set is non-expansive and $\theta^\ast_\gD\in\Theta$,
\[
    \|\theta_{t+1}-\theta^\ast_\gD\|_2
    =
    \|\pi_\Theta(\alpha_{t+1})-\pi_\Theta(\theta^\ast_\gD)\|_2
    \leq
    \|\alpha_{t+1}-\theta^\ast_\gD\|_2.
\]
Squaring both sides gives
\[
    \|\theta_{t+1}-\theta^\ast_\gD\|_2^2
    \leq
    \|\alpha_{t+1}-\theta^\ast_\gD\|_2^2.
\]
Multiplying by $-1$ reverses the inequality:
\[
    -\|\alpha_{t+1}-\theta^\ast_\gD\|_2^2
    \leq
    -\|\theta_{t+1}-\theta^\ast_\gD\|_2^2.
\]
Hence,
\[
\begin{aligned}
    \langle \bar g_t,\theta_t-\theta^\ast_\gD\rangle
    \leq{}&
    \frac{1}{2\eta}
    \left(
        \|\theta_t-\theta^\ast_\gD\|_2^2
        -
        \|\theta_{t+1}-\theta^\ast_\gD\|_2^2
    \right)
    +
    \frac{\eta}{2}\|\bar g_t\|_2^2.
\end{aligned}
\]
Substituting into the earlier convexity bound yields the one-step inequality
\[
\begin{aligned}
    \ell(\theta_t,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq{}&
    \frac{1}{2\eta}
    \left(
        \|\theta_t-\theta^\ast_\gD\|_2^2
        -
        \|\theta_{t+1}-\theta^\ast_\gD\|_2^2
    \right)
    \\
    &+
    \frac{\eta}{2}\|\bar g_t\|_2^2
    -
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle.
\end{aligned}
\]

Averaging over $t=0,\ldots,T-1$ gives
\[
\begin{aligned}
    \frac1T\sum_{t=0}^{T-1}
    \left(
        \ell(\theta_t,\gD)-\ell(\theta^\ast_\gD,\gD)
    \right)
    \leq{}&
    \frac{1}{2\eta T}
    \sum_{t=0}^{T-1}
    \left(
        \|\theta_t-\theta^\ast_\gD\|_2^2
        -
        \|\theta_{t+1}-\theta^\ast_\gD\|_2^2
    \right)
    \\
    &+
    \frac{\eta}{2T}\sum_{t=0}^{T-1}\|\bar g_t\|_2^2
    -
    \frac1T\sum_{t=0}^{T-1}
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle.
\end{aligned}
\]
The first sum telescopes:
\[
\begin{aligned}
    \sum_{t=0}^{T-1}
    \left(
        \|\theta_t-\theta^\ast_\gD\|_2^2
        -
        \|\theta_{t+1}-\theta^\ast_\gD\|_2^2
    \right)
    ={}&
    \|\theta_0-\theta^\ast_\gD\|_2^2
    -
    \|\theta_T-\theta^\ast_\gD\|_2^2
    \\
    \leq{}&
    \|\theta_0-\theta^\ast_\gD\|_2^2
    \leq
    D^2,
\end{aligned}
\]
where the last inequality uses $\theta_0,\theta^\ast_\gD\in\Theta$ and the fact that $\Theta$ has diameter $D$. Thus,
\[
\begin{aligned}
    \frac1T\sum_{t=0}^{T-1}
    \left(
        \ell(\theta_t,\gD)-\ell(\theta^\ast_\gD,\gD)
    \right)
    \leq{}&
    \frac{D^2}{2\eta T}
    +
    \frac{\eta}{2T}\sum_{t=0}^{T-1}\|\bar g_t\|_2^2
    \\
    &-
    \frac1T\sum_{t=0}^{T-1}
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle.
\end{aligned}
\]

By convexity of $\ell(\cdot,\gD)$ and the definition of $\bar\theta$,
\[
    \ell(\bar\theta,\gD)
    =
    \ell\left(\frac1T\sum_{t=0}^{T-1}\theta_t,\gD\right)
    \leq
    \frac1T\sum_{t=0}^{T-1}\ell(\theta_t,\gD).
\]
Therefore,
\[
\begin{aligned}
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq{}&
    \frac{D^2}{2\eta T}
    +
    \frac{\eta}{2T}\sum_{t=0}^{T-1}\|\bar g_t\|_2^2
    \\
    &-
    \frac1T\sum_{t=0}^{T-1}
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle.
\end{aligned}
\]

It remains to bound $\|\bar g_t\|_2^2$. Since $\bar g_t=g_t+n_t$,
\[
    \|\bar g_t\|_2^2
    =
    \|g_t+n_t\|_2^2.
\]
Using $\|a+b\|_2^2\leq 2\|a\|_2^2+2\|b\|_2^2$,
\[
    \|g_t+n_t\|_2^2
    \leq
    2\|g_t\|_2^2+2\|n_t\|_2^2.
\]
Since $\ell(\cdot,\gD)$ is $L$-Lipschitz, every subgradient satisfies $\|g_t\|_2\leq L$. Hence,
\[
    \|g_t+n_t\|_2^2
    \leq
    2L^2+2\|n_t\|_2^2.
\]
Therefore,
\[
\begin{aligned}
    \frac{\eta}{2T}\sum_{t=0}^{T-1}\|\bar g_t\|_2^2
    &\leq
    \frac{\eta}{2T}\sum_{t=0}^{T-1}
    \left(2L^2+2\|n_t\|_2^2\right)
    \\
    &=
    \eta L^2
    +
    \frac{\eta}{T}\sum_{t=0}^{T-1}\|n_t\|_2^2.
\end{aligned}
\]
Substituting this into the previous display gives
\[
\begin{aligned}
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq{}&
    \frac{D^2}{2\eta T}
    +
    \eta L^2
    +
    \frac{\eta}{T}\sum_{t=0}^{T-1}\|n_t\|_2^2
    \\
    &-
    \frac1T\sum_{t=0}^{T-1}
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle.
\end{aligned}
\]
Using the assumed bounds on the noise terms, we conclude that
\[
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    \frac{D^2}{2\eta T}
    +
    \eta L^2
    +
    \eta B_2
    +
    B_1.
\]
\end{proof}

We now have the following utility and privacy guarantee from Lemma B.4 of \citet{Cheu2021ShufflePS}. The privacy guarantee follows from the shuffle vector-summation protocol and its multi-round composition. For completeness, we prove the utility guarantee by instantiating \Cref{lemma:noisy_pgd_generic}.

\begin{lemma}[Shuffle-private convex optimizer]
\label{lemma:utility_shuffle_convex}
The protocol $\mathcal{P}_{\text{GD}}$ is multi-round $(\varepsilon,\delta)$ shuffle DP. Suppose $\ell(\cdot,\gD)$ is convex and $L$-Lipschitz over a convex set $\Theta\subset\mathbb{R}^d$ of diameter $D$. For any dataset $\gD=\{x_i\}_{i=1}^n$ and any $\eta>0$, the output of $\mathcal{P}_{\text{GD}}$ satisfies, with probability at least $1-\zeta$,
\[
\begin{aligned}
    \ell(\bar\theta,\gD)-\min_{\theta\in\Theta}\ell(\theta,\gD)
    \leq
    \widetilde O\left(
        \frac{D^2}{\eta T}
        +
        \eta L^2
        +
        \frac{\eta dT L^2}{n^2\varepsilon^2}
        +
        \frac{DL}{n\varepsilon}
    \right),
\end{aligned}
\]
where the $\widetilde O(\cdot)$ notation hides logarithmic factors in $n,d,T,1/\delta$, and $1/\zeta$. In particular, choosing
\[
    T=\frac{\varepsilon^2 n^2}{d\log^3(nd/\delta)}
    \qquad\text{and}\qquad
    \eta=\frac{D}{L\sqrt T},
\]
gives
\[
    \ell(\bar\theta,\gD)-\min_{\theta\in\Theta}\ell(\theta,\gD)
    \leq
    \widetilde O\left(
        \frac{DL\sqrt d}{\varepsilon n}
    \right).
\]
Equivalently, keeping the dominant logarithmic factor explicit,
\[
    \ell(\bar\theta,\gD)-\min_{\theta\in\Theta}\ell(\theta,\gD)
    \leq
    O\left(
        \frac{DL}{\varepsilon n}\sqrt{d\log^3(nd/\delta)}
    \right)
\]
up to additional logarithmic factors in $1/\zeta$.
\end{lemma}

\begin{proof}
The privacy statement is the multi-round shuffle-DP guarantee of the shuffle vector-summation protocol used in Algorithm~\ref{alg:shuffle_convex_optimizer}; see Lemma B.4 of \citet{Cheu2021ShufflePS}. We only prove the utility bound.

Let $g_t$ denote the true full-batch gradient at $\theta_t$, and write the noisy gradient returned by the shuffle protocol as
\[
    \bar g_t=g_t+n_t.
\]
By the utility guarantee of the shuffle vector-summation protocol, each coordinate of $n_t$ is mean-zero sub-Gaussian with variance proxy
\[
    \tau^2
    =
    O\left(
        \frac{T L^2\log^2(d^2T/\delta)}{n^2\varepsilon^2}
    \right).
\]
We now verify the two noise conditions required by \Cref{lemma:noisy_pgd_generic}.

First, since each $n_{t,j}$ is sub-Gaussian with variance proxy $\tau^2$, each $n_{t,j}^2$ is sub-exponential with scale controlled by $\tau^2$. Therefore, by concentration for sums of sub-exponential random variables, with probability at least $1-\zeta/2$,
\[
    \sum_{t=0}^{T-1}\sum_{j=1}^d n_{t,j}^2
    \leq
    \widetilde O(dT\tau^2).
\]
Since
\[
    \sum_{t=0}^{T-1}\|n_t\|_2^2
    =
    \sum_{t=0}^{T-1}\sum_{j=1}^d n_{t,j}^2,
\]
we get
\[
    \frac1T\sum_{t=0}^{T-1}\|n_t\|_2^2
    \leq
    \widetilde O(d\tau^2).
\]
Thus we may take
\[
    B_2=\widetilde O(d\tau^2).
\]

Second, we bound the inner-product noise term. Conditioned on the history before round $t$, the iterate $\theta_t$ is fixed, while $n_t$ is mean-zero sub-Gaussian coordinate-wise. Since $\theta_t,\theta^\ast_\gD\in\Theta$ and $\Theta$ has diameter $D$,
\[
    \|\theta_t-\theta^\ast_\gD\|_2\leq D.
\]
Hence the scalar random variable
\[
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle
\]
is mean-zero sub-Gaussian with variance proxy at most $O(\tau^2D^2)$. Summing over $t=0,\ldots,T-1$, we get that
\[
    \sum_{t=0}^{T-1}\langle n_t,\theta_t-\theta^\ast_\gD\rangle
\]
is sub-Gaussian with variance proxy at most $O(T\tau^2D^2)$. Thus, with probability at least $1-\zeta/2$,
\[
    \left|
    \sum_{t=0}^{T-1}\langle n_t,\theta_t-\theta^\ast_\gD\rangle
    \right|
    \leq
    \widetilde O\left(D\tau\sqrt{T}\right),
\]
and therefore
\[
    \left|
    \frac1T\sum_{t=0}^{T-1}\langle n_t,\theta_t-\theta^\ast_\gD\rangle
    \right|
    \leq
    \widetilde O\left(\frac{D\tau}{\sqrt T}\right).
\]
Thus we may take
\[
    B_1=\widetilde O\left(\frac{D\tau}{\sqrt T}\right).
\]

Applying \Cref{lemma:noisy_pgd_generic}, with probability at least $1-\zeta$,
\[
\begin{aligned}
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    \widetilde O\left(
        \frac{D^2}{\eta T}
        +
        \eta L^2
        +
        \eta d\tau^2
        +
        \frac{D\tau}{\sqrt T}
    \right).
\end{aligned}
\]
Substituting
\[
    \tau^2
    =
    O\left(
        \frac{T L^2\log^2(d^2T/\delta)}{n^2\varepsilon^2}
    \right)
\]
and hiding logarithmic factors gives
\[
\begin{aligned}
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    \widetilde O\left(
        \frac{D^2}{\eta T}
        +
        \eta L^2
        +
        \frac{\eta dT L^2}{n^2\varepsilon^2}
        +
        \frac{DL}{n\varepsilon}
    \right).
\end{aligned}
\]
Finally, choose $\eta=D/(L\sqrt T)$. Then
\[
    \frac{D^2}{\eta T}
    =
    \frac{DL}{\sqrt T},
    \qquad
    \eta L^2
    =
    \frac{DL}{\sqrt T},
\]
and
\[
    \frac{\eta dT L^2}{n^2\varepsilon^2}
    =
    \frac{D}{L\sqrt T}\cdot\frac{dT L^2}{n^2\varepsilon^2}
    =
    \frac{DLd\sqrt T}{n^2\varepsilon^2}.
\]
Balancing $DL/\sqrt T$ and $DLd\sqrt T/(n^2\varepsilon^2)$ gives $T\asymp \varepsilon^2 n^2/d$ up to logarithmic factors. With
\[
    T=\frac{\varepsilon^2 n^2}{d\log^3(nd/\delta)},
\]
we obtain
\[
    \ell(\bar\theta,\gD)-\min_{\theta\in\Theta}\ell(\theta,\gD)
    \leq
    \widetilde O\left(
        \frac{DL\sqrt d}{\varepsilon n}
    \right).
\]
Keeping the main displayed logarithmic factor gives
\[
    \ell(\bar\theta,\gD)-\min_{\theta\in\Theta}\ell(\theta,\gD)
    \leq
    O\left(
        \frac{DL}{\varepsilon n}\sqrt{d\log^3(nd/\delta)}
    \right)
\]
up to additional logarithmic factors in $1/\zeta$.
\end{proof}

We now present the analysis for the full-batch DP-SGD optimizer in terms of zero-concentrated differential privacy \cite{cryptoeprint:concentratedDP}. This gives better composition guarantees without assuming that the total privacy budget $\varepsilon$ is small.

\begin{lemma}[Noisy full-batch PGD under zCDP]
\label{lemma:noisy_full_batch_pgd_zcdp}
Suppose $\ell(\cdot,\gD)$ is convex and $L$-Lipschitz over a closed convex set $\Theta\subset\mathbb{R}^d$ of diameter $D$. Let
\[
    \theta^\ast_\gD \in \arg\min_{\theta\in\Theta}\ell(\theta,\gD).
\]
Consider full-batch projected gradient descent with Gaussian perturbations:
\[
    \theta_{t+1}
    =
    \pi_\Theta(\theta_t-\eta(g_t+n_t)),
    \qquad
    g_t\in \partial\ell(\theta_t,\gD),
\]
where $n_t\sim\mathcal{N}(0,\sigma^2 I_d)$ independently across $t=0,\ldots,T-1$, and
\[
    \sigma^2=\frac{2L^2T}{n^2\rho}.
\]
Under replacement adjacency, the sequence of $T$ noisy gradients is $\rho$-zCDP. Moreover, with probability at least $1-\zeta$,
\[
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    O\left(
        \frac{D^2}{\eta T}
        +
        \eta L^2
        +
        \eta d\sigma^2
        +
        D\sigma\sqrt{\frac{\log(1/\zeta)}{T}}
    \right).
\]
In particular, choosing
\[
    \eta=\frac{D}{L\sqrt T}
    \qquad\text{and}\qquad
    T=\frac{\rho n^2}{d}
\]
gives
\[
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    \widetilde O\left(
        \frac{DL\sqrt d}{n\sqrt\rho}
    \right).
\]
\end{lemma}

\begin{proof}
We first prove the privacy guarantee. Since $\ell(\theta,\gD)=\frac1n\sum_{i=1}^n\ell(\theta,x_i)$ and each per-example loss is $L$-Lipschitz, each per-example subgradient has Euclidean norm at most $L$. Under replacement adjacency, changing one data point can therefore change the full-batch gradient by at most $\Delta=\frac{2L}{n}$ in $\ell_2$ norm. A Gaussian mechanism with $\ell_2$-sensitivity $\Delta$ and covariance $\sigma^2 I_d$ is
$\frac{\Delta^2}{2\sigma^2}$ zCDP. Hence each noisy gradient release is
\[
    \rho_0
    =
    \frac{(2L/n)^2}{2\sigma^2}
    =
    \frac{2L^2}{n^2\sigma^2}
\]
zCDP. By adaptive composition of zCDP mechanisms \cite{cryptoeprint:concentratedDP}, the $T$ releases are
\[
    T\rho_0
    =
    \frac{2TL^2}{n^2\sigma^2}
\]
zCDP. Substituting $\sigma^2=2L^2T/(n^2\rho)$ gives $T\rho_0 = \frac{2TL^2}{n^2}\cdot\frac{n^2\rho}{2L^2T}= \rho$.

Thus the full optimizer is $\rho$-zCDP.

We next prove the utility guarantee by applying \Cref{lemma:noisy_pgd_generic}. Since $n_t\sim\mathcal{N}(0,\sigma^2I_d)$,
\[
    \frac{\|n_t\|_2^2}{\sigma^2}\sim \chi_d^2.
\]
Therefore,
\[
    \frac{1}{\sigma^2}\sum_{t=0}^{T-1}\|n_t\|_2^2
    \sim
    \chi_{dT}^2.
\]
By standard chi-square concentration, with probability at least $1-\zeta/2$,
\[
    \sum_{t=0}^{T-1}\|n_t\|_2^2
    \leq
    O\left(dT\sigma^2+\sigma^2\log(1/\zeta)\right).
\]
Dividing by $T$ gives
\[
    \frac1T\sum_{t=0}^{T-1}\|n_t\|_2^2
    \leq
    O\left(d\sigma^2+\frac{\sigma^2\log(1/\zeta)}{T}\right).
\]
Up to logarithmic and lower-order terms, we may take
\[
    B_2=O(d\sigma^2).
\]

It remains to bound the inner-product term. Conditioned on the history before round $t$, the iterate $\theta_t$ is fixed and $n_t$ is independent Gaussian noise. Therefore,
\[
    \langle n_t,\theta_t-\theta^\ast_\gD\rangle
\]
is a mean-zero Gaussian random variable with conditional variance
\[
    \sigma^2\|\theta_t-\theta^\ast_\gD\|_2^2.
\]
Since $\theta_t,\theta^\ast_\gD\in\Theta$ and $\Theta$ has diameter $D$,
\[
    \|\theta_t-\theta^\ast_\gD\|_2\leq D.
\]
Thus the conditional variance is at most $\sigma^2D^2$. Consequently,
\[
    \sum_{t=0}^{T-1}\langle n_t,\theta_t-\theta^\ast_\gD\rangle
\]
is sub-Gaussian with variance proxy at most $T\sigma^2D^2$. Hence, with probability at least $1-\zeta/2$,
\[
    \left|
    \sum_{t=0}^{T-1}\langle n_t,\theta_t-\theta^\ast_\gD\rangle
    \right|
    \leq
    O\left(D\sigma\sqrt{T\log(1/\zeta)}\right).
\]
Dividing by $T$ gives
\[
    \left|
    \frac1T\sum_{t=0}^{T-1}\langle n_t,\theta_t-\theta^\ast_\gD\rangle
    \right|
    \leq
    O\left(D\sigma\sqrt{\frac{\log(1/\zeta)}{T}}\right).
\]
Thus we may take
\[
    B_1=O\left(D\sigma\sqrt{\frac{\log(1/\zeta)}{T}}\right).
\]

Applying \Cref{lemma:noisy_pgd_generic} gives, with probability at least $1-\zeta$,
\[
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    O\left(
        \frac{D^2}{\eta T}
        +
        \eta L^2
        +
        \eta d\sigma^2
        +
        D\sigma\sqrt{\frac{\log(1/\zeta)}{T}}
    \right).
\]

Finally, substitute $\eta=D/(L\sqrt T)$ and $\sigma^2=2L^2T/(n^2\rho)$. The first term becomes
\[
    \frac{D^2}{\eta T}
    =
    \frac{D^2}{(D/(L\sqrt T))T}
    =
    \frac{DL}{\sqrt T}.
\]
The second term becomes
\[
    \eta L^2
    =
    \frac{D}{L\sqrt T}L^2
    =
    \frac{DL}{\sqrt T}.
\]
The third term becomes
\[
    \eta d\sigma^2
    =
    \frac{D}{L\sqrt T}\cdot d\cdot \frac{2L^2T}{n^2\rho}
    =
    \frac{2DLd\sqrt T}{n^2\rho}.
\]
Choosing $T=\rho n^2/d$, we have
\[
    \frac{DL}{\sqrt T}
    =
    \frac{DL\sqrt d}{n\sqrt\rho},
\]
and
\[
    \frac{2DLd\sqrt T}{n^2\rho}
    =
    \frac{2DLd}{n^2\rho}\sqrt{\frac{\rho n^2}{d}}
    =
    \frac{2DL\sqrt d}{n\sqrt\rho}.
\]
The final noise inner-product term satisfies
\[
    D\sigma\sqrt{\frac{\log(1/\zeta)}{T}}
    =
    D\sqrt{\frac{2L^2T}{n^2\rho}}\sqrt{\frac{\log(1/\zeta)}{T}}
    =
    \frac{\sqrt 2DL}{n\sqrt\rho}\sqrt{\log(1/\zeta)},
\]
which is lower order than the displayed $\sqrt d$ term up to logarithmic factors when $d\geq 1$. Therefore,
\[
    \ell(\bar\theta,\gD)-\ell(\theta^\ast_\gD,\gD)
    \leq
    \widetilde O\left(
        \frac{DL\sqrt d}{n\sqrt\rho}
    \right).
\]
\end{proof}


==> temp_svt_old.tex <==
We now prove this lemma below. One can observe that that our construction of the sets $\gT_o$ is inspired from  the sparse vector technique \cite[Algorithm 2]{dworkdpbook} and we restate it below.

However, we are unable to directly apply the privacy-utility guarantees of the sparse vector technique directly in our case as in our case the query $||x||_{\tV^{-1}}$ uses the value of $\tV$ that was computed from the previous step and thus it has a notion of a running internal state that may not be observed by an adversary. We thus reprove the privacy-utility guarantees for our setup below.

%For clarity, we restate the utility privacy guarantees of the sparse vector technique from \cite[Section 3.6]{dworkdpbook}. 

Recall that the sensitive of query $f$ is defined by $\Delta(f) := \max_{D \sim D'} |f(D) - f(D')|$ where $D$ and $D'$ are neighbouring datasets with at most one entry changed. 

\begin{algorithm}
\caption{Sparse($D$, $\{f_i\}$, $\srT$, $c$, $\epsilon$, $\delta>0$)}

\textbf{Input:} A private database $D$, an adaptively chosen stream of sensitivity 1 queries $f_1, \ldots$, a threshold $\srT$, and a cutoff point $c$\\
\textbf{Output:} A stream of answers $a_1, \ldots$

\begin{algorithmic}[1]


\State $\sigma = \sqrt{\frac{32c \ln \frac{1}{\delta}}{\epsilon^2}}$


\State $\hat{\srT}_0 = \srT + \textrm{Lap}(\sigma)$ and set $\textrm{count} = 0$

\For{Each query $i$}
    \State $\nu_i = \textrm{Lap}(2\sigma)$
    
    \If{$f_i(D) + \nu_i \geq \hat{\srT}_{\textrm{count}}$}
    
        \State Output $a_i = \top$\\
        \State Let $\textrm{count} = \textrm{count} + 1$
        \State Let $\hat{\srT}_{\textrm{count}} = \srT + \textrm{Lap}(\sigma)$
    
    \Else
    
        \State Output $a_i = \bot$
    
    \EndIf
    
    
    \If{$\textrm{count} \geq c$}
    
    \State Halt

    \EndIf
    
\EndFor
\end{algorithmic}

\end{algorithm}


% We now present the accuracy definition of \cite[Definition 3.9]{dworkdpbook}.

% \begin{definition}[Accuracy \cite{dworkdpbook}]
% We will say that an algorithm which outputs a stream of answers $a_1, \ldots, \in \{\top, \bot\}^*$ in response to a stream of $k$ queries $f_1, \ldots, f_k$ is $(\alpha, \beta)$-accurate with respect to a threshold $T$ if except with probability at most $\beta$, the algorithm does not halt before $f_k$, and for all $a_i = \top$: $f_i(D) \geq \srT - \alpha$ and for all $a_i = \bot$: $f_i(D) \leq \srT + \alpha$
% \end{definition}

% The following lemma states the utility/privacy guarantee of the sparse vector algorithm.

% \begin{theorem}[Utility-Privacy Guarantee \cite{dworkdpbook}]{\label{theorem:sparse_vector_accuracy}}
% For any sequence of $T$ queries $f_1, \ldots, f_T$ such that $L(\srT) \equiv |\{i : f_i(D) \geq \srT - \alpha\}| \leq c$. Sparse is $(\alpha, \beta)$ accurate for:
% \[
% \alpha = \left(\ln k + \ln \frac{2c}{\beta}\right) \sqrt{\frac{512c \ln \frac{1}{\delta}}{\epsilon^2}}
% \]
% Further, sparse is $(\epsilon,\delta>0)$ differentially private.
% \end{theorem}



Now one can view our algorithm below only consisting of the part where the set $\gT_o$ and $\tV$ is updated. For convenience, restate it in Algorithm \ref{alg:glm_adversarial_switching_criterion_I} below only the part that consists of $\tV$ and running set $\gT_o$. 


Further, recall that $\gR_t$ is a symmetric regualrizer matrix added at each step to compute a private sum.


We now prove the following lemma assuming that \cref{ass:regularizer_noise} holds. More specifically, we assume that $\tV \succeq \lambdalone \mI + \sum\limits_{t \in \gT_o} x_t x^{\top}_t$ at every step $t$ for proving the lemma.
 

% \begin{lemma}
%     Suppose $\tV \succeq \lambdalone\mI+ \sum\limits_{t \in \gT_o} x_t x^{\top}_t$ at every time step $t$ and $c > \left|\left\{t: \max_{x \in \gX_t} \left|\left| x\right|\right|^2_{\tV^{-1}} \geq \frac{1}{4 \gamma^2 \kappa R^2}\right\}\right|$ and $\lambdalone $ 
% \end{lemma}






% Let $\tV_t$ denote the value of $\tV$ at the $t^{th}$ time step. Further, denote the dataset $\gD = \{r_t,\gX_t\}_{t=1}^{T}$ and thus, $\{\tV_t\}_{t=1}^{T}$ can be viewed as a randomized function over the dataset $\gD$.

% Now, we define $f_t(\gD) = \lambdalone \max_{x\in \gX_t} \left|\left|x\right|\right|_{\tV_t^{-1}}$ which clearly has sensitivity one. We now prove the following lemma which effectively upper bounds $|\{i:f_i(D) \geq T- \alpha\}|$ for our case for 

\sss{To prove that the if condition holds true and then the desired lemma directly follows. invoke a variant of \cite[Lemma B.11]{sawarni2024generalizedlinearbanditslimited}}

\sss{New approach: Not using the sparse vector lemma as the queries depend on the running vector $\tV$ (which depends on previous evaluations) thus, reprove it for our case. }


\sss{Tried again more issues. See the standard lemma the error in prediction is typically much more than the sensitivity of the query in our case the sensitivity of the query is the range, thus will not work in our case as the predictions would go outside range. }

We now prove the following lemma. 

\begin{lemma}{\label{lemma:upper_bounding_policy_1_switch_lower_level}}
    Setting $\lambdalone \geq \frac{8\gamma^2\kappa R^2}{\epsilon}\log (32T/\zeta)) \sqrt{128\ccut \log (8/\delta)}$ and $\ccut =  8dR^2 \kappa \gamma^2 \log T$, we have the following with probability at least $1- \min \left(\delta/8, \zeta/8\right)$
    
    \begin{itemize}
        \item Any index $t$ with $\max\limits_{x \in \gX_t} ||x||^2_{\tV^{-1}} \geq \frac{3}{4 \gamma^2 \kappa R^2}$ is selected into $\gT_o$.
        \item Any index $t$ with $\max\limits_{x \in \gX_t} ||x||^2_{\tV^{-1}} \leq \frac{1}{4 \gamma^2 \kappa R^2}$ is never selected into $\gT_o$.
        \item The variable $\text{count}$ never exceeds the threshold $\ccut$.
    \end{itemize}
    
    
\end{lemma}

While this proof is inspired from \cite[Lemma B.12]{sawarni2024generalizedlinearbanditslimited}, it has an interesting variation. %as it also used techniques from Theorem \ref{theorem:sparse_vector_accuracy} in its proof.

\begin{proof}

        Observe that the noise added at every step $t$ in the comparison is given by $\nu_t$ and $\hat{n}_{\text{count}}$ where $\text{count}$ is the running value at each time step.

        Denote the set of indices $t$ where $\max_{x \in \gX_t} \left|\left|x\right|\right|_{\tV^{-1}} \geq \frac{1}{4\gamma^2 \kappa R^2}$ by $\gT^{(u)}_o$. We first show that $\gT_o \subseteq \gT^{(u)}_o$ with high probability where $\gT_o$ denotes the computed set at the end of the $T$ time steps. Further, let $\overline{ \text{count}}$ denote the value of the variable $\text{count}$ at the end of $T$ timesteps. 

        \begin{align}
            \mathbb{P}\left[ \gT_o \setminus \gT^{(u)}_o \neq \emptyset \right] \leq &\mathbb{P} \left[ \max_{t \in [T]} |\nu_t| \geq \frac{\lambdalone}{8\gamma^2 \kappa R^2} \cup \max_{t \in [\overline{ \text{count}}]} |\hat{n}_t| \geq \frac{\lambdalone}{8\gamma^2 \kappa R^2}\right]\\
            \overset{(a)}{\leq} & 2T\exp\left( \frac{-\epsilon}{\left(128 \ccut \log (8/\delta)\right)^{1/2}} \frac{\lambdalone}{8 \gamma^2 \kappa R^2}\right)\leq \zeta/16
        \end{align}

        The bound $(a)$ follows applying union bound and the fact that $\mathbb{P}[|Y|> t] = \exp(-\frac{t}{b})$ where $Y \sim \text{Lap}(b)$. We also upper bound $\ccut$ by $T$.


        
        Now, denote the set of indices $t$ where $\max_{x \in \gX_t} \left|\left|x\right|\right|_{\tV^{-1}} \geq \frac{1}{4\gamma^2 \kappa R^2}$ by $\gT^{(l)}_o$. One can use a very similar technique to bound the probability of the event $\gT^{(l)}_o \setminus \gT_o \neq \emptyset$ by $\zeta/16$. Thus, with probability at least $1- \zeta/8$, we have $\gT^{(l)}_o \subseteq \gT_o \subseteq \gT^{(u)}_o$.

        We now prove the third point in the lemma bounding the value of variable $\text{count}$ assuming this event $\gT^{(l)}_o \subseteq \gT_o \subseteq \gT^{(u)}_o$ holds.

        Further, we now define $\tV_t$ as the value of $\tV$ at time step $t$ and thus we have, $\tV_t \succeq \lambdalone \mI+ \sum_{t \in \gT_o} x_t x^{\top}_t$. 

        Thus, wherever the switching criterion is satisfied, we have $||x||^2_{\tV^{-1}} \geq \frac{1}{4\gamma^2 \kappa R^2}$ which further implies that 

        \begin{equation}
            \sum_{t \in \gT_o} ||x_t||^2_{\tV^{-1}} \geq \frac{|\gT_o|}{4 \gamma^2 \kappa R^2}
        \end{equation}


        However, applying the elliptic potential lemma (lemma \ref{lemma:elliptic_potential}), we have $\sum_{t \in \gT_o} ||x_t||^2_{\tV^{-1}} \leq 2d \log \left(1+ \frac{|\gT_o|}{\lambdalone d}\right)$ \footnote{One could bound $\tV \succeq \lambdalone \mI+ \sum_{t \in \gT_o} x_t x^{\top}_t$ and then apply the lemma.}

        Thus, we get $|\gT_o| \leq 8dR^2 \kappa \gamma^2 \log T$ as $\lambdalone > 1$ which further implies that the third point in lemma holds. 
        
\end{proof}


\begin{lemma}{\label{lemma:upper_bounding_policy_1_privacy}}
    The set of constructed indices $\{\gT_{o,t}\}_{t=1}^{T}$ is $(\epsilon/8,\delta/8)$ differentially private with respect to $\{r_t,\gX_t\}_{t=1}^{T}$ where $\gT_{o,t}$ denotes the set $\gT_o$ in Algorithm \ref{alg:glm_adversarial_switching_criterion_I} at time step $t$.
\end{lemma}

From the previous lemma, we know that the size of the set $\gT_o$ is bounded by $\ccut$ with high probability. We prove this lemma by invoking the advanced composition theorem \cite[Theorem 3.20]{dworkdpbook}.

We first show that the computation of first entry of the set $\gT_o$ is $(\epsilon/\sqrt{512\ccut \log (8/\delta)},0)$ private using an approach almost similar to \cite[Theorem 3.23]{dworkdpbook}.

\begin{lemma}
    The smallest index of the computed set $\gT_o$ is $(\epsilon/\left(8\sqrt{2\ccut \log (8/\delta)}\right),0)$ differentially private with respect to the dataset $\{r_t,\gX_t\}_{t=1}^{T}$.
\end{lemma}

\begin{proof}
    Consider two neighboring datasets $\gD$ and $\gD'$ over reward actions pairs at all time-steps. Let the first entry of the set $\gT_o$ be given by $\gT_{o,1}(\gD)$ when the algorithm \ref{alg:glm_adversarial_switching_criterion_I} is run on the dataset $\gD = \{r_t,\gX_t\}_{t=1}^{T}$ 


    First we denote the threshold $\frac{\lambdalone}{2 \gamma^2 \kappa R^2}$ as $\hat \srT$. We now consider the event that the first entry of $\gT_o(\gD)$ equals $k$. Now observe that there are two types of randomness in the algorithm: the noisy threshold $\hat{\srT} = \srT + \text{Lap}(\sigma_q)$ and the computed values $\{\nu_1, \nu_2, \nu_k\} \overset{\text{i.i.d}}{\sim} \text{Lap}(\sigma_q)$. For the following analysis, we denote 

    \begin{equation}
        g(\gD) = \max_{t <k} \left(\lambdalone \max_{x \in \gX_t} ||x||^2_{\tV^{-1}} + \nu_t\right) \text{ where $\tV$ denotes its value in Algorithm \ref{alg:glm_adversarial_switching_criterion_I} at start of $t^{th}$ step}
    \end{equation}

    Further, let $f_t(\gD) = ||x||^2_{\tV^{-1}}$ where $\tV$ denotes its value in Algorithm \ref{alg:glm_adversarial_switching_criterion_I} at start of $t^{th}$ step.


    Further, in the following analysis we arbitraily fix the values of $\nu_1, \nu_2, \ldots, \nu_{k-1}$ and take probabilities over randomness in $\nu_k$ and $\hat \srT$. Further, we abuse notation and use $\text{Pr}(\hat \srT = t)$ as a shorthand notation for the pdf of $\hat \srT$ (and similarly for $\nu_k$). Note that fixing 
    the values of $\nu_1, \ldots, \nu_{k-1}$ makes $g(D)$ a deterministic quantity.

    \begin{align}
\Pr_{\hat \srT, \hat{\nu}_k}[\gT_{o,1}(\gD) = k] &= \Pr_{\hat \srT, {\nu}_k}[\hat \srT > {g}(\gD) \text{ and } f_k(\gD) + \nu_k \geq \hat{\srT}] \\
&= \Pr_{\hat \srT, {\nu}_k} [\hat{\srT} \in (g(\gD), f_k(D) + \nu_k]] \\
&= \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} \Pr[\nu_k = v] \cdot \Pr[\hat{\srT} = t] \mathbf{1}[t \in (g(\gD), f_k(\gD) + v]] \, dv \, dt \\
\end{align}



We now make a change of variables. Define: \\
\begin{align}
    {v}' &= v + g(\gD) - g(\gD) + f_k(\gD') - f_k(\gD) \\
{t}' &= t + g(\gD) - g(\gD')
\end{align}

and note that for any $\gD, \gD'$, $|{v}' - v| \leq 2$ and $|{t}' - t| \leq 1$. This follows because each query $f_i(D)$ 
is 1-sensitive, and hence the quantity $g(D)$ is 1-sensitive as well. 
Applying this change of variables, we have

\begin{align}
(I) &= \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} \Pr[\nu_k = {v}'] \cdot \Pr[\hat{\srT} = {t}'] \mathbf{1}[(t + g(\gD) - g(\gD')) \in (g(\gD), f_k(\gD') + v + g(\gD) - g(\gD'))]] \, dv \, dt \\
&= \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} \Pr[\nu_k = \hat{v}] \cdot \Pr[\hat{\srT} = \hat{t}] \mathbf{1}[t \in (g(\gD'), f_k(\gD') + v)]  \, dv \, dt \\
&\leq \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} \exp(\epsilon/2) \Pr[\nu_k = v] \cdot \exp(\epsilon/2) \Pr[\hat{\srT} = t] \mathbf{1}[t \in (g(\gD'), f_k(\gD') + v)] \, dv \, dt \\
&= \exp(\epsilon) \Pr_{\hat{\srT}, \nu_k}[\hat{\srT} > g(\gD') \text{ and } f_k(\gD') + \nu_k \geq \hat{\srT}] \\
&= \exp(\epsilon) \Pr_{\hat{\srT}, \nu_k}[\gT_{o,1}(\gD') = k]
\end{align}


The inequality comes from our bounds on $|v' - v|$ and $|t' - t|$ and
the form of the pdf of the Laplace distribution 

This completes the proof.
    
\end{proof}


We prove lemma \ref{lemma:upper_bounding_policy_1_privacy} via a direct application of the advanced composition theorem.


\begin{proof}
    One can view the construction of the set $\gT_{o}$ as repeated calls to the same process that was used to compute the first element. This is because after the count increases by unity, the noise $\hat n_{\text{count}}$ is resampled and the algorithm moves indentically. One can thus apply the advanced composition theorem \cite[Theorem 3.20]{dworkdpbook} to prove the desired bound as the cardinality of the set $\gT_o$ is bounded by $\ccut$.
\end{proof}


%     Recall from \Cref{lemma:utility_privacy_glm_adv_3} that \Cref{ass:sco_loss} is satisfied with $\nu_1 = O\left(\frac{R^3S^2 \gamma \sqrt{d\kappa \log (8/\delta) \log T}}{\varepsilon} \sqrt{d \log^2 (Td/\delta)}\right)$ and now consider the parametric form \Cref{eq:parametric_form_gamma_glm_adv} for the chosen values of $\lambda$ and $\gamma$ from \Cref{alg:jdp_glm_adversarial}.
    %     \begin{align}
    %         \gamma(\lambdau) \leq & 4R^2S \sqrt{\lambdau} + \frac{7Sd}{\sqrt{\lambdau}} \log \left(\frac{16T}{\zeta R^2 d\lambdau} \right) + 4RS\sqrt{\nu_1} \nonumber\\
    %         \leq & 5R^2 S \sqrt {\lambdal} + \frac{7Sd}{\sqrt \lambdal} \log \left(16T/\zeta\right) + O\left(4R^{2.5}S^{2} \frac{\sqrt{d\gamma \sqrt \kappa \log T}}{\sqrt{\varepsilon}} \log^{0.5}(8/\delta)\right) \\
    %         \leq & CR^2S\sqrt{d \log\left(\frac{16T}{\zeta}\right)} + O\left(4R^{2.5}S^{2} \frac{\sqrt{d\sqrt \kappa} \sqrt {\log T}}{\sqrt{\varepsilon}} \log^{0.5}(8/\delta)\right) \sqrt \gamma \\
    %         & \hspace{12 em} + \frac{30R^2S}{ \sqrt{\varepsilon \kappa^{\ast}}} \sqrt{\log (32/\delta)} \sqrt{\log T} (\log (16T/\zeta)^{0.25} + d^{0.25})
    %     \end{align}

    %     The first inequality follows since $\lambdau/\lambdal = \frac{4 \sqrt d +2}{4 \sqrt d} \leq 6/4$ and the last inequality follows since $\lambdal \geq d \log (16T/\zeta)$. % and the fact that $\varepsilon < 9$.

    % \ss{Include $\kappa$ in $\gamma$ as well.}

    % Now choosing $\sqrt{\gamma} \geq \Theta\left( \frac{R^{2.5} S^{2} \sqrt {d\sqrt \kappa} \log (Td/\zeta) \sqrt{\log (32/\delta)}}{\sqrt {\varepsilon \kappa^{\ast}} }\right) + \Theta\left(\sqrt{CR^2S\sqrt{\frac{d \log (1/\delta)}{\min(\varepsilon \kappa^{\ast},1)}} \sqrt{\log\left(\frac{16T}{\zeta}\right)} \left(\log (16T/\zeta)^{0.25}+d^{0.25}\right)} \right)$ ensures that $\gamma(\lambdau) \leq \gamma$. This follows from the fact that $x \geq b+ \sqrt c \implies x^2 \geq bx+c$.


    % Thus, choosing $\gamma = \frac{CR^{5} S^{4} d \sqrt \kappa \log^2 (Td/\zeta) \log (32/\delta)}{\min(\varepsilon\kappa^{\ast},1) }$ for some appropriate constant $C$ ensures that the bound $\gamma(\lambdau) \leq \gamma$ holds.

    % We now prove a similar result for $\beta(\lambdau,\lambdal) \leq \beta$ where $\beta$ chosen in \Cref{alg:jdp_glm_adversarial} as $\beta(\lambdau,\lambdal)$ defined from \Cref{eq:beta_parametrized_glm_adv}. %Recall from \Cref{lemma:utility_privacy_glm_adv_3} that $\nu_2 = O\left( \frac{RS^2}{\varepsilon} \sqrt{d \log^3 (Td/\delta)\log (8/\delta)} \right)$

    % %\sss{check this calculation.}


    % \ss{Tighten this optimization bound}
    % \begin{align}
    %     \beta(\lambdau, \lambdal) & = 4R \frac{\lambdau}{\sqrt{\lambdal}} + \frac{7d}{R\sqrt{\lambdal}} \log \left(\frac{16 T}{\zeta R^2 d\lambdal}\right) + 10\sqrt{\nu_2} \\
    %     \leq & 5R \sqrt \lambdau + \frac{7d}{R \sqrt{\lambdal}} \log (16T/\zeta) + 10 \sqrt \nu_2\\
    %     \leq & 7 R \sqrt{d \log \left(16T/ \zeta\right)}+ \frac{30R^2S \sqrt{4 \sqrt d +1}}{ \sqrt{\varepsilon \kappa^{\ast}}} \sqrt{\log (32/\delta)} \sqrt{\log T }(\left(\log (16T/\zeta)\right)^{0.25} + d^{0.25}) \\
    %     & \hspace{20 em}+ O\left(\frac{R^{2.5}S}{\sqrt \varepsilon} (d^{0.25} + (\log T)^{0.25}) \left(d\log (T)\log (8/\delta)\right)^{0.25}\right)\\
    %     \leq & 7 R \sqrt{d \log \left(16T/ \zeta\right)} + O\left(\frac{R^{2.5}S}{\sqrt {\varepsilon \kappa^\ast}} d^{0.5} \sqrt{\log (T)\log (8/\delta)} \right) + O\left(\frac{R^{2.5}Sd^{0.25}}{\sqrt \varepsilon} (\log (T/\zeta))^{3/4}\right)
    % \end{align}


==> utility_privacy_regualarizer.tex <==
\section{Binary tree addition mechanism}

\noindent\textbf{Lemma~\ref{lemma:utility_privacy_glm_adv_1} (Restated):}
\lemmadputilitytwo

We prove this result using the 
